Counting Homomorphisms to Trees Modulo a Prime

Many important graph theoretic notions can be encoded as counting graph homomorphism problems, such as partition functions in statistical physics, in particular, independent sets and colourings. In this article we study the complexity of $\#_p\mathsf{H}$OMS$\mathsf{T}$O$H$, the problem of counting graph homomorphisms from an input graph to a graph $H$ modulo a prime number $p$. Dyer and Greenhill proved a dichotomy stating that the tractability of non-modular counting graph homomorphisms depends on the structure of the input graph. Many intractable cases in non-modular counting become tractable in modular counting due to the common phenomenon of cancellation. However, in subsequent studies on counting modulo $2$ the influence, the structure of $H$ has on the tractability, was shown to persist, yielding similar dichotomies. Our main result shows that for every tree $H$ and every prime $p$ the problem $\#_p\mathsf{H}$OMS$\mathsf{T}$O$H$ is either polynomial time computable or $\#_p\mathsf{P}$-complete. This addresses the conjecture of Faben and Jerrum stating this dichotomy for every graph $H$ when counting modulo 2. In order to prove this result, we study the structural properties of a homomorphism. As an important interim, this study yields a dichotomy for the problem of weighted counting independent sets in a bipartite graph modulo some prime $p$. Our results are the first suggesting that such dichotomies hold not only for the one-bit functions of the modulo~2 case but for the modular counting functions of all primes $p$.

==> asym_trees.tex <==
\subsection{Introduction: Asymmetric trees}

In this chapter we study the complexity of \phcol{} when~$p$ is a prime and~$H$ is an asymmetric tree. 
Asymmetric trees are connected graphs that have no cycles and their automorphism group only contains the trivial 
automorphism. To state the main theorem of this chapter recall Definition~\ref{defn:reduced-form} 
(Page~\pageref{defn:reduced-form}) of the order~$p$ reduced form $H^{*p}$ of a graph $H$.

{\renewcommand{\thetheorem}{\ref{thm:main-trees}}
\begin{theorem}
 Let $p$ be a prime and let $H$ be a graph where $H^{*p}$ is an asymmetric tree. If $H^{*p}$ has 
more than one vertex then \phcol{} is $\numpp$-hard, otherwise \phcol{} is computable in polynomial time.
\end{theorem}}

As we have already explained in Section~\ref{sec:intro-trees-asymmetric}, Theorem~\ref{thm:main-trees} actually extends 
Theorem~\ref{thm:FJ-dichotomy} of Faben and Jerrum~\cite[Theorem~3.8]{FJ13} to all prime moduli. If $H$ is an 
asymmetric 
tree, then $H^{*p}=H$, 
as $H$ has no non-trivial automorphisms. We have the following corollary.

\begin{corollary}
 Let $p$ be a prime and $H$ be an asymmetric tree. If $H$ has more than one vertex then \phcol{} is $\numpp$-complete, 
otherwise \phcol{} is computable in polynomial time.
\end{corollary}

To prove Theorem~\ref{thm:main-trees} we will use the pinning technique developed in Chapter~\ref{chpt:pinning}. 
When $H$ is asymmetric its automorphism group only contains the trivial automorphism, so for any prime $p$, $H$ and $p$ 
are orbit compatible. Thus we can use Theorem~\ref{thm:partlabcol} and reduce 
\partlabphcol{} to \phcol{}. In order to show hardness for \phcol{} it suffices to show hardness for \partlabphcol{}.
The starting point of our reduction is~\gpart: the problem of computing the partition function 
of a two-spin system on a multigraph modulo a prime. The partition function of a multigraph $G$ is given by 
\[\gspin(G)=\!\!\!\!\sum_{\sigma: V(G)\rightarrow\{0,1\}}\!\!\!\!\gamma^{c(\sigma)},\]
where $c(\sigma)$ denotes the number of edges $(u,v)$ (including self-loops) with $\sigma(u)=\sigma(v)=1$.
An immediate corollary of a result of Guo et al.~\cite{GHLX11} shows that \gpart{} is $\numpp$-hard. We then 
show that for all non-trivial graphs $H$, \gpart{} reduces to \partlabphcol{}.

The reduction from \gpart{} to \partlabphcol{} (Theorem~\ref{p:thm:hardness-gadget}) works as follows. Given a 
multigraph~$G$ as input of \gpart{} 
we construct a partially labelled simple graph $J$, input for \partlabphcol{}. To construct $J$ we replace the vertices 
and edges of $G$ with partially labelled graphs, which we call ``gadgets''.
In~$J$, the gadget corresponding to the vertex~$v$ of~$G$ has a vertex~$y^v$. We also choose an appropriate vertex~$i$ 
in~$H$.  Any homomorphism~$\sigma$ from $J$ to the target graph~$H$ defines a set
$I(\sigma) = \{v\in V(G)\mid \sigma(y^v)=i\}$. The configuration of the gadgets ensures that  
a set $I \subseteq V(G)$ has an appropriate number of homomorphisms
$\sigma$ with $I(\sigma)=I$. Each two-spin configuration~$\tau$ of $G$ has weight $\gamma^{c(\tau)}$, where $c(\tau)$ 
can be determined by the set~$I'(\tau)$ of vertices that are mapped to ``1'' by $\tau$. That weight is equivalent 
to the number of homomorphisms~$\sigma$ with $I(\sigma)=I'(\tau)$. Thus, the two-spin partition function of~$G$ is 
equivalent to $|\Homs{J}{H}|$, modulo~$p$.

We call the gadgets that we use $(\gamma,p)$-gadgets (Definition~\ref{p:defn:hardness-gadget}). A \ggadget{} is chosen 
according to the structure and 
properties of $H$. If for an asymmetric graph $H$ we can find a \ggadget, then we can reduce \gpart{} to \phcol{}. The 
reduction from \gpart{} to \phcol{} can be seen as assigning colours to both the vertices and the edges 
of~$G$, where each ``colour'' is a vertex of~$H$. Each \ggadget{} has three main parts. One part of the gadget controls 
which colours can be assigned to each vertex, where each colour corresponds to a spin.
The second part controls which colours can be assigned to each edge, where the edge--colours determine the 
interractions among the vertex--colours. Finally, a third part determines how many homomorphisms there are from $G$ 
to~$H$, given the choice of colours for the vertices and edges.

Since we are working with trees, we are able to use gadgets with very simple structure: our gadgets are essentially 
paths and we exploit the limited structure of asymmetric trees. We show that every non-trivial asymmetric tree~$H$ 
contains three consecutive vertices of appropriate degrees (Lemma~\ref{lem:consecutive-degrees}). These three 
consecutive vertices can then be used to obtain a $(3,p)$-gadget for $H$ (Lemmas~\ref{lem:tree-23-gadget} 
and~\ref{lem:tree-22-gadget}).

Finally, in this chapter, we discuss the complexity of \khcol{} when $k$ is a composite. The polynomial-time 
algorithm of Faben and Jerrum works for \khcol{} only when $k$ is a prime. By the Chinese remainder 
theorem (Theorem~\ref{thm:chinese-remainder}), if $p_1^{r_1}p_2^{r_2}\dots 
p_m^{r_m}=k$ is the prime factorisation of $k$, then for each $j\in[m]$, the complexity of \khcol{} is equivalent to 
the complexity of $\#_{p_j^{r_j}}\prb{HomsTo}H$. For a prime $p$ and an integer $r$, if \phcol{} is 
hard, then $\#_{p^r}\prb{HomsTo}H$ is also hard. The inverse is not always true. In modular counting problems there 
have 
been cases in the literature (Guo et al.~\cite{GHLX11}) where the complexity of a modular counting problem $\#_{p}A$ is 
equivalent to the complexity of $\#_{p^r}A$. We will illustrate 
that this is not the case with counting graph homomorphisms, as we identify a graph~$P_4$ where $\#_2\prb{HomsTo}P_4$ 
is easy while $\#_4\prb{HomsTo}P_4$ is hard.



\subsubsection{Organisation}

In Section~\ref{sec:spins-for-trees} we formally define \gpart{} and show that \gpart{} is hard for some value of 
its parameters. In Section~\ref{sec:p-gadgets} we define \ggadget s and show that when~$H$ has a \ggadget{} then 
\phcol{} is $\numpp$-complete. In Section~\ref{sec:trees-dichotomy} we show that every asymmetric tree~$H$ has a 
$(3,p)$-gadget and we also prove Theorem~\ref{thm:main-trees}. Finally in Section~\ref{sec:composites} we show that
$\#_4\prb{HomsTo}P_4$ is $\parp$-hard but $\#_2\prb{HomsTo}P_4$ is computable in polynomial time.




\subsection{Gadgets}
\label{sec:p-gadgets}

Let $H$ be a target graph for \phcol{}. To define the gadgets that we use, we need choose a set 
$\Oy\subseteq V(H)$ and a vertex $i\in\Oy$.  Given a multigraph~$G$ whose two-spin partition function we wish to compute
modulo~$p$, we will construct a partially
$H$-labelled graph~$J$ and consider homomorphisms from $J$ to~$H$.
$J$~will contain a copy of $V(G)$ and we will be interested in
homomorphisms that map every vertex in this copy to~$\Oy$.  Vertices
mapped to~$i$ will be vertices mapped to ``1'' in the two-spin configuration under consideration;
vertices mapped to $\Oy-i$ will be the vertices mapped to ``0''.

\begin{definition}
\label{p:defn:hardness-gadget}
A \emph{$(\gamma,p)$-gadget} $(i,s,(J_1,y),(J_2,z),(J_3,y,z))$ consists
of vertices $i$ and $s$ of $H$ together with three partially labelled
graphs with distinguished vertices $(J_1,y)$, $(J_2,z)$ and $(J_3,y,z)$, where $y$ and $z$ are distinct, satisfying the 
properties explained bellow. Let

\begin{align*}
N_1(v) &= |\Homs{(J_1,y)}{(H,v)}|\\
N_2(v) &= |\Homs{(J_2,z)}{(H,v)}|\\
N_3(u,v) &=|\Homs{(J_3,y,z)}{(H,u,v)}|\\
\Oy &= \{ u \in V(H) \mid N_1(v)\equiv1\pmod p\}\\
\Oz &= \{ u \in V(H) \mid N_2(v)\not\equiv0\pmod p\}\,.
\end{align*}

The properties that we require are:
\begin{enumerate}
 \item $i\in\Oy$, $|\Oy|\equiv 2\pmod p$ and, for each $u\notin\Oy$, $N_1(u)\equiv 0 \pmod p$.
 \item $\sum_{b\in\Oz}N_2(b)\equiv\gamma\kappa$ and $N_2(s)\equiv\kappa \pmod p$, where $\kappa\not\equiv0\pmod p$. 
 \item For each $o\in \Oy-i$ and each $x\in \Oz-s$, $\Sox\equiv0\pmod p$.\
\item And for each $o\in \Oy-i$ and each $x\in \Oz-s$ the following hold:
\begin{enumerate}
       \item $\Sis\equiv1\pmod p$
       \item $\Sos\equiv1\pmod p$
       \item $\Six\equiv1\pmod p$.
      \end{enumerate}
\end{enumerate}
\end{definition}

% Since $H$ is non-directed, and the definition of \ggadget is symmetric in the sense of $y$ and $z$ we have the 
% following observation that will be useful in a later chapter.
% 
% \marge{this observation will be needed after I run my program}
% \begin{observation}\label{obs:gadget-symmetry}
%  If $H$ has a \ggadget, then $H$ has an \lggadget.
% \end{observation}

Now we can show that for every graph~$H$ and every prime~$p$, such that $H$ and $p$ are orbit compatible and~$H$ has a 
\ggadget{}, the problem of counting (modulo $p$) graph homomorphisms to $H$ is $\numpp$-hard. We will use the 
following 
notation to build partially labelled graphs containing many copies of some subgraph.  For any ``tag''~$T$ (which
we will treat just as an arbitrary string) and any partially labelled
graph~$J$, denote by $J^T$ a copy of~$J$ with every vertex $v\in
V(G(J))$ renamed~$v^T\!$.

\begin{figure}
\begin{center}
%\begin{tikzpicture}[scale=.35,node distance = 1.5cm]
%\tikzstyle{vertex}=[fill=black, draw=black, circle, inner sep=1.5pt]
%\tikzstyle{blob1}=[cloud, cloud puffs=21, draw, minimum width=.1cm,
%                   minimum height=.1cm, aspect=2.1]
%\tikzstyle{blob2}=[cloud, cloud puffs=7, draw, minimum width=.1cm,
%                   minimum height=.1cm, aspect=3.1]
%
%    \begin{scope}[shift={(-32,0)}]
%        \node[vertex] (u) at (0,   1.4) [label=180:{$u$}] {};
%        \node             at (2.2,-4.8) {$g$};
%        \node             at (-2.2,-4.8) {$f$};
%        \node		  at (-1.4,3.5) {$e$};
%        \node[vertex] (v) at (0,  -11 ) [label=180:{$v$}] {};
% 
%        \draw (0,2.8) circle [x radius=1cm, y radius=1.4cm];
%        \draw (0,-4.8) circle [x radius=1.7cm, y radius=6.2cm];
% 
%        \node at (0,-14) {$G$};
%    \end{scope}
%
%    \begin{scope}[shift={(-19,0)}]
%
%  \draw (-2.3, -1.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=55];
%  \node at (-2.3,-1.8) {$J_3^{f,u}$};    
%  
%  \draw (2.3,-1.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=-55];
%  \node at (2.3,-1.8) {$J_3^{g,u}$};    
%  
%  \draw (-2.3, -7.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=-55];
%  \node at (-2.3,-7.8) {$J_3^{f,v}$};
%  
%  \draw (2.3,-7.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=55];
%  \node at (2.3,-7.8) {$J_3^{g,v}$};    
% 
%  \draw (0,4.8) circle [x radius=1.1cm, y radius=4.6cm];
%  \node at (0,4.8) {$J_3^{e,u}$};
%
%        \node[vertex] (u) at (0,  1.4 ) {};
%        \node at(1.6,2.1) {$y^u$};
%        
%        \node[vertex] (v) at (0,  -11 ) {};
%        \node at (1.6,-11.7) {$y^v$};
%        
%        \node[vertex]  (f) at (-4.5,-4.8)  {};
%        \node at (-2.5,-4.6) {$z^f$};
%        
%        \node[vertex]  (g) at (4.5,-4.8) {};
%        \node at (2.5,-4.8) {$z^g$};
%        
%        \node[vertex] (e) at (0, 8.4) {};
%        \node at (-1.4,8.7) {$z^e$};       
%
%    \node[blob2] at (1.8,8.4) {$\quad\quad$};
%    \node        at (1.8,8.4) {$J_2^e$};  
%    \node[blob2] at (6.3,-4.8) {$\quad\quad$};
%    \node        at (6.3,-4.8) {$J_2^g$};
%    \node[blob2] at (-6.3,-4.8) {$\quad\quad$};
%    \node        at (-6.2,-4.8) {$J_2^f$};
%          
%    \node         at (0,-14 ) {$K$};
%    \end{scope}
% 
% 
%    \draw (-2.3, -1.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=55];
%  \node at (-2.3,-1.8) {$J_3^{f,u}$};    
%  
%  \draw (2.3,-1.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=-55];
%  \node at (2.3,-1.8) {$J_3^{g,u}$};    
%  
%  \draw (-2.3, -7.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=-55];
%  \node at (-2.3,-7.8) {$J_3^{f,v}$};
%  
%  \draw (2.3,-7.8) circle [x radius=4.6cm, y radius=1.1cm, rotate=55];
%  \node at (2.3,-7.8) {$J_3^{g,v}$};    
% 
%  \draw (0,4.8) circle [x radius=1.1cm, y radius=4.6cm];
%  \node at (0,4.8) {$J_3^{e,u}$};
%
%        \node[vertex] (u) at (0,  1.4 ) {};
%        \node at(1.6,2.1) {$y^u$};
%        
%        \node[vertex] (v) at (0,  -11 ) {};
%        \node at (1.6,-11.7) {$y^v$};
%        
%        \node[vertex]  (f) at (-4.5,-4.8)  {};
%        \node at (-2.5,-4.6) {$z^f$};
%        
%        \node[vertex]  (g) at (4.5,-4.8) {};
%        \node at (2.5,-4.8) {$z^g$};
%        
%        \node[vertex] (e) at (0, 8.4) {};
%        \node at (-1.4,8.7) {$z^e$};       
%
%    \node[blob2] at (1.8,8.4) {$\quad\quad$};
%    \node        at (1.8,8.4) {$J_2^e$};  
%    \node[blob2] at (6.3,-4.8) {$\quad\quad$};
%    \node        at (6.3,-4.8) {$J_2^g$};
%    \node[blob2] at (-6.3,-4.8) {$\quad\quad$};
%    \node        at (-6.2,-4.8) {$J_2^f$};
%  
%    \node[blob1] at (-2.5,1.4) {$\quad\quad\quad$};
%    \node at (-2.5,1.4) {$J_1^u$};
%    
%    \node[blob1] at (-2.5,-11) {$\quad\quad\quad$};
%    \node at (-2.5,-11) {$J_1^v$};
%     
%    \node at (0,-14) {$J$};
%\end{tikzpicture}
\includegraphics[]{TikZ/hardness_gadget.pdf}
\end{center}
\caption{The construction of the partially labelled graphs $K$ and~$J$
  from an example graph~$G$, as in the proof of
  Theorem~\ref{p:thm:hardness-gadget}. Here graph $G$ consists of two vertices $u,v$ connected with the parallel edges 
$f,g$ and the self-loop~$e$ on vertex~$u$.}
\label{fig:hardness-gadget}
\end{figure}

\begin{theorem}\label{p:thm:hardness-gadget}
 Let $p$ be a prime and let $H$ be a graph such that $H$ and $p$ are orbit compatible. If~$H$ has 
a \ggadget{}, with $\gamma\in\zp$ and
$\gamma^2\not\equiv1\pmod p$, then \phcol{} is $\numpp$-hard.
\end{theorem}
\begin{proof}
    Let $(i,s,(J_1,y),(J_2,z),(J_3,y,z))$ be the \ggadget{}
    for~$H$ and recall the sets $\Oy$ and $\Oz$ from Definition~\ref{p:defn:hardness-gadget}.
    We will reduce \gpart{} to \partlabphcol{}. The rest of the proof follows from 
Corollary~\ref{cor:spin-unary} and Theorem~\ref{thm:partlabcol}. Given 
an input multigraph~$G$ to
    \gpart{}, we construct an appropriate partially $H$-labelled
   graph~$J$ and show that $|\Homs{J}{H}|\equiv\kappa^{|E(G)|}\gspin(G)\pmod p$, where $\kappa$ comes from property~2 
of Definition~\ref{p:defn:hardness-gadget}.
    
    We construct~$J$ in two stages (see Figure~\ref{fig:hardness-gadget}).  Take the union of disjoint
    copies~$J_3^{e,v}$ of~$J_3$ for every edge $e\in G$ and each
    endpoint~$v$ of~$e$.  If $e$ is a self-loop of $G$, then $J$ will contain a single copy of 
$J_3^{e,v}$. For each edge $e=(u,v)\in G$, identify the
    vertices $z^{e,u}$ and~$z^{e,v}\!$ --- if $e=(v,v)$ ignore this step. For each vertex $v\in G$,
    identify all the vertices~$y^{e,v}$ such that $e$~has $v$~as an
    endpoint. For every edge $e\in G$ add a disjoint copy~$J_2^e$ of~$J_2$ and identify $z^e$ with the 
    already-identified vertices $z^{e,v}\!$.  
    Call this graph~$K$. 
    
    We show that $K$ is a simple graph and not a multigraph. By construction, every edge~$e$ 
with distinct endpoints in $G$ corresponds to the graphs $J_3^{e,v}$, $J_3^{e,u}$ and $J_2^e$ in $K$, where $z^{e,v}$, 
$z^{e,u}$ and $z^e$ are identified. Every pair of parallel edges~$e$ and~$f$ forms a $2$-cycle in $G$. In $K$, this 
corresponds to a cycle of length $4\dist_{J_3}(y,z)$. Since $J_3$ is a simple graph with no parallel edges and 
$\dist_{J_3}(y,z)>0$, there are no 1-cycles or 2-cycles in $K$ that correspond to $e$ and $f$ in $G$. So there are no 
self-loops or parallel edges in $K$ that correspond to $e$ and $f$. Let $e=(v,v)$ be a self-loop in $G$. By 
construction, this will correspond to the graphs $J_3^{e,v}$ and $J_2^e$ as subgraphs of $K$, where $z^{e,v}$ is 
identified with $z^e$. As both $J_2$ and $J_3$ are simple graphs, they do not introduce any self-loops or parallel 
edges 
in $K$. Hence $K$ is a simple graph with no self-loops or parallel edges.
    
    To make~$J$, take~$K$ and add a disjoint copy~$J_1^v$ of~$J_1$ for every vertex $v\in G$ and identify $y^v$ with 
the already-identified vertices $y^{e,v}$. Since $K$ and $J_1$ are simple graphs, by construction $J$ is also a simple 
graph.

    We now proceed to show that $|\Homs{J}{H}|\equiv \kappa^{|E(G)|}\gspin(G)\pmod p$.

    For a homomorphism $\sigma\in\Homs{K}{H}$, let $\eqclass{\sigma}$
    be the set of extensions of $\sigma$ to homomorphisms from $J$
    to~$H$, i.e.,

    \begin{equation*}
        \eqclass{\sigma} =
            \{\sigma'\in\Homs{J}{H}\mid
                  \sigma(v) = \sigma'(v) \text{ for all } v\in V(G(K))\}\,.
    \end{equation*}

    Every homomorphism from $J$ to~$H$ is the extension of a unique
    homomorphism from $K$ to~$H$, so we have

    \begin{equation}
    \label{p:eq:sum-eq-classes}
        |\Homs{J}{H}| \ \ \ = \!\!\!\!\!\!
            \sum_{\sigma\in\Homs{K}{H}} \!\!\!\!\!\! |\eqclass{\sigma}|\,.
    \end{equation}

    From the structure of~$J$, we have

    \begin{equation*}
        |\eqclass{\sigma}|
            = \prod_{v\in V(G)} \big|\Homs{(J_1,y)}{(H,\sigma(y^v)}\big|.
    \end{equation*}

    By Definition~\ref{p:defn:hardness-gadget} (property~1),
    $|\Homs{(J_1,y)}{(H,a)}|\equiv 1\pmod p$ if $a\in\Oy$, otherwise $|\Homs{(J_1,y)}{(H,a)}|\equiv0\pmod p$. 
Therefore, 
$|\eqclass{\sigma}|$~is non-zero (modulo~$p$) if and only if $\sigma$~maps every vertex~$y^v$ into~$\Oy$; call such a 
homomorphism 
``legitimate'' with respect to $J_1$.  We can rewrite~\eqref{p:eq:sum-eq-classes} as

    \begin{equation}
    \label{eq:legitimate}
        |\Homs{J}{H}| \equiv |\{\sigma\in\Homs{K}{H}\mid
                               \sigma\text{ is legitimate}\}| \pmod p\,,
    \end{equation}

    and, from this point, we restrict our attention to legitimate
    homomorphisms.

    Given a legitimate homomorphism $\sigma\in\Homs{K}{H}$, let
    $\sigma|_Y$~be the restriction of~$\sigma$ to the domain
    $\{y^v\mid v\in V(G)\}$.  Write $\sigma \sim_Y \sigma'$ if
    $\sigma|_Y = \sigma'|_Y$ and write $\eqclass{\sigma}_Y$ for the
    $\sim_Y$-equivalence class of~$\sigma$.  The
    classes~$\eqclass{\sigma}_Y$ partition the set of legitimate
    homomorphisms from $K$ to~$H$.  
    
   Recall from Definition~\ref{p:defn:hardness-gadget} that $N_2(v) 
= |\Homs{(J_2,z)}{(H,v)}|$ and recall that $N_3(u,v) =|\Homs{(J_3,y,z)}{(H,u,v)}|$. 
Let
\[n(u,u') = \sum_{b\in \Oz}N_3(u,b)N_3(u',b)N_2(b)\]
and let
\[n'(u)=\sum_{b\in \Oz}N_3(u,b)N_2(b).\]
    From the structure of $K$ we have,

    \begin{equation*}
        \big|\eqclass{\sigma}_Y\big| \ 
            = \left(\prod_{\substack{(u,v)\in E(G),\\ u\neq v}}\!\!\!\!\!\! n(\sigma(u), 
\sigma(v))\right)\left(\prod_{(u,u)\in E(G)}\!\!\!\!\!\! n'(\sigma(u))\right)\,.
    \end{equation*}

  We will claim that for $u\in\Oy$ and for $o\in\Oy\setminus\{i\}$ the following hold:
  \begin{itemize}
   \item $n(i,i)\equiv \gamma\kappa\pmod p$,
   \item $n'(i)\equiv \gamma\kappa \pmod p$,
   \item $n(o,u)\equiv n(u,o)\equiv \kappa \pmod p$ and
   \item $n'(o)\equiv \kappa \pmod p$.
  \end{itemize}
  To prove the claim, recall from Definition~\ref{p:defn:hardness-gadget} that $\sum_{b\in 
\Oz}N_2(b)=\gamma\kappa$ (property~2) and that for $b\in\Oz$, $N_3(i,b)\equiv1\pmod p$ (property~4). Therefore, both
$n(i,i)\equiv \sum_{b\in \Oz}N_2(b)\equiv\gamma\kappa\pmod p$ and $n'(i)\equiv\sum_{b\in 
\Oz}N_2(b)\equiv\gamma\kappa\pmod p$. For $o\in\Oy\setminus\{i\}$, 
$\Sos\equiv1\pmod p$ and for $x\in\Oz\setminus\{s\}$, $\Sox\equiv 0 \pmod p$ ---this comes from properties~3 and~4 of 
Definition~\ref{p:defn:hardness-gadget}. So, when at least one of $u$ or $u'$ is not $i$, the only non-zero 
term in the sum defining $n(u,u')$ is $N_3(u,s)N_3(u',s)N_2(s)$. As $N_3(u,s)\equiv N_3(u',s)\equiv1\pmod p$, from 
property~2 we have $n(u,u')\equiv N_2(s)\equiv \kappa\pmod p$. Similarly, $n'(o)\equiv\kappa\pmod p$. This concludes 
the proof of the claim.

For a homomorphism $\sigma:V(K)\rightarrow V(H)$,  let $c'(\sigma)$ be the number of edges 
$(v,v')\in E(G)$, where $v$ and $v'$ are not necessarily distinct, with $\sigma(v)=\sigma(v')=i$.  From the above 
claim, we 
have, 
\begin{equation}\label{p:eq:g-relations}
|\eqclass{\sigma}_Y|\equiv\kappa^{|E(G)|}\gamma^{c'(\sigma)}\,. 
\end{equation}

    Choose representatives $\sigma_1, \dots, \sigma_k$, one from each
    $\sim_Y$-equivalence class.  From (\ref{eq:legitimate}) and the fact that the classes~$\eqclass{\sigma}_Y$ 
partition the legitimate homomorphisms from $K$ to~$H$, we have,
\[|\Homs{J}{H}|\equiv\ \sum_{j=1}^k \big|\eqclass{\sigma_j}_Y\big|\pmod p.\]
From~\eqref{p:eq:g-relations}, the definition of $\sim_Y$-equivalence and the definition of a legitimate homomorphism 
we have,
 \begin{equation}\label{eq:homs-to-edges}
|\Homs{J}{H}|\equiv\kappa^{|E(G)|}\!\!\!\!\!\! \sum_{\sigma: V(G)\rightarrow\Oy}\!\!\!\!\!\! \gamma^{c'(\sigma)}\pmod 
p. 
 \end{equation}

 Given $\sigma,\sigma':V(G)\rightarrow\Oy$, we write $\sigma\sim_i\sigma'$ if, for all $v\in V(G)$, 
$\sigma(v)=i \Leftrightarrow\sigma'(v)=i$. Let $\eqclass{\sigma}_i$ denote the $\sim_i$ equivalence-class of $\sigma$. 
The classes 
$\eqclass{\sigma}_i$ partition the set of functions from $V(G)$ to $\Oy$ and, by definition, for $\sigma\sim_i\sigma'$, 
$c'(\sigma)=c'(\sigma')$.

Choose representatives $\sigma_1, \dots 
\sigma_m$, one from each $\sim_i$ equivalence class. From~\eqref{eq:homs-to-edges} we have
\begin{equation}
 \label{eq:classes-of-mappings}
 |\Homs{J}{H}|\equiv \kappa^{|E(G)|}\sum_{j=1}^m |\eqclass{\sigma}_i|\gamma^{c'(\sigma_j)} \pmod p.
\end{equation}


For $\sigma:V(G)\rightarrow\Oy$, let $\ell(\sigma)$ denote the number of vertices~$v\in V(G)$ with 
$\sigma(v)\in\Oy\setminus\{i\}$. $|\eqclass{\sigma}_i|\equiv (|\Oy|-1)^{\ell(\sigma)}\pmod p$. Recall from property~1 of
Definition~\ref{p:defn:hardness-gadget} that $|\Oy|\equiv 2 \pmod p$, so $|\eqclass{\sigma}_i|\equiv1\pmod p$. For each 
$\sigma:V(G)\rightarrow\Oy$, there is exactly one configuration $\sigma':V(G)\rightarrow\{0,1\}$, such that for 
each $v\in V(G)$, $\sigma(v)=i\Leftrightarrow\sigma'(v)=1$. Therefore there is a bijection between the 
equivalence 
classes $\eqclass{\sigma}_i$ and distinct mappings $\sigma':V(G)\rightarrow\{0,1\}$. 
Using this bijection and~\eqref{eq:classes-of-mappings} we have,
\begin{equation*}
|\Homs{J}{H}|\equiv\kappa^{|E(G)|}\!\!\!\!\!\!\sum_{\sigma: V(G)\rightarrow\{0,1\}}\!\!\!\!\!\!\gamma^{c(\sigma)} \pmod 
p.
\end{equation*}

Recall the definition of the partition function $\gspin(G)=\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\gamma^{c(\sigma)}$. We have
\begin{equation*}
|\Homs{J}{H}|\equiv\kappa^{|E(G)|}\gspin(G) \pmod p. \qedhere
\end{equation*}
\end{proof}

In this chapter we are interested in asymmetric trees. Recall from Section~\ref{sec:pinning-prelim}, that if a graph 
$H$ is asymmetric, its automorphism group contains only the trivial automorphism. Hence, for any prime~$p$, $H$ has no 
automorphism of 
order~$p$ and for every $r\in\posints$ and for every $r$-tuple $\ybar\in(V(H))^r$, $|\Orb_H(\ybar)|\equiv 1\pmod p$. 
Recall Definition~\ref{defn:orbit} of orbit compatibility. We have the following observation.

\begin{observation}\label{obs:asymmetric-compatible}
 Let $p$ be a prime and let $H$ be an asymmetric graph. $H$ and $p$ are orbit compatible.
\end{observation}

To show hardness for \phcol{}, when $H$ is an asymmetric tree we can now use the following.

\begin{corollary}\label{cor:asymmetric-pinning}
Let $p$ be a prime and let $H$ be an asymmetric graph. If~$H$ has a \ggadget{}, with $\gamma\in\zp$ and 
$\gamma^2\not\equiv1\pmod p$, then 
\phcol{} is $\numpp$-hard.
\end{corollary}
\begin{proof}
 This is immediate from Theorem~\ref{p:thm:hardness-gadget} and Observation~\ref{obs:asymmetric-compatible}.
\end{proof}

\subsection{A dichotomy for asymmetric trees}
\label{sec:trees-dichotomy}

In this section we will show that every asymmetric tree has a $(\gamma,p)$-gadget, whith $\gamma^2\not\equiv1\pmod p$ 
for all primes $p$. Our first lemma shows that every asymmetric tree has three adjacent vertices of appropriate degree. 
We will use this to construct $(\gamma,p)$-gadgets. 

The following lemma extends \cite[Lemma~5.3]{FJ13} of Faben and Jerrum by following a similar proof approach.

\begin{figure}[t]
	\begin{center}
%		\begin{tikzpicture}[scale=.85]
%		\tikzstyle{vertex}=[fill=black, draw=black, circle]
%		\tikzstyle{grey}=[fill=black!30!white, draw=black!30!white, circle]
%		
%		\node[vertex] at (0,0) (0) [label=135:$v_0$] {} ;
%		\node[vertex] at (2,0) (1) [label=90:{$v_1=s$}] {} ;
%		\node[vertex] at (4,0) (2) [label=45:{$v_2=i$}] {} ;
%		
%		\node[vertex] at (3,1) (a) [label=90:$u_2$] {} ;
%		
%		\node[grey] at (1,-1) (b) [label=-135:$u_1$] {} ;
%		\node[grey] at (3,-1) (c) [label=-90:$u_3$] {};
%		\node[grey] at (2,2) (d) [label=90:$u_2'$] {} ;
%		\node[grey] at (4,2) (e) [label=90:$u_2''$] {} ;
%		
%		\node at (7.5,.5) {$P$};
%		
%		\draw (0)--(1)--(2)--(a);
%		\draw[black!30!white] (1)--(b);
%		\draw[black!30!white] (d)--(a)--(e);
%		\draw[black!30!white] (2)--(c);
%		\draw[decorate, decoration=snake] (2)--(7,0);
%		\end{tikzpicture}
\includegraphics[]{TikZ/consecutive_degrees.pdf}
		\caption{An illustration of the proof of Lemma~\ref{lem:consecutive-degrees}. The vertices that appear with grey are 
			the vertices that their existence is contradicted in the proof. The rest of the longest path of the graph 
			$P$ is indicated with a wavy line.}
		\label{fig:consecutive-degrees}
	\end{center}
\end{figure}

\begin{lemma}\label{lem:consecutive-degrees}
	Every asymmetric tree~$H$ with more than one vertex has a vertex~$s$ of degree~2 that is adjacent to a leaf. 
	Furtherore, $s$~is adjacent to a vertex $i$, where $\deg_H(i)\in\{2,3\}$.
\end{lemma}
\begin{proof}
	Let $P=v_0\dots v_k$ be a longest path in~$H$. Since stars have non-trivial automorphisms, $H$ cannot be a star and 
	$k\geq 3$. Let $v_1=s$ and 
	$v_2=i$. For an illustration of the proof that follows see Figure~\ref{fig:consecutive-degrees}.
	
	From the maximality of the length of~$P$, $v_0$ must be a leaf vertex. Now assume for 
	contradiction that $u_1\in\Gamma_H(v_1)\setminus\{v_0,v_2\}$. If $u_1$ is not a leaf, then the maximality of the 
	length of~$P$ is contradicted. If $u_1$ is a leaf, then $H$ has a non-trivial 
	automorphism~$\tau$, with $\tau(u_1)=v_0$ and $\tau(v_0)=u_1$. Hence $u_1$ cannot exist and $v_1$ has degree~2.
	
	We claim that every neighbour of $v_2$ that is not in~$P$ must be a leaf. Let 
	$u_2\in\Gamma_H(v_2)\setminus\{v_1,v_3\}$. Assume for contradiction that $u_2$ is not a leaf. By the maximality of the 
	length of $P$, any vertex $u'_2\in\Gamma_H(u_2)\setminus\{v_2\}$ must be a leaf. First assume that there are at least 
	two vertices $u'_2,u''_2\in\Gamma_H(u_2)\setminus\{v_2\}$. Since both of them can only be leaves, $H$ has a 
	non-trivial automorphism~$\tau$ with $\tau(u'_2)=u''_2$ and $\tau(u''_2)=u'_2$. Hence $u_2$ can only have one 
	neighbour~$u'_2$ that is a leaf. But now $H$ has a non-trivial automorphism~$\tau$ with 
	$\tau(v_0)=u'_2$, $\tau(v_1)=u_2$, $\tau(u'_2)=v_0$ and $\tau(u_2)=v_1$, so the claim follows.
	
	Finally we show that $v_2$ can only have one neighbour $u_2\in\Gamma_H(v_2)\setminus\{v_1,v_3\}$. If there was 
	$u_3\neq u_2$ with $u_2\in\Gamma_H(v_2)\setminus\{v_1,v_3\}$ then $H$ would have a non-trivial automorphism~$\tau$ with 
	$\tau(u_2)=u_3$ and $\tau(u_3)=u_2$.
\end{proof}

Now we will show that if $H$ has a degree~2 vertex adjacent to a vertex of degree~$\gamma$, then $H$ has a 
$(\gamma,p)$-gadget.

\begin{figure}[ht]
	\begin{center}
%		\begin{tikzpicture}[scale=1.2,node distance = 1.5cm]
%		\tikzstyle{dot}   =[fill=black, draw=black, circle, inner sep=0.15mm]
%		\tikzstyle{vertex}=[fill=black, draw=black, circle, inner sep=2pt]
%		\tikzstyle{dist}  =[fill=white, draw=black, circle, inner sep=2pt]
%		\tikzstyle{pinned}=[fill=white, draw=black, minimum size=9mm, circle,inner sep=0pt]
%		
%		\begin{scope}[shift={(-3,0)}]
%		\node[vertex] at (0,0) (0) [label=135:$o$] {} ;
%		\node[vertex] at (1,0) (1) [label=90:{$s$}] {} ;
%		\node[vertex] at (2,0) (2) [label=45:{$i$}] {} ;
%		
%		\node[vertex] at (1,1) (a)  {} ;
%		
%		\draw[dashed] (4.5,0) ellipse  (1.5cm and 1cm);
%		\draw (0)--(1)--(2)--(a);
%		\draw (2)--(3,0);
%		\draw[dashed] (3,0)--(3.4,0);
%		
%		\node at (3,-1) {$H$};
%		\end{scope}
%		
%		\begin{scope}[shift={(4,1.75)}]
%		\node at (0,0) {$J_1$:};
%		
%		\node[pinned] (p1) at (1,0) [label=-90:$u$]{$\strut s$};
%		\node[dist]   (y)  at (2,0) [label=-90:$y$] {};
%		
%		\draw (p1) -- (y);
%		\end{scope}
%		
%		\begin{scope}[shift={(4,0.5)}]
%		\node at (0,0) {$J_2$:};
%		
%		\node[pinned] (p3) at (1,0) [label=-90:$w$]{$\strut i$};
%		\node[dist]   (z)  at (2,0) [label=-90:$z$] {};
%		
%		\draw (p3) -- (z);
%		\end{scope}
%		
%		\begin{scope}[shift={(4,-0.75)}]
%		\node at (0,0) {$J_3$:};
%		
%		\node[dist] (yy) at (1,0) [label=-90:$y$] {};
%		\node[dist] (zz) at (2,0) [label=-90:$z$] {};
%		
%		\draw (yy) -- (zz);
%		\end{scope}
%		
%		\end{tikzpicture}
	\includegraphics[]{TikZ/tree_23_gadget.pdf}
	\end{center}
	\caption{A $(\gamma,p)$-gadget for the asymmetric tree~$H$ as in the proof of Lemma~\ref{lem:tree-23-gadget}, where 
		$\gamma=3$. In the figure we assumed that $o$ is a leaf, but it is not needed for the proof of 
		Lemma~\ref{lem:tree-23-gadget}. Normal vertices appear as black dots, distinguished vertices as small white circles. 
		Pinned vertices appear as large white circles where the label inside the vertex indicates what the vertex is pinned to. 
		The ellipse denotes the rest of the 
		graph $H$.}
	\label{fig:tree-23-gadget}
\end{figure}

\begin{lemma}\label{lem:tree-23-gadget}
	Let $p$ be a prime and let $H$ be a tree. If $H$ has a vertex~$s$ of degree~2 that is adjacent to a vertex 
	$i$ of degree~$\gamma$, then $H$ has a $(\gamma,p)$-gadget.
\end{lemma}
\begin{proof}
	We define the $(\gamma,p)$-gadget of $H$ to be $(i,s,(J_1,y),(J_2,z),(J_3,y,z))$, where $J_1,J_2,J_3$ are defined as 
	follows (See Figure~\ref{fig:tree-23-gadget}):
	\begin{itemize}
		\item $J_1$ is the edge $(u,y)$, with $\tau(J_1)=\{u\mapsto s\}$.
		\item $J_2$ is the edge $(w,z)$, with $\tau(J_2)=\{w\mapsto i\}$.
		\item $J_3$ is the edge $(y,z)$.
	\end{itemize}
	
	It remains to show that properties 1-4 of Definition~\ref{p:defn:hardness-gadget} hold.
	
	$G(J_1)$ is just an edge so, for each $v\in\Gamma_H(s)$, $N_1(v)=1$ and, for every $v'\notin\Gamma_H(v_1)$, it holds 
	that $N_1(u)=0$. Therefore $\Oy=\Gamma_H(s)$. Clearly $i\in\Oy$ and $|\Oy|=\deg_H(s)=2$. Hence 
	property~1 of Definition~\ref{p:defn:hardness-gadget} holds. 
	
	Similarly, as $J_2$ is a simple edge, $\Oz=\Gamma_H(i)$ and for any $b\in\Oz$, $N_2(b)=1\not\equiv0 \pmod p$. 
	Therefore $\sum_{b\in\Oz}N_2(b)=\deg_H(i)=\gamma$ and $N_2(s)=1$, hence property~2 of 
	Definition~\ref{p:defn:hardness-gadget} 
	holds, with $\kappa=1$.
	
	$G(J_3)$ is a simple edge, so for $a,b\in V(G)$, $N_3(a,b)=1$ if and only if $a$ is adjacent to $b$, otherwise 
	$N_3(a,b)=0$. Let $o\in\Oy-i$ and let $x\in\Oz-s$. Since there is a path $P=osix$ in $H$, $o$ is not adjacent to $x$, 
	otherwise there would be a cycle in $H$. Thus $\Sox=0$ and property~3 of 
	Definition~\ref{p:defn:hardness-gadget} holds. Since $\Oy=\Gamma_H(s)$, both $i$ 
	and $o$ are adjacent to $s$. Therefore, $\Sis=\Sos=1$ and properties 4(a) and 4(b) of 
	Definition~\ref{p:defn:hardness-gadget} hold. Every $x\in\Oz-s$ is adjacent to $i$, so $\Six=1$ and property~4(c) 
	Definition~\ref{p:defn:hardness-gadget} 
	holds. 
\end{proof}

\begin{figure}
	\begin{center}
%		\begin{tikzpicture}[scale=1,node distance = 1.5cm]
%		\tikzstyle{vertex}=[fill=black, draw=black, circle, inner sep=1.5pt]
%		
%		\node[vertex] (1) at (0,0) {};
%		\node[vertex] (2) at (1,0) {};
%		\node[vertex] (3) at (2,0) {};
%		\node[vertex] (4) at (3,0) {};
%		\node[vertex] (5) at (4,0) {};
%		\node[vertex] (6) at (5,0) {};
%		\node[vertex] (7) at (6,0) {};
%		\node[vertex] (8) at (7,0) {};
%		\node[vertex] (9) at (2,1) {};
%		\node[vertex] (10) at (4,1) {};
%		\node[vertex] (11) at (5,1) {};
%		
%		\draw (1)--(2)--(3)--(4)--(5)--(6)--(7)--(8);
%		\draw (4)--(9);
%		\draw (4)--(10)--(11);
%		\end{tikzpicture}
	\includegraphics[]{TikZ/3_problem_case.pdf}
	\end{center}
	\caption{An example of an asymmetric tree that does not have a degree~2 vertex adjacent to a degree~3 vertex.}
	\label{fig:3-problem-case}
\end{figure}

When $p=3$ there exists assymetric trees, for which applying Lemma~\ref{lem:tree-23-gadget} would give us a 
$(2,3)$-gadget. Such an example is shown in Figure~\ref{fig:3-problem-case}.
This is not sufficient to give us hardness for \threehcol{}, as $2^2\equiv 1\pmod 3$, so 
Theorem~\ref{p:thm:hardness-gadget} doesn't apply. 
By Lemma~\ref{lem:consecutive-degrees}, if $H$ is an asymmetric tree that does not have a degree~2 vertex adjacent 
to a degree~3 vertex, then it must have two adjacent vertices of degree~2 and 
one of them is adjacent to a leaf. It turns out that this structure is sufficient to give us a $(3,3)$-gadget for $H$.

\begin{figure}[t]
	\begin{center}
%		\begin{tikzpicture}[scale=1.2,node distance = 1.5cm]
%		\tikzstyle{dot}   =[fill=black, draw=black, circle, inner sep=0.15mm]
%		\tikzstyle{vertex}=[fill=black, draw=black, circle, inner sep=2pt]
%		\tikzstyle{dist}  =[fill=white, draw=black, circle, inner sep=2pt]
%		\tikzstyle{pinned}=[fill=white, draw=black, minimum size=9mm, circle,inner sep=0pt]
%		
%		\begin{scope}[shift={(-3,0)}]
%		\node[vertex] at (0,0) (0) [label=135:{$o$}]{};
%		\node[vertex] at (1,0) (1) [label=135:{$s$}] {};
%		\node[vertex] at (2,0) (2) [label=135:{$i$}] {};
%		\node[vertex] at (3,0) (3) [label=135:{$x$}] {};
%		
%		\draw[dashed] (4,0) ellipse  (1.5cm and 1cm);
%		\draw (0)--(1)--(2)--(3);
%		\draw[dashed] (3)--(3.6,0);
%		\draw[dashed] (3)--(3.4,-.4);
%		\draw[dashed] (3)--(3.4,.4);
%		
%		\node at (3,-1) {$H$};
%		\end{scope}
%		
%		\begin{scope}[shift={(4,1.75)}]
%		\node at (0,0) {$J_1$:};
%		
%		\node[pinned] (p1) at (1,0) [label=-90:$u$]{$\strut s$};
%		\node[dist]   (y)  at (2,0) [label=-90:$y$] {};
%		
%		\draw (p1) -- (y);
%		\end{scope}
%		
%		\begin{scope}[shift={(4,0.5)}]
%		\node at (0,0) {$J_2$:};
%		
%		\node[pinned] (p3) at (1,0) [label=-90:$w_1$]{$\strut s$};
%		\node[vertex]  (w) at (2,0) [label=-90:$w_2$]{};
%		\node[dist]   (z)  at (3,0) [label=-90:$z$] {};
%		
%		\draw (p3)-- (w)-- (z);
%		\end{scope}
%		
%		\begin{scope}[shift={(4,-0.75)}]
%		\node at (0,0) {$J_3$:};
%		
%		\node[dist] (yy) at (1,0) [label=-90:$y$] {};
%		\node[dist] (zz) at (2,0) [label=-90:$z$] {};
%		
%		\draw (yy) -- (zz);
%		\end{scope}
%		
%		\end{tikzpicture}
		\includegraphics[]{TikZ/tree_22_gadget.pdf}
	\end{center}
	\caption{A $(3,3)$-gadget for the asymmetric tree~$H$ as in the proof of Lemma~\ref{lem:tree-22-gadget}. Normal 
		vertices appear as black dots, distinguished vertices as small white circles. Pinned vertices appear as large white 
		circles where the label inside the vertex indicates what the vertex is pinned to. The ellipse denotes the rest 
		of the graph $H$.}
	\label{fig:tree-22-gadget}
\end{figure}

\begin{lemma}\label{lem:tree-22-gadget}
	Let $p$ be a prime and let $H$ be a tree. If $H$ has a vertex~$s$ of degree~2 that is adjacent to a 
	leaf~$o$ and a vertex~$i$ of degree~$2$, then $H$ has a $(3,3)$-gadget.
\end{lemma}
\begin{proof}
	We define the $(3,p)$-gadget of $H$ to be $(i,s,(J_1,y),(J_2,z),(J_3,y,z))$, where $J_1,J_2,J_3$ are defined as 
	follows (see Figure~\ref{fig:tree-22-gadget}):
	\begin{itemize}
		\item $J_1$ is the edge $(u,y)$, with $\tau(J_1)=\{u\mapsto s\}$.
		\item $J_2$ is the path $w_1w_2z$, with $\tau(J_2)=\{w_1\mapsto s\}$.
		\item $J_3$ is the edge $(y,z)$.
	\end{itemize}
	
	It remains to show that properties 1-4 of Definition~\ref{p:defn:hardness-gadget} hold.
	
	$G(J_1)$ is just an edge so, for each $v\in\Gamma_H(s)$, $N_1(v)=1$ and, for every $v'\notin\Gamma_H(v_1)$, it holds 
	that $N_1(u)=0$. Therefore $\Oy=\Gamma_H(s)$. Clearly $i\in\Oy$ and $|\Oy|=\deg_H(s)=2$. Hence, 
	property~1 of Definition~\ref{p:defn:hardness-gadget} holds. 
	
	Let $x\neq s$ be the other neighbour of $i$ and consider $G(J_2)$. Any homomorphism $\sigma:V(G(J_2))\rightarrow H$ 
	that 
	respects $\tau(J_2)$ must have $\sigma(w_2)\in\Gamma_H(s)=\{o,i\}$. If $\sigma(w_2)=o$, then $\sigma(z)=s$, otherwise 
	$\sigma(w_2)=i$ and $\sigma(z)\in\Gamma_H(i)=\{s,x\}$. This shows that $\Oz=\{s,x\}$, $N_2(s)=2$ and $N_2(x)=1$. So 
	$\sum_{b\in\Oz}N_2(b)=3\equiv6 \pmod3$ and property~2 of Definition~\ref{p:defn:hardness-gadget} holds for $\kappa=2$.
	
	$G(J_3)$ is a simple edge, so for $a,b\in V(G)$, $N_3(a,b)=1$ if and only if $a$ is adjacent to $b$, otherwise 
	$N_3(a,b)=0$. Since $o$ is a leaf that is only adjacent to $s$, $\Sox=0$ and property~3 of 
	Definition~\ref{p:defn:hardness-gadget} holds. 
	
	Since $\Oy=\Gamma_H(s)$, both $i$ 
	and $o$ are adjacent to $s$. Therefore $\Sis=\Sos=1$ and properties 4(a) and 4(b) of 
	Definition~\ref{p:defn:hardness-gadget} hold. Every $x\in\Oz-s$ is adjacent to $i$, so $\Six=1$ and property~4(c) 
	Definition~\ref{p:defn:hardness-gadget} 
	holds.
\end{proof}

Recall that we have shown that when an asymmetric graph $H$ contains a $(\gamma,p)$-gadget, where 
$\gamma^2\not\equiv1\pmod p$ then \phcol{} is $\numpp$-hard (Theorem~\ref{p:thm:hardness-gadget}). The latter combined 
with Lemmas~\ref{lem:consecutive-degrees},~\ref{lem:tree-23-gadget} and~\ref{lem:tree-22-gadget} suffices to show that, 
for every asymmetric tree~$H$ with more than one vertex \phcol{} is 
$\numpp$-hard.

\begin{lemma}\label{p:lem:hardness}
	Let $H$ be an asymmetric tree with more than one vertex. For any prime $p\geq3$, \phcol{} is $\numpp$-hard.
\end{lemma}
\begin{proof}
	Since $H$ is an asymmetric tree and has more than one vertex we can apply Lemma~\ref{lem:consecutive-degrees} to find 
	a vertex~$s$, with $\deg_H(s)=2$, that is adjacent to a leaf~$o$ and a vertex~$i$ with $\deg_H(i)\in\{2,3\}$. Let 
	$\gamma=\deg_H(i)$.
	
	If $p>3$, then, by Lemma~\ref{lem:tree-23-gadget}, $H$ has a $(\gamma,p)$-gadget. Since $\gamma\in\{2,3\}$ and $p>3$, 
	we have that $\gamma^2\not\equiv1\pmod p$ and the lemma follows from Theorem~\ref{p:thm:hardness-gadget}.
	
	If $p=3$ and $\gamma=3$, then, by Lemma~\ref{lem:tree-23-gadget}, $H$ has a $(3,3)$-gadget; otherwise $\gamma=2$ and, 
	by Lemma~\ref{lem:tree-22-gadget}, $H$ has a $(3,3)$-gadget. The lemma follows from Theorem~\ref{p:thm:hardness-gadget}.
\end{proof}

When $p=2$, hardness for \parhcol{} comes from the results of Faben and Jerrum \cite[Lemma~5.4]{FJ13} 
and~\cite[Theorem~5.6]{FJ13}.

\begin{lemma}[Faben and Jerrum, Lemma~5.4]
	An involution-free tree has trivial automorphism group.
\end{lemma}

\begin{theorem}[Faben and Jerrum, Theorem~5.6]\label{thm:hardness-tree-2}
	Given an involution-free tree $H$ with more than one vertex, \parhcol{} is $\parp$-complete.
\end{theorem}


We have shown that for all primes $p$ and all asymmetric graphs~$H$ with more than one vertex \phcol{} is 
$\numpp$-hard. Recall Definition~\ref{defn:reduced-form} of an order $p$ reduced form of a graph $H$.
By Theorem~\ref{thm:involution-unique}, $H^{*p}$ is unique (up to isomorphism). By 
Theorem~\ref{thm:involution-reduction}, \phcol{} has the same complexity as $\phcol[H^{*p}]$. 

We can now prove the main theorem of this chapter.

{\renewcommand{\thetheorem}{\ref{thm:main-trees}}
	\begin{theorem}
		Let $p$ be a prime and let $H$ be a graph whose order~$p$ reduced form~$H^{*p}$ is an asymmetric tree. If $H^{*p}$ has 
		more than one vertex then \phcol{} is $\numpp$-hard, otherwise \phcol{} is computable in polynomial time.
	\end{theorem}}
	\begin{proof}
		By Theorem~\ref{thm:involution-reduction}, \phcol{} and $\phcol[H^{*p}]$ have the same computational complexity.
		If $H^{*p}$ has at most one vertex, then, by Corollary~\ref{cor:involution-polynomial}, \phcol{} is computable in 
		polynomial-time. Otherwise, $H^{*p}$ has more than one vertex. If $p=2$ \phcol{} is $\parp$-complete by 
		Theorem~\ref{thm:hardness-tree-2}. Otherwise, $p>2$ and \phcol{} is $\numpp$-complete by Lemma~\ref{p:lem:hardness}.
	\end{proof}
	
\subsubsection{Gadgets}
	
	Since we will be dealing with all trees, not just asymmetric, we need to extend the definition of a $(g,p)$-gadget to 
	the following.
	
	\begin{definition}\agob{defined it with $\alpha,\beta$ for now, but we should switch to $\gamma,\lambda$ if we don't 
			need the generality}
		\label{defn:gl-gadget}
		A \emph{$(\alpha,\beta,p)$-gadget} $(i,s,(J_1,y),(J_2,z),(J_3,y,z))$ consists
		of vertices $i$ and $s$ of $H$ together with three partially labelled
		graphs with distinguished vertices $(J_1,y)$, $(J_2,z)$ and $(J_3,y,z)$, where $y$ and $z$ are distinct, satisfying the 
		properties explained bellow. Let
		
		\begin{align*}
		N_1(v) &= |\Homs{(J_1,y)}{(H,v)}|\\
		N_2(v) &= |\Homs{(J_2,z)}{(H,v)}|\\
		N_3(u,v) &=|\Homs{(J_3,y,z)}{(H,u,v)}|\\
		\Oy &= \{ u \in V(H) \mid N_1(v)\not\equiv0\pmod p\}\\
		\Oz &= \{ u \in V(H) \mid N_2(v)\not\equiv0\pmod p\}\,.
		\end{align*}
		
		The properties that we require are:
		
		\begin{enumerate}
			\item $\Oy\neq\emptyset$, $N_1(i)\equiv \kappa_i\pmod p$ and for each $o\in\Oy-i$, $N_1(o)\equiv \kappa_o \pmod p$, 
			with $\kappa_i^{-1}\kappa_o|\Oy|\equiv \beta\pmod p$.
			\item $\sum_{b\in\Oz}N_2(b)\equiv\alpha\kappa$ and $N_2(s)\equiv\kappa \pmod p$, where $\kappa\not\equiv0\pmod p$. 
			\item For each $o\in \Oy-i$ and each $x\in \Oz-s$, $\Sox\equiv0\pmod p$.
			\item And for each $o\in \Oy-i$ and each $x\in \Oz-s$ the following hold:\agob{I can even be more general with the 
				requirements for $J_3$, just the reduction is gonna get even uglier and I don't know what more we can get.}
			\begin{enumerate}
				\item $\Sis\equiv1\pmod p$
				\item $\Sos\equiv1\pmod p$
				\item $\Six\equiv1\pmod p$.
			\end{enumerate}
		\end{enumerate}
	\end{definition}
	
	
	The main theorem we can prove is the following:
	\agob{The $\lambda+1$ is annoying to carry around, For now I leave it in the reduction.}
	\begin{theorem}
		Let $p$ be a prime and let $H$ be a graph. If $H$ contains a $(\gamma,\lambda+1,p)$-gadget, then \glpart{} reduces to 
		\phcol{} via polynomial time Turing reductions.
	\end{theorem}
	\begin{proof}
		The proof should be similar to the proof of Theorem~\ref{p:thm:hardness-gadget}, with some extra's for the vertex 
		weights.
	\end{proof}
	
\subsubsection{List of possible Gadgets}
	
	We will be concerned with the graph~$H$ containing two adjacent non-leaf vertices $s$ and $i$, where $\deg_H(s)=b$ and 
	$\deg_H(i)=a$, with $a,b\not\equiv1\pmod p$. Note that $i$ and $s$ are interchangeable so in the following graphs we 
	can always inverse $a$ and $b$. We have the following gadgets:
	
	\begin{itemize}
		\item $(a,b,p)$:
		\begin{itemize}
			\item $J_1$ is the edge $(u,y)$, with $\tau(J_1)=\{u\mapsto s\}$.
			\item $J_2$ is the edge $(w,z)$, with $\tau(J_2)=\{w\mapsto i\}$.
			\item $J_3$ is the edge $(y,z)$.
		\end{itemize}
		
		\item $(1+b^{-1}(a-1),b,p)$:
		\begin{itemize}
			\item $J_1$ is the edge $(u,y)$, with $\tau(J_1)=\{u\mapsto s\}$.
			\item $J_2$ is the path $w_1w_2z$, with $\tau(J_2)=\{w_1\mapsto s\}$.
			\item $J_3$ is the edge $(y,z)$.
		\end{itemize}
		
		\item $(a,a^{-1}b,p)$:
		\begin{itemize}
			\item $J_1$ is the path $u_1u_2y)$, with $\tau(J_1)=\{u_1\mapsto i\}$.
			\item $J_2$ is the edge $(w,z)$, with $\tau(J_2)=\{w\mapsto i\}$.
			\item $J_3$ is the edge $(y,z)$.
		\end{itemize}
		
		\item $(1+b^{-1}(a-1),a^{-1}b,p)$:
		\begin{itemize}
			\item $J_1$ is the path $u_1u_2y)$, with $\tau(J_1)=\{u_1\mapsto i\}$.
			\item $J_2$ is the path $w_1w_2z$, with $\tau(J_2)=\{w_1\mapsto s\}$.
			\item $J_3$ is the edge $(y,z)$.
		\end{itemize}
		In general I can get $(1+b^{-k}(a-1),a^{-k'}b,p)$ by using $k$ copies of $J_2$ and $k'$ copies of $J_1$.
	\end{itemize}
	
	Note that, because of bipartition of $H$, we can only get that $\Oy=\{o,i\}$ for all copies of $o$ and $\Oz=\{s,x\}$ 
	for all copies of $x's$. We can only alter the way they interact.


==> bipartite-copy.tex <==

% \newcommand{\pbislr}[2]{\ensuremath{\#_p\prb{BIS}_{#1,#2}}}
%
%\section{The bipartite approach}


For every graph $G=(V,E)$ we denote by $\calI(G):=\{I\subseteq V\mid \forall x_1,x_2\in I \; (x_1,x_2)\notin E\}$ the set of independent sets of $G$.
\ks{add reference}
It is well known that for every $k\in\Z$ the problem of determining the number $|\calI (G)| \pmod k$ is $\nkp$-complete.
A graph is bipartite in case there exist disjoint subsets $V_L$, $V_R$ of $V$ such that $V=V_L\cup V_R$ and for all $x_1,x_2 \in V$ from $(x_1,x_2)\in E$ follows $x_1\in V_L$ and $x_2\in V_R$ or vice versa.
The starting point of our reduction is the problem $\kbis{k}$, where the task is to compute $|\calI(G)|\pmod k$ for a bipartite input graph with a given partition $G=\bipG$.
Therefore, in the rest of this section we only consider (simple) bipartite graphs already equiped with a partition.
In fact, \citet*[Theorem~3.7]{Fab08}
\ks{this reference is incorrect}
showed that $\kbis{k}$ is still hard.
\GL{Is simple needed? I suggest to use $N(v)$ for the neighbourhood of $v$, $\Gamma$ lets me think of the $\Gamma$-function.}

%When the input graph $G$ is restricted to be bipartite the problem is given as follows.
%
%The starting point for our reductions is the 
%following problem.

%\prob{\kbis{k}.\label{prob:kbis}}
%{A bipartite graph $G=\bipG$.}
%{$|\calI(G)|\pmod k$.}


\begin{theorem}[\citet*{Fab08}]\label{thm:bis}
	For all positive integers~$k$, \kbis{k} is $\nkp$-complete.
\end{theorem}


%\agob{Maybe I need $Z(G)$ to be in a definition as I use it a lot in this section.}

Aiming at
\ks{what is the goal?},
we consider the weighted version $\pbislr{\lweight}{\rweight}$
\agob{explain focus on primes.
Maybe composites sections first?} of $\kbis{k}$, in which each partition has a weight attached to it: $\lweight$ or $\rweight$.
Every independent set $I$ will now contribute a product with $\lweight$ as factor for every vertex in $\lpart \cap I$ and $\rweight$ for every vertex in $\rpart \cap I$, respectively. 
%Every independent set $I$ will now contribute the product $\lweight^{n_L(I)} \rweight^{n_R(I)}$, where $n_L(I):=|I\cap V_L|$ and $n_R(I):=|I\cap V_R|$ are the size of $I$ restricted to vertices in $\lpart$ or $\rpart$, respectively. 
More formally, given a partitioned bipartite graph $G$ we define 
$$\wISet{G}=\sum_{I\in\calI(G)}\lweight^{|\lpart \cap I|}\rweight^{|\rpart \cap I|}.$$
Clearly, the empty set always contributes a summand of $1$ to $\wISet{G}$.
\agob{explain the weight of the hardcore model, so maybe mention the hardcore model beforehand}


%We will study the following problem.
\probpar{\pbislr{\lweight}{\rweight}.}
	{$p$ prime and $\lweight, \rweight \in\zsp$}
	{partitioned bipartite graph $G=\bipG$.}
	{$\wISet{G} \pmod p$.}

Since $\pbislr{1}{1}$ corresponds to the special case $\kbis{p}$, Theorem~\ref{thm:bis} directly implies that \pbislr{1}{1} is $\numpp$-complete for all primes~$p$.
Further note that \pbislr{\lambda}{\lambda} corresponds to the hard-core model on bipartite graphs with activity $\lambda$.
\agob{Citations and talk a bit more on the importance of the hard-core model.} 

\medskip
We first observe that $\pbislr{\lweight}{\rweight}$ is easy in case $\lweight$ or $\rweight$ is a multiple of $p$.

\begin{proposition}\label{prop:BIS_easy_cases}
	If $\lweight\equiv 0 \pmod p$  or $\rweight \equiv 0 \pmod p$ then \pbislr{\lweight}{\rweight} is computable in polynomial time. 
\end{proposition}
\begin{proof}
	Without loss of generality we assume $\lweight \equiv 0 \pmod p$. Thus, any 
	independent set that contains at least one vertex from $\lpart$ contributes zero to the sum in \wISet{G}. 
	Therefore, we only need to consider the independent sets~$I$ with $I\not\subseteq\lpart$. Since the vertices of $\rpart$ form an independent set, we sum up over all subsets of $V_R$ and obtain
	\begin{align*}
		\wISet{G} & \equiv 1+\sum_{i=1}^{|\rpart|}\binom{|\rpart|}{i}(\rweight)^i\pmod p \\
		 & = \sum_{i=0}^{|\rpart|}\binom{|\rpart|}{i}(\rweight)^i 
		 = (\rweight+1)^{|\rpart|},
	\end{align*}
	which can be computed in polynomial time.
\end{proof}

The rest of this section is dedicated to proving that in all other cases \pbislr{\lweight}{\rweight} is hard.
Our proof employes the construction in the proof of \citet*[Theorem~3.7]{Fab08},
\ks{change reference according to above}
but with a more careful consideration of gadgets.
\ks{explain term gadget or replace it by other formulation}

\begin{definition}\label{def:is-l-r-lr}
Let $G=\bipG$ be a partioned bipartide graph.
We denote by $\calI{_L}(G)$ the set $\{I\in\calI(G)\setminus\{\varnothing\}\mid I\subseteq V_L \}$ of independent sets containing only vertices from $\lpart$.
Similarly, we write $\calI{_\R} (G)$ for the set of independent sets that contain only vertices from $\rpart$.
Finally, $\calI_{\L \R} (G) := \calI(G)\setminus(\,\calI_L(G)\cup\calI_R(G)\,)$ contains all independent sets $I$ with at least one vertex from $\lpart$ and at least one vertex from $\rpart$. 
\end{definition}

In order to avoid double-counting we excluded the empty set from $\calI_\L(G)$ and $\calI_\R(G)$.

%This definition shall retain clarity as well as avoid double-counting.
We first shed a bit more light on the proof of Proposition~\ref{prop:BIS_easy_cases}.
If $\lweight \equiv 0 \pmod p$ only the empty set and independent sets in $\calI_R$ contribute non-zero terms to \wISet{G}.
Repeating the argument for $\rweight \equiv 0 \pmod p$ reveals that for hardness results the independent sets in $\calI_{\L \R}$ may play a crucial role.
Therefore, the next lemma takes apart the computation of $\wISet{G}$ according to the provided partition $\{\calI_\L (G),\calI_\R (G),\calI_{\L\R}(G),\{\emptyset\}\}$ of $I(G)$ in Definition \ref{def:is-l-r-lr}.


\begin{lemma}\label{lem:split-sum-part}
Let $G=\bipG$ be a partitioned bipartite graph.
Then,
\[
\wISet{G} =(\lweight+1)^{|\lpart|}+(\rweight+1)^{|\rpart|}-1+\sum_{I\in\calI_{\L \R}} \lweight^{|\lpart\cap I|} \rweight^{|\rpart \cap I|}.
\]
\end{lemma}
\begin{proof}
Refering to Definition~\ref{def:is-l-r-lr} we observe
\begin{align}
		\wISet{G}& =\sum_{I\in\calI(G)}\lweight^{|\lpart\cap I|}\rweight^{|\rpart\cap I|} \nonumber \\
		 &= \sum_{I\in\calI_\L (G)}\lweight^{|I|}+\sum_{I\in\calI_\R(G)}\rweight^{|I|}+\sum_{I\in\calI_{\L\R}(G)}\lweight^{|\lpart \cap I|}\rweight^{|\rpart \cap I|}+1. \label{eq:tot-sum}
\end{align}

%Since the graph is bipartite, there is no adjacent pair of vertices in $\lpart$ (resp. $\rpart$). Hence, any subset of $\lpart$ (resp. $\rpart$) yields an independent set of $G$.
As in the proof Proposition \ref{prop:BIS_easy_cases}, we obtain
\begin{align}
	 \label{eq:left-is}
	 \sum_{I\in\calI_\L(G)} \lweight^{|I|} &= \sum_{i=0}^{|\lpart|}\binom{|\lpart|}{i}\lweight^i - 1 = (\lweight+1)^{|\lpart|}-1, \qquad \mbox{and analoguously} \\
	 \label{eq:right-is}
	 \sum_{I\in\calI_\R (G)} \rweight^{|I|} &= (\rweight+1)^{|\rpart|}-1.
\end{align}
%
%	Similarly, 
%	\begin{equation}
%		 \sum_{I_\R \in \calI_\R (G)} \rweight^{|I_\R|} = (\rweight+1)^{|\rpart|}-1.  \label{eq:right-is}
%	\end{equation}
	Inserting \eqref{eq:right-is} and \eqref{eq:left-is} into \eqref{eq:tot-sum} yields the lemma.
\end{proof}

In order to deal with the behaviour afflicted by independent sets in $\calI_{\L \R}$ we are going to use the following graph as a gadget.
\begin{definition}\label{def:special_bip_graph}
	Given a prime $p$ and two weights $\lweight, \rweight \in \zsp$ we define the bipartite graph $B(k, p)=\bipG$ as follows. The two vertex partitions are given by $V_L=\{u_1\dots u_{2(p-1)}\}$ and
	$V_R=\{w_1,\dots, w_{2(p-1)}\}$. The edge set given by $E=\{(u_i,w_j)\mid i,j\in[2(p-1)], \textrm{ where } i\neq 
	j\}\cup\{(u_i,w_i)\mid 	i \notin [k]\}$ consists of any possible edges subtracted by edges $(u_i, w_i)$ with $i\in [k]$.	 
\end{definition}

The reason each partition has $2(p-1)$ vertices instead of $p-1$ is to ensure the existence of the edges $(u_i,w_i)$ for all possible choices of $k$. As an example, the graph $B(1, 3)$ is shown in Figure~\ref{fig:bip_gadget}.
\begin{figure}[t] \label{fig:bip_gadget}
	\centering
	\includegraphics{TikZ/bip_gadget_construction.pdf}
	\caption{Construction for $p=3$ and $k=1$. Starting with the complete bipartite graph $K_{4,4}$ the edge $(u_1, w_1)$ is removed.}
\end{figure}

The freedom of choice for $k$ will entail the possibility to, given $\lweight, \rweight \not\equiv 0\pmod p$, choose $k$ such that $\wISet{B(k, p)} \equiv 0 \pmod p$. Moreover, removing one vertex $v$ out of $B$ will yield a non-zero weighted sum $\wISet{B(k, p) - v}$. As we shall see, it suffices to choose $k \in \zsp$ such that $k \equiv -(\lweight \rweight)^{-1} \pmod p$. Since $p$ is a prime, $\zp$ is a field and such a $k$ exists uniquely in \zp. More formally, we have the following Lemma.
\begin{lemma}\label{lem:bip-gadget}
	Let~$p$ be a prime, $\lweight, \rweight \in \zsp$ and $k \in \zsp$ with $k \equiv -(\lweight \rweight)^{-1} \pmod p$. Then, the bipartite graph $B=B(k, p)$ with two 
	distinguished vertices $v_\L = u_{2(p-1)} \in V_\L$ and $v_\R = w_{2(p-1)} \in V_\R$ satisfies the following properties
	\begin{enumerate}
		 \item $\wISet{B} \equiv 0\pmod p$,
		 \item $\wISet{B-v_\L} \equiv (\lweight+1)^{-1} -1\pmod p$ and
		 \item $\wISet{B-v_\R} \equiv (\rweight+1)^{-1} -1 \pmod p$.
	\end{enumerate}
\end{lemma}
\begin{proof}
%	Since $p$ is a prime $\zp$ is a field. Moreover,
%	since $\lweight, \rweight \not\equiv 0\pmod p$ there exists a unique $k \in \zsp$, such that $k=-(\lweight \rweight)^{-1}$. We choose $B=B(k,p)$ as given by Definition~\ref{def:special_bip_graph} and
%	fix $v_\L=u_{2(p-1)}$, $v_\R=w_{2(p-1)}$ to be the distinguished vertices of $B$. 
%
	By Lemma~\ref{lem:split-sum-part} we obtain
	\begin{align*}
		\wISet{B}&=(\lweight+1)^{|\lpart|}+(\rweight+1)^{|\rpart|}-1+\sum_{I\in\calI_{\L\R}}\lweight^{|\lpart\cap I_{\L\R}|}\rweight^{|\rpart\cap	I_{\L\R}|}\\
		&= (\lweight+1)^{2(p-1)}+(\rweight+1)^{2(p-1)}-1+\sum_{I\in\calI_{\L\R}}\lweight^{|\lpart\cap I_{\L\R}|}\rweight^{|\rpart\cap	I_{\L\R}|} ,
	\end{align*}
	which simplifies due to Fermat's little Theorem~\ref{thm:Fermat} to
	\begin{align}\label{eq:proof_bip-gadget}
		\wISet{B} \equiv 1 + \sum_{I\in\calI_{\L\R}}\lweight^{|\lpart\cap I_{\L\R}|}\rweight^{|\rpart\cap I_{\L\R}|} \pmod p .
	\end{align}
	Therefore, it suffices to study $\calI_{\L\R}(B)$. Let $I_{\L\R}\in\calI_LR(B)$ be a non-empty independent set containing a vertex $u_j \in \rpart$ and $v_j \in \lpart$. In fact, by the definition of $B$ there is no independent set containing two vertices $u_i$ and $w_j$ with $i \neq j$.
	%We first show that $\calI_{LR}(B)=\{\{u_i,w_i\}\mid i\in[k]\}$. 
	For $k<j\leq 2(p-1)$, $u_j$ is connected to 
	every vertex in $\rpart$ and $w_j$ is connected to every vertex in $\lpart$, thus $I_{\L\R}$ cannot contain $u_j$ nor $w_j$. 
	%Let $I_{\L\R}\in\calI_LR(B)$ 
	For $1 \leq j \leq k$ by definition of $B$ the only vertex in $\rpart$ 
	not adjacent to $u_j$ is $w_j$. Therefore, $I_{\L \R} = \{u_j, w_j\}$
	%and there is no $k\neq i$ such that $u_k\in I_{LR}$. 
	%Likewise, the only vertex in $V_L$ that is not adjacent to $w_i$ is $u_i$, hence there is no $i'\neq i$ such that 
	%$u_{i'}\in I_{LR}$. Hence $I_{LR}=\{u_i,w_i\}$ 
	yielding $\calI_{LR}=\{\{u_i,w_i\}\mid i\in[k]\}$, and by \eqref{eq:proof_bip-gadget}	
	\begin{align*}
		\wISet{B}
		%&=
		%(\lweight+1)^{|\lpart|}+(\rweight+1)^{|\rpart|}-1+\sum_{I\in\calI_{\L\R}}\lweight^{|\lpart\cap I_{\L\R}|}\rweight^{|\rpart\cap	I_{\L\R}|}\\
		%&= (\lweight+1)^{2(p-1)}+(\rweight+1)^{2(p-1)}-1+\sum_{i=1}^k \lweight \rweight\\
		&\equiv 1-(\lweight \rweight )^{-1}(\lweight \rweight) \pmod p
		= 0 .
	\end{align*}
	This proves Property~$\mathit{1}$ of the lemma. 
	
	Property~$\mathit{2}$ and $\mathit{3}$ are analogue. Therefore, it remains to show property~$\mathit{2}$ since the similar argument yields property~$\mathit{3}$. $B-v_L$ is a bipartite graph and we can apply Lemma~\ref{lem:split-sum-part} similarly as above yielding
	\begin{align*}
		\wISet{B-v_\L} 
%		&=(\lweight+1)^{|\lpart|} + (\rweight+1)^{|\rpart|} - 1 + \sum_{I\in\calI_{\L\R}(B-v_\L)}\lweight^{|\lpart\cap 
%		I_{\L\R}|} \rweight^{|\rpart \cap I_{\L\R}|}
		&= (\lweight+1)^{2p-3} + (\rweight+1)^{2(p-1)} - 1 + \sum_{I\in\calI_{\L\R}(B-v_\L)}\lweight^{|\lpart\cap 
			I_{\L\R}|} \rweight^{|\rpart \cap I_{\L\R}|} \\
		&\equiv (\lweight+1)^{-1} + + \sum_{I\in\calI_{\L\R}(B-v_\L)}\lweight^{|\lpart\cap 
			I_{\L\R}|} \rweight^{|\rpart \cap I_{\L\R}|} \pmod p .
%		+ \sum_{i=1}^k \lweight \rweight\\
%		&\equiv (\lweight+1)^{-1} - (\lweight \rweight)^{-1}(\lweight \rweight) \pmod p\\
%		&\equiv (\lweight +1)^{-1} - 1 \pmod p.
	\end{align*}
	Finally, we observe that deleting $v_\L = u_{2(p-1)}$ from $B$ does not afflict the set $\calI_{\L \R}$ since $2(p-1) > k$ for all possible choices of k. Hence, $I_{\L \R} = \{u_j, w_j\}$ still holds concluding the proof.
%
%Hence, Property~$2$ of the lemma holds. 
%The proof of Property~$3$ is similar to the proof of Property~$2$ and the lemma follows.
\end{proof}

Lemma~\ref{lem:bip-gadget} can be used in Faben's proof to give the following theorem. For the sake of completeness we 
include a self contained proof.
\todo{Define \numpsat{} formally and cite its hardness. We also need to define $\sat()$.}

The following theorem yields the desired hardness result for \pbislr{\lweight}{\rweight}. In order to prove it, we are going to reduce from the well-known \numpp{}-complete problem \numpsat{} by using a suitable gadget graph, whose construction we are going to give at this point for the sake of clarity. Given a Boolean formula $\varphi$ in conjunctive normal form with set of variables $\var(\varphi)=\{x_1\dots x_n\}$ and set of clauses $\clause(\varphi)=\{c_1,\dots,c_m\}$, we are going to construct the gadget graph $G_\varphi$ in two stages:

First, we construct the graph $G'_\varphi$ (see the left part of Figure~\ref{fig:weighted_BIS} for an example). For variable $x_i$ in $\var(\varphi)$ we introduce the three vertices $v_i$ ,$\bar{v_i}$ and $z_i$ to the first vertex-partition $\lpart (G'_\varphi)$ as well as the three vertices $u_i$, $\bar{u_i}$ and $w_i$ to the second vertex partition $\rpart (G'_\varphi)$. Furthermore, for every clause $c_j$ in $\clause(\varphi)$ we introduce a vertex $y_j$ to the second vertex partition $\rpart (G'_\varphi)$. This yields $V_L(G'_\varphi)=\{v_i,\bar{v_i},z_i\mid i\in[n]\}$ and $V_R(G'_\varphi)=\{u_i,\bar{u_i},w_i\mid i\in[n]\}\cup\{y_j\mid j\in[m]\}$.

For every $i \in [n]$ we introduce the edges forming the cycle $v_iu_iz_i\bar{u_i}\bar{v_i}w_iv_i$ to $E(G'_\varphi)$. Additionally, for every $j \in [m]$ we introduce an edge connecting $y_j$ to $v_i$ or $\bar{v_i}$ depending on the appearance of $x_i$ in the clause $c_j$: if $x_i$ appears non-negated we connect $y_j$ to $v_i$ and if $x_i$ appears negated we connect $y_j$ to $\bar{v_i}$. This yields 
$E(G'_\varphi) = \bigcup_{i \in [n]} \bigcup_{j \in [m]}  E(v_iu_iz_i\bar{u_i}\bar{v_i}w_iv_i) \cup \{(y_j, v_i) \mid x_i \in c_j\} \cup \{(y_j, \bar{v_i}) \mid \bar{x_i} \in c_j\}$.
%$E(G'_\varphi)=\{(v_i,u_i),(u_i, z_i), (z_i, \bar{u_i}), (\bar{u_i},\bar{v_i}),(v_i,w_i),(\bar{v_i},w_i),\}$. 
We note that there are no adjacent vertices in each partition. Hence, the graph $G'_\varphi$ is bipartite. For the second step we apply the following notation in order to build a graph containing many copies of some subgraph.

\begin{notation}
	For any ``tag''~$T$ (which we will treat just as an arbitrary string) and any 
	graph~$J$, denote by $J^T$ a copy of~$J$ with every vertex $v\in V(J)$ renamed~$v^T\!$. 
\end{notation}

\begin{figure}[t]\label{fig:weighted_BIS}
	\centering
	\includegraphics[width=\textwidth]{TikZ/weighted_BIS.pdf}
	\caption{The graphs $G'_\varphi$ and $G_\varphi$ for $\varphi = \textcolor{mycolor1}{(x_1 \vee x_2)} \wedge \textcolor{mycolor2}{(\bar{x}_1 \vee x_2 \vee x_3)}.$}
\end{figure}
\GL{We changed notation for the vertex $c_j$ to $y_j$.}
Second, we construct the graph $G_\varphi$ (see the right part of Figure~\ref{fig:weighted_BIS} for an example). This construction starts with the graph $G'_\varphi$. Lemma~\ref{lem:bip-gadget} yields the graph $B$ along with its two distinguished vertices $v_\L$, $v_\R$ and the three properties, which we are going to be central to the proof.
For every $j \in [2n + m]$ we take a copy of $B$ denoted $B^j$, essentially we introduce one copy for every clause and two for every variable of $\varphi$. For every variable $x_i$ in $\varphi$ we identify $z_i$ with $v_\L^i$ as well as $w_i$ with $v_\R^{n+i}$. Additionally, for every clause $c_j$ in $\varphi$ we identify $y_j$ with $v_\R^{2n+j}$. This 
concludes the construction of $G_\varphi$.

We note, that the identification has been done in a way ensuring that $G_\varphi$ is bipartite and the assignment of vertices to the partition is preserved, i.e. $v \in \lpart (G_\varphi)$ if and only if $v \in \lpart (G'_\varphi)$ or $v \in \lpart(B^j)$ for some $j \in [2n +m]$ (analogue for the second partition). This can be easily justified with the identification of a vertex $v \in \lpart (G'_\varphi)$ with a vertex $w \in \lpart (B)$ in the construction of $G_\varphi$ (analogue for the second partition).

We continue with a definition and an auxiliary lemma regarding $G_\varphi$.

\begin{definition}\label{def:wbis_gadget_partitioning}
	Given a Boolean formula $\varphi$ in conjunctive normal form with $n$ variables and $m$ clauses. We define a partitioning~$\{S_i\}_{i=0}^{2n+m}$ of $\calI(G_\varphi)$ in the following recursive manner:
	
	Initiating with $S_1=\{I\in\calI(G_\varphi)\mid v_1,\bar{v_1}\notin I\}$ we define for every $i \in [n]$
	\begin{itemize}
		%\item Let $S_1=\{I\in\calI(G_\varphi)\mid v_1,\bar{v_1}\notin I\}$;
		%\item $S_i=\{I\in\calI(G_\varphi)\setminus\bigcup_{t=1}^{i-1} S_{t}\mid v_i,\bar{v_i}\notin I\}$ and
		\item $S_i=\{I\in\calI(G_\varphi)\setminus\bigcup_{t=1}^{i-1} S_{t}\mid \Gamma_{G'_\varphi}(z_i) \cap I = \emptyset\}$ and
		\item $S_{n+i}=\{I\in\calI(G_\varphi)\setminus\bigcup_{t=1}^{n+i-1} S_{t}\mid \Gamma_{G'_\varphi}(w_i) \cap I = \emptyset\}$.
		%\item $S_{n+i}=\{I\in\calI(G_\varphi)\setminus\bigcup_{t=1}^{n+i-1} S_{t}\mid u_i,\bar{u_i}\notin I\}$.
	\end{itemize}
	Subsequently, for every $j \in [m]$ we define $S_{2n+j}=\{I\in\calI(G_\varphi)\setminus\bigcup_{t=1}^{2n+j-1} S_{t}\mid 
	\Gamma_{G'_\varphi}(y_j) \cap I = \emptyset\}$.
%		\item for $i\in[m]$, let $S_{2n+i}=\{I\in\calI(G_\varphi)\setminus\bigcup_{j=1}^{2n+i-1} S_{j}\mid 
%		\Gamma_{G_\varphi}(c_i)\notin I\}$;
	Finally, let $S_{0}=\calI(G_\varphi)\setminus \bigcup_{t=1}^{2n+m} S_{t}$.
\end{definition}

In this sense, for every variable in $\varphi$, \emph{only} $S_i$ and $S_{n+i}$ contain all independent sets of $G_\varphi$, which do \emph{not} contain $u_i,\bar{u_i}$ and $v_i,\bar{v_i}$ respectively. Additionally, for every clause in $\varphi$, \emph{only} $S_{2n+j}$ contains all independent sets of $G_\varphi$, which do \emph{not} intersect with the neighbourhood of $y_j$ in $G'_\varphi$. Hence, any independent set $J \in \calI (B^t)$ yields an independent set in $S_t$.
Finally, $S_{0}$ contains any independent set~$I$, such that, for all $i\in[n]$, at least one of  $v_i,\bar{v_i}\in I$, at least one of  $u_i,\bar{u_i}\in I$ as well as, for all $j\in[m]$, $\Gamma_{G'_\varphi}(y_j)\cap I\neq \emptyset$. The following lemma allows us to focus on $S_0$. %\GL{previously it said "...or one of...". Additionally, the neighbourhood was unified with $I$.}
\begin{lemma}\label{lem:wbis_gadget_partitioning}
	Given a Boolean formula $\varphi$ in conjunctive normal form with $n$ variables and $m$ clauses. Let $G_\varphi = \bipG$ be the associated gadget graph and  $\{S_i\}_{i=0}^{2n+m}$ the partitioning of $\calI(G_\varphi)$ as defined in Definition~\ref{def:wbis_gadget_partitioning}. Then, for every $i\in[2n+m]$ 
	\[
		\sum_{I\in S_i}\lweight^{|\lpart\cap I|}\rweight^{|\rpart\cap I|}\equiv 0\pmod p.
	\]
\end{lemma}
\begin{proof}
	We fix $i\in[2n+m]$ and commence by defining the relation $\sim_i$. Given two independent sets $I,I'\in S_i$, then $I\sim_i I'$ if $I\setminus V(B^i)=I'\setminus V(B^i)$. That is, $I$ and $I'$ only differ in the vertices of $B^i$. We observe that $\sim_i$ is an equivalence relation yielding the $\sim_i$-equivalence class of $I$ denoted $\eqclass{I}_i$. Thus, the classes $\eqclass{I}_i$ partition the independent sets in $S_i$.
	
	Let $J_1\dots J_s$ be representatives from each $\sim_i$-equivalence class. We obtain
	\begin{equation*}
		\sum_{I\in S_i} \lweight^{|\lpart\cap I|} \rweight^{|\rpart \cap I|}=\sum_{j=1}^s \sum_{I\in \eqclass{J_j}_i} \lweight^{|\lpart \cap I|} \rweight^{|\rpart \cap I|}.
	\end{equation*}
	Therefore, if for every $j \in [s]$ we have $\sum_{I\in \eqclass{J_j}_i} \lweight^{|\lpart \cap I|} \rweight^{|\rpart \cap I|} \equiv 0 \pmod p$ the proof is established.
	
	Let $J$ be one of the representatives $J_1\dots J_s$ with its associated equivalence class $\eqclass{J}_i$. We continue by studying the set $J_B= J\setminus V(B^i)$ of common vertices among the independent sets of $\eqclass{J}_i$. Let $x^i$ be the vertex of $B^i$ that is identified with one of the vertices of $G'_\varphi$ for the 
	construction of $G_\varphi$. Therefore, $x^i=v_\L^i$ if $i<n$, and $x^i=v_\R^i$ otherwise.
	%\agob{We might need to explain the 	equation a bit more.} 
	By Definition~\ref{def:wbis_gadget_partitioning} we observe that for any $I\in S_i$ no neighbour of $x_i$ outside 
	$B^i$ is in $I$. 
%	\GL{This is NOT true with the current definition. Would be true if $S_i$ are the independent sets such that the neighbours of $x_i$ are not in the independent set. E.g.: $S_1=\{I\in\calI(G_\varphi)\mid u_1,\bar{u_1}\notin I\}$ , therefore interchange $u$ and $v$?}
	Hence, any vertex in $B^i$ is eligible for a construction of an independent set in $\eqclass{J}_i$. Since $B^i$ is a bipartite graph and the assignment of vertices to their relative partition is conserved in the construction of $G_\varphi$ we obtain 
	\begin{align}\label{eq:is-into-eq-classes}
		\sum_{I\in \eqclass{J}_i} \lweight^{|\lpart\cap I|} \rweight^{|\rpart \cap I|} & = \lweight^{|\lpart\cap J_B|} \rweight^{|\rpart\cap J_B|}
		\sum_{I\in\calI(B^i)} \lweight^{|\lpart(B^i)\cap I|} \rweight^{|\rpart(B^i)\cap I|}\nonumber \\
		&= \lweight^{|\lpart\cap J_B|} \rweight^{|\rpart\cap J_B|} \wISet{B^i}.
	\end{align}
	We recall that each $B^i$ was chosen utilizing Lemma~\ref{lem:bip-gadget}, whose Property~$\mathit{1}$ in conjunction with \eqref{eq:is-into-eq-classes} yields the desired
	\begin{equation*}\label{eq:gadget-0}
		\sum_{I\in \eqclass{J}_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|} \equiv 0\pmod p.
	\end{equation*}

%	Finally, let $J_1\dots J_s$ be representatives from each $\sim_i$-equivalence class. We obtain due to~\eqref{eq:gadget-0} the desired result
%	\begin{equation*}
%		\sum_{I\in S_i} \lweight^{|\lpart\cap I|} \rweight^{|\rpart \cap I|}=\sum_{j=1}^s \sum_{I\in \seqclass{J_j}_i} \lweight^{|\lpart \cap I|} \rweight^{|\rpart \cap I|} \equiv 0 \pmod p.
%	\end{equation*}
	%The above display equation combined with~\eqref{eq:gadget-0} proves the claim.	
\end{proof}
%Note that, for each $i\in[n]$, $z_i\in V_L(G_\varphi)$ and $v_L^i\in V_L(B)$ and, similarly, $w_i\in V_R(G_\varphi)$ and $v_R^{n+i}\in V_R(B)$. 
%This ensures that the identified vertices are on the same side of the bipartition. For each $j\in[m]$ identify $c_j$ 
%with $v_R^{2n+j}$, and again, for each $j\in[m]$, $c_j\in V_R(G_\varphi)$ and $v_R^{2n+i}\in V_R(B)$. This 
%concludes the construction of $G_\varphi$.

\begin{theorem}\label{thm:wbis-hardness}
	Let $p$ be a prime and let $\lweight$, $\rweight \in\zp$. If $\lweight \equiv 0 \pmod p$ or $\rweight \equiv 0 \pmod p$ then \pbislr{\lweight}{\rweight} is computable in polynomial time. Otherwise, \pbislr{\lweight}{\rweight} is \numpp{}-complete.
\end{theorem}
\begin{proof}
	The first statement is a direct consequence of Proposition~\ref{prop:BIS_easy_cases}. Therefore, let $\lweight, \rweight \in\zsp$.
	We are going to show hardness for \pbislr{\lweight}{\rweight} by establishing a Touring reduction from \numpsat{}, which is known to be \numpp{}-complete.
	\agob{citation of the \numpp{} completeness of SAT}
	
	Let $\varphi$ be a Boolean formula in conjunctive normal form, with $n$ variables and $m$ clauses. 
	We will show that the constructed bipartite graph $G_\varphi = \bipG$ satisfies $\wISet{G_\varphi}\equiv K |\sat(\varphi)|\pmod p$, where 
	$K=(\lweight \rweight)^n \left((\lweight+1)^{-1} -1\right)^n$ $\left((\rweight+1)^{-1} -1\right)^{n+m}\not\equiv0\pmod p$.

%	We construct $G_\varphi$ in two stages (see Figure \agob{make a picture}). We first construct the graph $G'_\varphi$. 
%	Let $\var(\varphi)=\{x_1\dots x_n\}$ be the set of variables of $\varphi$ and let $\clause(\varphi)=\{c_1,\dots,c_m\}$ 
%	be the set of clauses of $\varphi$. For every variable of~$\varphi$, $G'_\varphi$ has three vertices in its left part 
%	and three in its right part, and for every clause of~$\varphi$, $G'_\varphi$ has a vertex in its right part. That is, 
%	$V_L(G'_\varphi)=\{v_i,\bar{v_i},z_i\mid i\in[n]\}$, $V_R(G'_\varphi)=\{u_i,\bar{u_i},w_i\mid i\in[n]\}\cup\{c_i\mid 
%	i\in[m]\}$. 
%	$G'_\varphi$, for each $i\in[n]$, has the edges forming the cycle $v_iu_iz_i\bar{u_i}\bar{v_i}w_iv_i$, and 
%	the edges connecting $v_i$ with $c_j$, if $x_i$ appears in clause $c_j$ non-negated, and the edges connecting the 
%	$\bar{v_i}$ with $c_j$, if $x_i$ appears in clause $c_j$ negated. That is,
%	$E(G'_\varphi)=\{(v_i,u_i),(\bar{v_i},\bar{u_i}),(v_i,w_i),(\bar{v_i},w_i),\}$. Note that there are no the edges 
%	among the vertices of each part.
%
%Now we describe how to obtain~$G_\varphi$ from~$G'_\varphi$. Apply Lemma~\ref{lem:bip-gadget} to obtain the graph 
%$B$. $G_\varphi$ contains a copy of $G'_\varphi$ together with $2n+m$ disjoint copies of $B$, call each 
%\agob{we should use a similar notation with my thesis when adding multiple copies of a gadget} copy~$G^i_\Gamma$. Now 
%for each $i\in[n]$ identify $z_i$ with $v_L^i$, and $w_i$ with $v_R^{n+i}$. Note that, for each $i\in[n]$, $z_i\in 
%V_L(G_\varphi)$ and $v_L^i\in V_L(B)$ and, similarly, $w_i\in V_R(G_\varphi)$ and $v_R^{n+i}\in V_R(B)$. 
%This ensures that the identified vertices are on the same side of the bipartition. For each $j\in[m]$ identify $c_j$ 
%with $v_R^{2n+j}$, and again, for each $j\in[m]$, $c_j\in V_R(G_\varphi)$ and $v_R^{2n+i}\in V_R(B)$. This 
%concludes the construction of $G_\varphi$.

%\agob{this itemization looks horrible we need to fix it}
%We define a partitioning~$\{S_i\}_{i=0}^{2n+m}$ of $\calI(G_\varphi)$.
%\begin{itemize}
% \item Let $S_1=\{I\in\calI(G_\varphi)\mid v_1,\bar{v_1}\notin I\}$;
% \item for $1\in[n]$, let $S_i=\{I\in\calI(G_\varphi)\setminus\bigcup_{j=1}^{i-1} S_{j}\mid v_i,\bar{v_i}\notin I\}$ and
% \item $S_{n+i}=\{I\in\calI(G_\varphi)\setminus\bigcup_{j=1}^{n+i-1} S_{j}\mid u_i,\bar{u_i}\notin I\}$;
% \item for $i\in[m]$, let $S_{2n+i}=\{I\in\calI(G_\varphi)\setminus\bigcup_{j=1}^{2n+i-1} S_{j}\mid 
%\Gamma_{G_\varphi}(c_i)\notin I\}$;
% \item finally, let $S_{0}=\calI(G_\varphi)\setminus \bigcup_{j=1}^{2n+m} S_{j}$.
%\end{itemize}
%Thus, $S_{0}$ contains the independent sets~$I$, such that, for all $i\in[n]$, at least one of  $v_i,\bar{v_i}\in I$ or 
%one of  $u_i,\bar{u_i}\in I$ and, for all $j\in[m]$, $\Gamma_{G_\varphi}(c_j)\cup I\neq \emptyset$.

	Based on the partitioning~$\{S_i\}_{i=0}^{2n+m}$ given by Definition~\ref{def:wbis_gadget_partitioning}, we obtain
	\begin{equation}\label{eq:is-partitioned}
		 \wISet{G_\varphi}=\sum_{i=0}^{2n+m}\sum_{I\in S_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}.
	\end{equation}

%We claim that for $i\in[2n+m]$, $\sum_{I\in S_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}\equiv 0\pmod p$. 
%To prove the claim, 
%fix $i\in[2n+m]$. Given two independent sets $I,I'\in S_i$, let $I\sim_i I'$ if $I\setminus V(B^i)=I'\setminus V(B^i)$, 
%and write $\eqclass{I}_i$ for the $\sim_S$-equivalence class of $I$.\agob{I think it is obvious here that it is an 
%equivalence class.} That is $I$ and $I'$ only differ in the vertices of $B^i$. The classes $\eqclass{I}_i$ partition 
%the independent sets in $S_i$.
%
%Let $J\in S_i$, let $J_B= J\setminus V(B^i)$, that is the set of common vertices among the independent sets of 
%$\seqclass{J}_i$. Let $x^i$ be the vertex of $B^i$ that is identified with one of the vertices of $G'_\varphi$ for the 
%construction of $G_\varphi$. That is $x^i=v_L^i$ if $i<n$, and $x^i=v_R^i$ otherwise.\agob{We might need to explain the 
%equation a bit more.} From the definition of $S_i$, we have, that for any $I\in S_i$, no neighbour of $x_i$ outside 
%$B^i$ is in $I$. We have, 
%\begin{align}\label{eq:is-into-eq-classes}
%\sum_{I\in \seqclass{J}_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|} & = w_L^{|V_L\cap J_B|}w_R^{|V_R\cap J_B|}
%\sum_{I\in\calI(B^i)} w_L^{|V_L(B^i)\cap I|}w_R^{|V_R(B^i)\cap I|}\nonumber \\
%&= w_L^{|V_L\cap J_B|}w_R^{|V_R\cap J_B|}Z_{w_L,w_R}(B^i).
%\end{align}
%Recall that~$B$ was chosen by applying Lemma~\ref{lem:bip-gadget}. From Property~1 of Lemma~\ref{lem:bip-gadget}
%and~\eqref{eq:is-into-eq-classes} we have,
%\begin{equation}\label{eq:gadget-0}
% \sum_{I\in \seqclass{J}_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|} \equiv 0\pmod p.
%\end{equation}
%
%Let $J_1\dots J_k$ be representatives from each $\sim_i$-equivalence class. We have,
%\begin{equation*}
% \sum_{I\in S_i}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}=\sum_{j=1}^k\sum_{I\in \seqclass{J_j}_i}w_L^{|V_L\cap 
%I|}w_R^{|V_R\cap I|}.
%\end{equation*}
%The above display equation combined with~\eqref{eq:gadget-0} proves the claim.

	By Lemma~\ref{lem:wbis_gadget_partitioning} every term of~\eqref{eq:is-partitioned} is equivalent to $0 \pmod p$ \emph{except} for the one regarding $S_0$. This yields
	\begin{equation}\label{eq:sum-only-0}
		  \wISet{G_\varphi)} \equiv \sum_{I\in S_{0}} \lweight^{|\lpart\cap I|}\rweight^{|\rpart\cap I|}.
	\end{equation}

	As in the proof of Lemma~\ref{lem:bip-gadget} we are going to use an equivalence relation $\sim_0$ along with the associated equivalence class $\eqclass{\cdot}_0$. Let $U=\{v_i,\bar{v_i},u_i,\bar{u_i}\mid i\in[n]\}$, for two independent sets $I,I'\in S_{0}$ we have $I\sim_0 I'$ if $I\cap U= I'\cap U$. That is, $I$ and $I'$ have the same assignment regarding $U$. Let $J_1\dots J_\ell$ be representatives from each $\sim_0$-equivalence class. We obtain
	\begin{align}\label{eq:wbis_partitioning_S0}
		\sum_{I\in S_{0}} \lweight^{|\lpart\cap I|}\rweight^{|\rpart\cap I|}& = \sum_{i=1}^\ell\sum_{I\in \seqclass{J}_0} \lweight^{|\lpart\cap I|} \rweight^{|\rpart\cap I|}.
	\end{align}

	Let $I \in \eqclass{J_j}_0$ for a $j \in [\ell]$. Since $I \in S_0$ at least one of $v_i,\bar{v_i}$ and at least one of $u_i,\bar{u_i}$ are in $I$. We observe that for each $i\in[n]$ both $(v_i,u_i)$ and $(\bar{v_i},\bar{u_i})$ are connected in $(G_\varphi)$. Therefore, either the pair $\{v_i,\bar{u_i}\} \subseteq I$ or the pair $\{\bar{v_i},u_i \} \subseteq I$. And consequently, for each $i \in [n]$ neither $v_\L^i$ nor $v_R^{n+i}$ can be in $I$. Furthermore, for each $j\in[m]$ there exists at least one vertex $y\in\Gamma_{G_\varphi}(y_j)$ with $y\in I$. Hence, for each $j \in [m]$ the vertex $y_j=v_R^{2n+j}$ cannot be in $I$.

	We deduce that $I$ contains exactly $n$ vertices from $V_L(G'_\varphi)$ and exactly $n$ vertices from 
	$V_L(G'_\varphi)$. Moreover, each graph $B^i$ is a copy of the graph $B$ and the vertex $v_L^i$, $v_R^i$ if $i > n$ respectively, is a cut vertex in $G_\varphi$. There are $n$ copies of $B$ with $v_L$ identified with a vertex in $G'_\varphi$ and $n+m$ copies of $B$ with $v_R$ identified with a vertex in $G'_\varphi$. This yields
	\begin{align*}%\label{eq:equiv-class-0}
		\sum_{I\in \seqclass{J_j}_0} \lweight^{| \lpart \cap I|} \rweight^{|\rpart \cap I|}=
		(\lweight \rweight)^n & \left(\sum_{I\in\calI(B-v_\L)} \lweight^{|\lpart(B-v_\L)\cap I|} \rweight^{|\rpart(B-v_\L)\cap I|}\right)^n \nonumber \\
		&\left(\sum_{I\in\calI(B-v_\R)} \lweight^{|\lpart(B-v_\R)\cap I|} \rweight^{|\rpart(B-v_\R)\cap I|}\right)^{n+m}.
	\end{align*}

	Since $B$, $B-v_\L$ and $B - v_\R$ are bipartite graphs we obtain
	\begin{equation*}
		\sum_{I\in \seqclass{J}_0}\lweight^{|\lpart\cap I|} \rweight^{|\rpart\cap I|}=(\lweight \rweight)^n 
		\left(\wISet{B-v_\L}\right)^n \left(\wISet{B-v_\R}\right)^{n+m}.
	\end{equation*}

	We recall that $B$ was chosen due to Lemma~\ref{lem:bip-gadget}, whose Property~$\mathit{2}$ and Property~$\mathit{3}$ simplify the above equation to
	\begin{align}\label{eq:equiv-class-0-is-K}
		\sum_{I\in \seqclass{J}_0}\lweight^{|\lpart\cap I|} \rweight^{|\rpart\cap I|}& \equiv (\lweight \rweight)^n \left((\lweight+1)^{-1} -1\right)^n
		\left((\rweight+1)^{-1} -1\right)^{n+m} \nonumber \\
		&\equiv  K\pmod p,
	\end{align}
	since $K$ was defined as $K=(\lweight \rweight)^n \left((\lweight+1)^{-1} -1\right)^n$ $\left((\rweight+1)^{-1} -1\right)^{n+m}$.

	Combining \eqref{eq:equiv-class-0-is-K} and \eqref{eq:wbis_partitioning_S0} in conjunction with \eqref{eq:sum-only-0} we derive
	\begin{align}\label{eq:sum-of-K}
		\wISet{G_\varphi} \equiv \sum_{i=1}^\ell K \pmod p.
	\end{align}

	We will conclude the proof by constructing a bijection between the $\sim_0$-equivalence classes and the satisfying assignment of $\varphi$.
	
	For every equivalence class $\eqclass{J_j}_0$ with $j \in [\ell]$ we define the set of common vertices in $\eqclass{J_j}_0$ as $U_j=\bigcap_{I\in\seqclass{J_j}_0}I$. We recall by the definition of $\sim_0$ that the set $U_j$ is precisely for every $i \in [n]$ either the pair $\{v_i, \bar{u_i}\}$ or the pair $\{\bar{v_i}, u_i\}$ shared by all sets in $\eqclass{J_j}_0$. Hence, $U_i$ contains exactly $n$ such pairs of vertices.
	
	Given a satisfying assignment $a$ for $\varphi$, this assignment gives rise to the set 
	\[
		U_a= \bigcup_{i \in [n]} \{v_i,\bar{u_i}\mid \textrm{if $x_i$ is set ``true'' 
			in } a\}\cup\{\bar{v_i},u_i\mid \textrm{if $x_i$ is set ``false'' in } a\}
	\]
	and we map $a$ to the $\eqclass{J_j}$ with $U_j=U_a$.
	
	Vice versa, given an equivalence class~$\eqclass{J_j}$ utilizing $U_j$ we obtain an assignment~$a_j$ 
	for~$\varphi$ by
	\[
		\forall i \in [n] ,\quad x_i \mapsto 
		\begin{cases}
			\mathrm{true } , \quad \mathrm{if } \{v_i, \bar{u_i}\} \subseteq U_j; \\
			\mathrm{false } , \quad \mathrm{if } \{\bar{v_i},u_i\} \subseteq U_j.
		\end{cases}
	\]
	We observe that each $\eqclass{J_j}_0$ yields a unique assignment $a_j$. In order to show that it is a satisfying assignment it suffices to show that each clause of $\varphi$ is satisfied when we apply $a_j$.
	
	Given an independent set $I\in \eqclass{J_j}_{0}$, for each clause $c_s$ of $\varphi$ there exists at least one vertex $y \in \Gamma_{G'_\varphi}(y_j)$ with $y\in I$. Due to the construction of $G_\varphi$ this vertex $y$ is either $v_i$, if $x_i$ appears non-negated in the clause $c_s$, or $\bar{v_i}$, if $x_i$ appears negated in the clause $c_s$. Hence, $a_j$ satisfies $c_s$ at least once.
	
	We deduce that there are $\ell$ satisfying assignments of $\varphi$ and by \eqref{eq:sum-of-K}
	\[
		\wISet{G_\varphi}\equiv K|\sat(\varphi)|\pmod p,
	\]
	which establishes the theorem.
%Let $U=\{v_i,\bar{v_i},u_i,\bar{u_i}\mid i\in[n]\}$. For $I,I'\in S_{0}$, let $I\sim_0 I'$ if $I\cap U= I'\cap U$ and 
%write $\eqclass{I}_0$ for the $\sim_0$-equivalence class of $I$. By definition, $S_{0}$ contains independent sets~$I$, 
%such that for each $i\in[n]$, at least one of $v_i,\bar{v_i}$ is in $I$ and at least one of $u_i,\bar{u_i}$ are in $I$. 
%Since for each $i\in[n]$ both $(v_i,u_i)\in E(G_\varphi)$ and $(\bar{v_i},\bar{u_i})\in E(G_\varphi)$, $S_{0}$ contains 
%independent sets~$I$, such that for each $i\in[n]$, either the pair $v_i,\bar{u_i}\in I$ or the pair $\bar{v_i},u_i\in 
%I$. Furthermore, for each $I\in S_{0}$, for each $i\in[m]$, there exists at least one vertex 
%$y\in\Gamma_{G_\varphi}(c_i)$, with $y\in I$. \agob{maybe the $x_i'$ should be defined globally?-- That means we might 
%have to pull the definition of $G_\varphi$ outside the lemma}
%Let, again, $x^i$ be the vertex of $B^i$ that is identified with one of the vertices of $G'_\varphi$ for the 
%construction of $G_\varphi$. That is $x^i=v_L^i$ if $i<n$, and $x^i=v_R^i$ otherwise. Thus, for every $I\in S_0$, for 
%every $i\in[2n+m]$, $x_i\notin I$. Fix $J\in S_0$, we have,
%\begin{align}\label{eq:equiv-class-0}
% \sum_{I\in \seqclass{J}_0}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}=
%(w_Lw_R)^n & \left(\sum_{I\in\calI(B-v_L)}w_L^{|V_L(B-v_L)\cap I|}w_R^{|V_R(B-v_L)\cap 
%I|}\right)^n \nonumber \\
%&\left(\sum_{I\in\calI(B-v_R)}w_L^{|V_L(B-v_R)\cap I|}w_R^{|V_R(B-v_R)\cap 
%I|}\right)^{n+m}.
%\end{align}
%Every independent set~$J\in S_0$ contains exactly $n$ vertices from $V_L(G'_\varphi)$ and exactly $n$ vertices from 
%$V_L(G'_\varphi)$, hence the factor $(w_Lw_R)^n$ in the right-hand side of~\eqref{eq:equiv-class-0}. Furthermore, 
%during the construction of $G_\varphi$ from $G'_\varphi$, $n$ copies of $B$ are added, where for each such copy, $v_L$ 
%is a cut vertex and $n+m$ copies of $B$ are added, where for each such copy, $v_R$ is a cut vertex. The latter explains 
%the rest of the factors in the right-hand side of~\eqref{eq:equiv-class-0}.

%Since $B$, $B-v_\L$ and $B - v_\R$ are bipartite graphs we obtain
%\begin{equation*}
% \sum_{I\in \seqclass{J}_0}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}=(w_Lw_R)^n 
%\left(Z_{w_L,w_R}(B-v_L)\right)^n\left(Z_{w_L,w_R}(B-v_R)\right)^{n+m}.
%\end{equation*}
%
%We recall that $B$ was chosen due to Lemma\ref{lem:bip-gadget}, whose Property~$\mathit{2}$ and Property~$\mathit{3}$ simplify the above equation to
%\begin{align}\label{eq:equiv-class-0-is-K}
% \sum_{I\in \seqclass{J}_0}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}& \equiv (w_Lw_R)^n \left((w_L+1)^{-1} -1\right)^n
%\left((w_R+1)^{-1} -1\right)^{n+m} \nonumber \\
%& \equiv  K\pmod p,
%\end{align}
%since $K=(w_Lw_R)^n \left((w_L+1)^{-1} -1\right)^n$ $\left((w_R+1)^{-1} -1\right)^{n+m}$.

%Let $J_1\dots J_\ell$ be representatives from each $\sim_0$-equivalence class. We have,
%\begin{align}\label{eq:sum-of-K}
% \sum_{I\in S_{0}}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}& = \sum_{i=1}^\ell\sum_{I\in \seqclass{J}_0}w_L^{|V_L\cap 
%I|}w_R^{|V_R\cap I|} \nonumber \\
%\equiv\sum_{i=1}^\ell K \pmod p,
%\end{align}
%where the equivalence holds from~\eqref{eq:equiv-class-0-is-K}.

%We will show that there exists a bijection from the satisfying assignments of $\varphi$ to the $\sim_0$-equivalence 
%classes of $S_0$. Recall the definition of $\sim_0$ and recall that $S_{0}$ contains the independent sets~$I$, such 
%that for each $i\in[n]$, either the pair $v_i,\bar{u_i}\in I$ or the pair $\bar{v_i},u_i\in I$. Let $J_1\dots J_\ell$ be 
%representatives from each $\sim_0$-equivalence class and for $j\in[\ell]$, let $U_j=\bigcap_{I\in\seqclass{J_j}_0}I$. 
%Notice that each $U_i$ contains exactly $n$ such pairs of vertices. 
%
%Given a satisfying assignment $a$ for $\varphi$, let $U_a=\{v_i,\bar{u_i}\mid i\in[n]\textrm{ and $x_i$ is set ``true'' 
%in } a\}\cup\{\bar{v_i},u_i\mid i\in[n]\textrm{ and $x_i$ is set ``false'' in } a\}$. The bijection maps $a$ to 
%the $\eqclass{J_j}$ with $U_j=U_a$. Vice versa, given an equivalence class~$\eqclass{J_j}$, we obtain an assignment~$a$ 
%for~$\varphi$ as follows. For each $i\in[n]$, set $x_i$ to ``true'' if $v_i,\bar{u_i}\in U_j$, otherwise, 
%$\bar{v_i},u_i\in U_J$, therefore set $x_i$ to ``false''. Since, for each $I\in S_{0}$, and for each $j\in[m]$, there 
%exists at least one vertex $y\in\Gamma_{G_\varphi}(c_i)$, with $y\in I$, we know that every clause of $\varphi$ 
%contains at least a positive literal, hence $a$ is a satisfying assignment of $\varphi$.
%
%Thus, there are $\ell$ satisfying assignments of $\varphi$ and we can write~\eqref{eq:sum-of-K} as follows.
%\[\sum_{I\in S_{0}}w_L^{|V_L\cap I|}w_R^{|V_R\cap I|}\equiv K|\sat(\varphi)|\pmod p.\]
%By~\eqref{eq:sum-only-0}, we have,
%\[Z_{w_L,w_R}(G_\varphi)\equiv K|\sat(\varphi)|\pmod p,\]
%which concludes the proof of the lemma.
\end{proof}


==> cspandspinsys.tex <==
\subsection{Preliminaries}

As in the previous chapter, graphs are undirected and have no parallel edges or self-loops. Multigraphs are also 
undirected but they may have parallel edges and may have (multiple) self-loops. We will also use partially labelled 
graphs and 
graphs with distinguished vertices which we introduced in Section~\ref{sec:pinning-prelim}.
We use $\Gamma_H(v)$ to denote the set of neighbours of vertex~$v$ in~$H$ and $\deg_H(v)$ to denote the degree of~$v$ 
in 
$H$. 
%A path~$P$ is a graph with vertex set $V(P)$ and edge set $E(P)$. However, where convenient, we specify~$P$ by simply listing the vertices of the path, in order. We use $\dist_H(u,v)$ to denote the length of a shortest path from~$u$ to~$v$ in~$H$.

\subsection{Two-spin systems}
\label{sec:spins-for-trees}

Let $G$ be a multigraph as in Definition \ref{}. Given a non-zero integer $k$ and $\gamma \in \zk$ the corresponding partition function is defined by
\[ \gspin(G)=\quad\sum_{\sigma: V(G)\rightarrow\{0,1\}}\gamma^{c(\sigma)}, \]
where for an assignment $\sigma$ we denote by $c(\sigma)$ the number of $(u,v) \in E(G)$ with $\sigma(u)=\sigma(v)=1$. Note that $u$ may equal $v$, such that potential self-loops are included.

\smallskip
By $\kpart$ we denote the problem of computing from a given multigraph $G$ as input the value of $\gspin(G) \pmod k$ as output. In the following we identify values of $k$ and $\gamma$, for which this is $\nkp$-hard.

For this, we view $\kpart$ as $\pcsp(\{F\})$, where $F$ is a Boolean binary function into the integers.
Recall that for $m, k\in\posints$ and a set of Boolean functions $\calF=\{f_1,\ldots,f_m\}$, where for each $j\in[m]$, $f_j:\{0,1\}^{r_j}\rightarrow \zk$ and $r_j\in\posints$ the expression $\kcsp[k](\calF)$ denotes the problem of computing from a finite set of constraints over Boolean variables $x_1,\dots,x_n$ of the form $f_j(x_{i_{j,1}}, 
x_{i_{j,2}},\dots,x_{i_{j,r_j}})$ as input the output $\sum_{x_1,\dots,x_n\in\{0,1\}}\prod_j f_j(x_{i_{j,1}}, x_{i_{j,2}},\dots,x_{i_{j,r_j}})\pmod k$.

The complexity of $\kcsp[k]$ has been studied by \cite{guo2011complexity}. We employ two of their hardness results in case $\calF$ consists of a single binary function $F:\{0,1\}^2\rightarrow\ints$, also \emph{expressed by a matrix} 
$A = \left[\begin{smallmatrix}
a & b\\
c & d
\end{smallmatrix}\right]$,
where for $i,j\in\{0,1\}$, $A_{i,j}=F(i,j)$.
In case $b=c$ we call $F$ symmetric and simply write $[a,b,d]$.

The results of interest read as follows, where the first one is a corollary of a result of \cite[Theorem~4.11]{Fab08}.

\begin{lemma}[\cite{guo2011complexity}, Corollary~2.1] \label{lem:csp-hard-IS}
If $F$ is one of the symmetric Boolean binary functions expressed by $[1,1,0]$ and $[0,1,1]$, then for all integers $k$, $\kcsp[k](\{F\})$ is $\nkp$-hard.
\end{lemma}

\begin{lemma}[\cite{guo2011complexity}, Lemma~3.6]\label{lem:csp-hard-p}
Let $p$ be a prime and let $F:\{0,1\}^2\rightarrow\zp$ be the Boolean binary function expressed by $\left[\begin{smallmatrix} a & b\\ c & d \end{smallmatrix}\right]$
with $abcd\not\equiv0\pmod p$ and $a^2d^2\not\equiv b^2c^2\pmod p$.
Then $\pcsp(\{F\})$ is $\numpp$-hard.
\end{lemma}

Now we come to state our first observation regarding the hardness of $\kpart$.

\begin{lemma}\label{cor:spin-unary}
For every prime~$p$ and $\gamma\in\zp$ with $\gamma^2\not\equiv 1\pmod p$, $\gpart$ is $\numpp$-hard.
\end{lemma}
\begin{proof}
$\kpart$ is equivalent to $\pcsp(\{F\})$, where $F$ is 
the symmetric Boolean binary function expressed by $[1,1,\gamma]$, i.e. $F(0,0)=F(0,1)=F(1,0)=1$ and $F(1,1)=\gamma$.
More precisely, for an input multigraph $G$ consider $n:=|V(G)|$, i.e., $V(G)=\{v_1,\ldots,v_n\}$ and all $i,j \in [n]$ with $(v_i,v_j)\in E(G)$ yield a contraint $F(x_i,x_j)$.

If $\gamma\equiv0\pmod p$ then, by Lemma \ref{lem:csp-hard-IS} \gpart{} is $\numpp$-hard.
Otherwise, $\gamma\not\equiv0\pmod p$ and \gpart{} is $\numpp$-hard by Lemma\ref{lem:csp-hard-p}.
\end{proof}


\iffalse
We consider the following two-spin model which applies to spin systems on multigraphs. The model has two parameters, a 
prime number~$p$ and an integer $\gamma\in\zk$. A configuration $\sigma: 
V(G)\rightarrow\{0,1\}$ is an assignment of the two spins ``0'' and ``1'' to the vertices of $G$. Let $c(\sigma)$ 
denote 
the 
number of edges $(u,v)$ of $G$ with $\sigma(u)=\sigma(v)=1$. note that it may be $u=v$, so $c(\sigma)$ also includes 
the number of self-loops~$(v,v)$ of~$G$ with $\sigma(v)=1$. The partition function of the model is given by:

\[\gspin(G)=\!\!\!\!\sum_{\sigma: V(G)\rightarrow\{0,1\}}\!\!\!\!\gamma^{c(\sigma)}.\]

Formally, we are interested in the following modular counting problem.

\begin{problem}\label{defn:spins}
\begin{description}
\item \emph{Name.} \kpart.
\item \emph{Parameter.} $k\in\posints$ and $\gamma\in\zk$.
\item \emph{Input.} A multigraph $G$.
\item \emph{Output.} $\gspin(G) \pmod k$.
\end{description} 
\end{problem}

We will identify values of the parameters $k$ and $\gamma$, for which \kpart{} is $\nkp$-hard, to use it as a starting 
point for the reductions in Section~\ref{sec:p-gadgets}. To do so, we need to 
define the Boolean constraint satisfaction problem.

\begin{problem}\label{prb:pcsp}
\begin{description}
\item \emph{Name.} $\kcsp[k](\calF)$.
\item \emph{Parameter.} $k\in\posints$ and a set of Boolean functions $\calF=\{f_1\dots f_m\}$, where for each 
$j\in[m]$, $f_j:\{0,1\}^{r_j}\rightarrow \zp$ and $r_j\in\posints$.
\item \emph{Input.} A finite set of constraints over Boolean variables $x_1\dots x_n$ of the form \\ $f_j(x_{i_{j,1}}, 
x_{i_{j,2}},\dots,x_{i_{j,r_j}})$.
\item \emph{Output.} $\sum_{x_1,\dots,x_n\in\{0,1\}}\prod_j f_j(x_{i_{j,1}}, x_{i_{j,2}},\dots,x_{i_{j,r_j}})\pmod k$.
\end{description}
\end{problem}


The complexity of $\kcsp[k]$ has been studied by Guo et al.~\cite{GHLX11}. We are interested in two of their 
hardness results~\cite[Corollary~2 and Lemma~11]{GHLX11}, which will give us the cases for which \gpart{} is 
hard. Before we state their results we define the following.

\begin{definition}\label{defn:function-matrix}
 We say that a Boolean binary function~$F:\{0,1\}^2\rightarrow\ints$ is \emph{expressed by the matrix} 
$A=\left[\begin{smallmatrix}
                                             a & b\\
                                             c & d
                                            \end{smallmatrix}\right]$ if for $i,j\in\{0,1\}$, $F(i,j)=A_{i,j}$.
\end{definition}

The first result of Guo et al. we will use \cite[Corollary~2.1]{GHLX11} is a corollary of a result of 
Faben~\cite[Theorem~4.11]{Fab08}.

\begin{lemma}[Guo et al.]\label{lem:csp-hard-IS}
 Let $F_1:\{0,1\}^2\rightarrow\{0,1\}$ be the Boolean binary function expressed by the matrix 
$A_1=\left[\begin{smallmatrix}
                                             1 & 1\\
                                             1 & 0
                                            \end{smallmatrix}\right]$ and let $F_2:\{0,1\}^2\rightarrow\{0,1\}$ be the 
Boolean binary function expressed by the matrix $A_2=\left[\begin{smallmatrix}
                                             0 & 1\\
                                             1 & 1
                                            \end{smallmatrix}\right]$. For all integers $k$, $\kcsp[k](\{F_1\})$ and 
$\kcsp[k](\{F_2\})$ are $\nkp$-hard.
\end{lemma}

The other result of Guo et al. we will use is the following~\cite[Lemma~3.6]{GHLX11}.
\begin{lemma}[Guo et al.]\label{lem:csp-hard-p}
 Let $p$ be a prime and let $F:\{0,1\}^2\rightarrow\zp$ be the Boolean binary function expressed by the matrix 
$\left[\begin{smallmatrix}
                                             a & b\\
                                             c & d
                                            \end{smallmatrix}\right]$, where $abcd\not\equiv0\pmod p$ and 
$a^2d^2\not\equiv 
b^2c^2\pmod p$. $\pcsp(\{F\})$ is $\numpp$-hard.
\end{lemma}

From the definitions of \gpart{} and $\kcsp[p]$, we can see that \gpart{} is equivalent to $\pcsp(\{F\})$, where $F$ is 
the Boolean binary function expressed by the matrix $\left[\begin{smallmatrix}
                 1 & 1\\
                 1 & \gamma
                 \end{smallmatrix}\right]$.
We have the following.
\begin{corollary}\label{cor:spin-unary}
 For every prime~$p$ and $\gamma\in\zp$ with $\gamma^2\not\equiv 1\pmod p$, $\gpart$ is $\numpp$-hard.
\end{corollary}
\begin{proof}
 If $\gamma\equiv0\pmod p$ then, by Lemma~\ref{lem:csp-hard-IS} \gpart{} is $\numpp$-hard. Otherwise, 
$\gamma\not\equiv0\pmod p$ and \gpart{} is $\numpp$-hard by Lemma~\ref{lem:csp-hard-p}.
\end{proof}
\fi


% \chapter{Computing the partition function (modulo a prime) of a two-spin system with an external field}
% \label{chpt:spin-systems}

\subsection{Introduction: Spin Systems with field}

In this chapter we study the complexity of \glpart{}, the problem of computing (modulo a prime~$p$) the partition 
function of a two spin system on multigraphs with an external field. The two-spin model with external field has three 
parameters, a prime~$p$ and $\gamma,\lambda\in\{0,1,\dots p-1\}$.
A configuration $\sigma: V(G)\rightarrow\{0,1\}$ is 
an 
assignment of 
the 
two spins ``0'' and ``1'' to the vertices of $G$. Let $c(\sigma)$ denote the number of edges $(u,v)$ of $G$ with 
$\sigma(u)=\sigma(v)=1$ and let $\ell(\sigma)$ denote the number of vertices $u$ of $G$ with $\sigma(u)=0$. The 
partition function of the model is given by:

\[\spin{\gamma}{\lambda}(G)=\!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\!\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}.\]

Formally, \glpart{} is the following modular counting problem.

\begin{problem}\label{defn:spins-unary-weights}
\begin{description}
\item \emph{Name:} \glpart.
\item \emph{Parameter:} A prime~$p$ and $\gamma,\lambda\in\{0,1,\dots p-1\}$.
\item \emph{Input:} A multigraph $G$.
\item \emph{Output:} $\spin{\gamma}{\lambda}(G) \pmod p$.
\end{description} 
\end{problem}

In the definition above we could have $\gamma,\lambda\in\nints$, instead of restricting $\gamma,\lambda\in\{0,1,\dots 
p-1\}$. This 
does not weaken our results. To see this let $\gamma,\lambda\in\{0,1,\dots p-1\}$ and let $\gamma',\lambda'\in\nints$ 
with
$\gamma'\equiv\gamma\pmod p$ and $\lambda'\equiv\lambda\pmod p$. From the definition of $\spin{\gamma}{\lambda}$, for 
any graph $G$, $\spin{\gamma}{\lambda}(G)\equiv\spin{\gamma'}{\lambda'}(G)\pmod p$.

Recall that for a prime $p$, we let $i_p\in\{0,1,\dots p-1\}$, such that $i_p^2\equiv-1\pmod p$. For $p\geq3$ there can 
be either zero or two elements satisfying this definition. In the first case
consider the conditions involving $i_p$ redundant. In the second case the choice of $i_p$ has no effect, since we only rely on the property of being a square root of $-1$ in $\zp$. 
The main theorem of this chapter is the following.

{\renewcommand{\thetheorem}{\ref{thm:spin-field-main}}
\begin{theorem}
 Let $p$ be a prime and let $\gamma,\lambda\in\{0,1,\dots p-1\}$. \glpart{} is computable in polynomial time when one 
of 
the 
following holds.
 \begin{enumerate}
  \item $\lambda=0$.
  \item $\gamma=1$.
  \item $\gamma=-1$ and $\lambda\in\{0,\pm1,\pm i_p\}$.
 \end{enumerate}
Furthermore, \glpart{} is $\numpp$-complete when one of the following holds.
\begin{enumerate}
\setcounter{enumi}{3}
 \item $\lambda\not\equiv 0\pmod p$ and $\gamma\equiv 0 \pmod p$.
 \item $\lambda\not\equiv 0\pmod p$, $\gamma\not\equiv\pm1\pmod p$ and there exists an integer~$k$ with 
$\gamma^k\equiv\lambda\pmod p$.
 \item $\lambda\not\equiv 0\pmod p$, $\gamma\not\equiv\pm1\pmod p$ and $p<100$, where $p\neq41$.
\end{enumerate}
\end{theorem}}

The proof follows in the sections \ref{} and \ref{}.
Theorem~\ref{thm:spin-field-main} extends the results we have presented in Section~\ref{sec:spins-for-trees}, for the 
complexity of \gpart{} (Problem~\ref{defn:spins}), the problem of computing the partition function of a two 
spin system on multigraphs without an external field. As we saw in Section~\ref{sec:spins-for-trees} any 
instance multigraph~$G$ of \gpart{} can be seen as an instance of $\kcsp[p](\{F\})$, where $F$ is the binary function expressed by $[1,1,\gamma]$, $\gamma \in \zp$ and
the instance is given by the edge structure of $G$. Hence Corollary~\ref{cor:spin-unary} that describes the complexity of 
\gpart{} is an immediate corollary of the dichotomy theorem on the complexity of \kcsp{} by Guo et al.~\cite{GHLX11}.


Obviously, from the definitions of Problem~\ref{defn:spins} and Problem~\ref{defn:spins-unary-weights} \gpart{} 
is the special case of \glpart{} with $\lambda=1$. 
Like \gpart{}, the problem \glpart{} can interpreted as a special case of 
$\kcsp[p]$. More precisely, any instance multigraph~$G$ of \glpart{} can be seen as a restricted input of 
$\kcsp[p](\{F,U\})$, where $F$ is defined as above and applied corresponding to the edge structure, whereas $U$ denotes the unary Boolean function expressed by $[\lambda, 1]$, where $\lambda \in \zp$, applied to every variable.
In contrast to the equivalence of $\gpart{}$ and $\kcsp[p](\{[1,1,\gamma]\})$, our transformation of an input for  $\glpart{}$ to one for $\kcsp[p](\{[1,1,\gamma],[\lambda,1]\})$ is not surjective and thus only positive results transfer.

More precisely, if $\kcsp[p](\{E,U\})$ is tractable, so is every  
restricted input \glpart{}. So the polynomial cases of \glpart{} in Theorem~\ref{thm:spin-field-main} come directly 
from the dichotomy theorem of \cite{GHLX11}, Lemma 3.10 for the complexity of \kcsp{}. For the hardness results though 
that is not true in general, as hardness for $\kcsp[p](\{E,U\})$, does not imply hardness for \glpart{}.

To prove our hardness results we reduce \gpart{} to \glpart{} for various values of the parameter space. Our 
reductions, informally, work as follows: Let $G$ be the input multigraph for \gpart{}. We construct an input multigraph 
$G'$ for \glpart{} in the following way. Let $(J,x)$ be an ``appropriate'' gadget-multigraph with a distinguished 
vertex. Take the union of $|V(G)|$ disjoint copies of $(J,x)$ and a copy of $G$. For every vertex~$v$ of $G$, identify 
$x$ with $v$. By appropriate we mean that the gadget~$(J,x)$ cancels out the vertex weights in 
$\spin{\gamma}{\lambda}$ in the following way. The total ``weight'' contribution of $J$ to $\spin{\gamma}{\lambda}(J)$ 
when $x$ is mapped to ``0'' is 
equivalent to the total ``weight'' contribution of $J$ to $\spin{\gamma}{\lambda}(J)$ when $x$ is mapped to ``1''. 
Therefore $\spin{\gamma}{\lambda}(G')=k\left(\spin{\gamma}{\lambda}(J)\right)^{|V(G)|}\gspin(G)$, where $k$ is a 
constant. Since $J$ is a fixed graph, if we where able to compute $\gspin(G)$ we would be able to compute 
$\spin{\gamma}{\lambda}(G')$. Therefore, in order to prove hardness for \glpart{} it suffices to find appropriate 
gadgets $(J,x)$ for the values of the parameters $\gamma$, $\lambda$ and $p$.

To find appropriate gadgets, we also establish pinning for \glpart{}. The pinning we use for \glpart{} is similar to 
the pinning we used for \phcol{}: \pinnedglpart{} has as an input a multigraph $G$ and a pinning function 
$\tau:V(G)\rightarrow\{0,1\}$ and as output the value of partition function $\spin{\gamma}{\lambda}(G)$ (modulo~$p$) 
over 
all 
configuration that respect $\tau$. We show that \pinnedglpart{} reduces to \glpart{}. This allows us to use multigraphs 
$J$ that have vertices pinned to either ``0'' or ``1'' as gadgets, in order to show hardness for \glpart{}.

By using cliques as gadgets we can prove that \glpart{} is hard when $\lambda\not\equiv0\pmod p$ and $\gamma=0$. By 
using two vertices connected with~$k$ parallel edges where one of them is pinned to ``1'' as a gadget, we can show 
hardness for \glpart when $\lambda\not\equiv0\pmod p$, $\gamma\not\equiv\pm1\pmod p$ and $\gamma^k\equiv\lambda\pmod 
p$. Finally, using a combination of cliques, paths and the ``two vertices with $k$ parallel edges'' gadget we show that 
\glpart{} is hard for small primes when $\lambda\not\equiv0\pmod p$, $\gamma\not\equiv\pm1\pmod p$.


\subsubsection{Organisation}

In Section~\ref{sec:spins-field} we explain our choice of vertex weights. In Section~\ref{sec:spins-poly-cases} we give 
values of the parameters for which \glpart{} is computable in polynomial 
time. 

In Section~\ref{sec:spins-hard-cases} we show that for other values of the parameters, \glpart{} is 
$\numpp$-complete. More specifically in Section~\ref{sec:spins:pin} we establish pinning for \glpart{}. In 
Section~\ref{sec:spins:property} we identify a property for the gadgets we will use, in order to obtain hardness 
results. In Section~\ref{sec:spins:gadgets} we find appropriate gadgets for values of the parameter space.

Finally, in Section~\ref{sec:spins:summary} we tie all our results together in the main theorem of this section.

\subsection{Preliminaries}

In this chapter we only use multigraphs. For a multigraph $G$ and a subset of its edges $U\subseteq V$ we denote with 
$G[U]$ the sub-multigraph of $G$ induced by $U$. For a multigraph $G$ and $v\in V(G)$ we denote with $G-v$ the 
sub-multigraph of $G$ induced by $V\setminus\{v\}$. As with graphs we specify simple paths~$P$ by simply listing the 
vertices of the path, in order.

\smallskip

\noindent Let $\zp$ be the additive group of integers modulo~$p$. For a prime $p$ and an integer $k\in\zp$, when 
working in $\zp$ we will, sometimes, denote $p-k$ with $-k$.

\subsection{Vertex weights}
\label{sec:spins-field}

We defined \glpart{} so that vertices contribute a factor of $\lambda$ when they are mapped to ``0''. We can also 
consider the version of the problem when the unary weight comes from the vertices mapped to ``1''. Let $G$ be a 
multigraph, let $\sigma: V(G)\rightarrow\{0,1\}$ and let $\ell'(\sigma)=|V(G)|-\ell(\sigma)$, i.e. the number of 
vertices 
mapped to ``1'' by $\sigma$. Define

\[\spin{\gamma}{\lambda}'(G)=\!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\!\gamma^{c(\sigma)}\lambda^{\ell'(\sigma)}.\]

Let $p$ be a prime and let $\lambda^{-1}$ be the inverse of $\lambda$ in $\zp$. From the definitions of 
$\spin{\gamma}{\lambda}$, $\spin{\gamma}{\lambda}'$ and $\ell'$ we have,

\begin{align*}
(\lambda^{-1})^{|V(G)|}\spin{\gamma}{\lambda}(G)& \equiv (\lambda^{-1})^{|V(G)|} \!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\!\gamma^{c(\sigma)}\lambda^{\ell(\sigma)} & \pmod p \\
& \equiv\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\gamma^{c(\sigma)}(\lambda^{-1})^{|V(G)|-\ell(\sigma)}& \pmod p\\
&\equiv \!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\gamma^{c(\sigma)}(\lambda^{-1})^{\ell'(\sigma)}& \pmod p\\
&\equiv\spin{\gamma}{\lambda^{-1}}'(G). & \pmod p
\end{align*}

That is for any multigraph $G$, if we can compute $\spin{\gamma}{\lambda}(G)$ modulo a prime~$p$, then we can compute 
$\spin{\gamma}{\lambda^{-1}}'(G)$ modulo a prime~$p$. So classifying the complexity of \glpart{}, for every prime~$p$ 
and every $\lambda\in\zp$, is equivalent to determining the complexity of computing $\spin{\gamma}{\lambda^{-1}}'$ 
modulo~$p$. 


\subsection{Polynomial solvable cases}
\label{sec:spins-poly-cases}
As we have already mentioned in Section~\ref{sec:spins-for-trees}, Guo et al.~\cite{GHLX11} study the complexity of 
$\kcsp[k]$ and give a dichotomy theorem completely characterising its complexity. We will review the results 
of~\cite{GHLX11} and explain how they are relevant to identifying values of the parameters $\gamma$, $\lambda$ and $p$, 
for which \glpart{} is computable in polynomial time.

Recall definition~\ref{defn:function-matrix} of a Boolean binary function that is expressed by a matrix. To show the 
dichotomy for $\kcsp[k]$ Guo et al. define the classes of functions $\calP_k$ and $\calA_k$. 

\begin{definition}\label{defn:calP}
Let $\calU$ be the set of Boolean unary functions $f:\{0,1\}\rightarrow\ints$, let $F_1:\{0,1\}^2\rightarrow\{0,1\}$ be 
the 
Boolean binary function expressed by the matrix $\left[\begin{smallmatrix}
                 1 & 0\\
                 0 & 1
                 \end{smallmatrix}\right]$ and let $F_2:\{0,1\}^2\rightarrow\{0,1\}$ be the Boolean binary function 
expressed by 
the matrix $\left[\begin{smallmatrix}
                 0 & 1\\
                 1 & 0
                 \end{smallmatrix}\right]$.

Let $\calP$ contain functions of the form $\prod_i 
f_i(x_{i_1},\dots,x_{i_{r_i}})$, where  
$f_i\in\calU\cup\{F_1,F_2\}$. The functions of $\calP$ are also called product functions.
For an integer $k$, let $\calP_k=\{f:\{0,1\}^r\rightarrow\zp\mid f\equiv g\pmod k \textrm{, where }g\in\calP\}$.
\end{definition}

\begin{definition}\label{defn:calA}
 Let $X$ be an $r+1$ dimensional column vector $(x_1,\dots,x_r,1)$ of $\{0,1\}^{r+1}\!\!.$ For an integer $r'$, let $A$ 
be 
a $r'\times(r+1)$ Boolean matrix 
and let 
\[\chi_{AX}=\left\{\begin{array}{lc}
                  1 & \textrm{if } AX=0\\
                  0 & \textrm{otherwise.}
                 \end{array}\right.\]
$\calA_k$ contains the affine functions. That is, $\calA_k$ is the class of functions of the form 
\mbox{$\chi_{AX}\cdot (i_k)^{L_1(X)+\dots+L_m(X)}$}, where         
for $j\in[m]$, $L_j(X)$ is an indicator function $\chi_{\langle\alpha_j,X\rangle}$, $\alpha_j$ is an 
$(r+1)$-dimensional vector and the inner product $\langle\alpha_j,X\rangle$ is taken over $\mathbb{Z}_2$. 
\end{definition}

We are now ready to state the dichotomy result of Guo et al.~\cite[Lemma~3.10]{GHLX11} for 
$\kcsp[p]$.

\begin{lemma}[Guo et al.]\label{lem:kcsp-dichitomy}
 Let $p$ be an odd prime and let \calF{} be a class of functions mapping Boolean inputs to $\zp$. If 
$\calF\subseteq\calP_p$ or $\calF\subseteq\calA_p$, then $\kcsp[p](\calF)$ is computable in polynomial time. Otherwise 
$\kcsp[p](\calF)$ is $\numpp$-hard.
\end{lemma}

Let $E_\gamma$ be the function expressed by the matrix 
		 $\left[\begin{smallmatrix}
                 1 & 1\\
                 1 & \gamma
                 \end{smallmatrix}\right]$.
Additionally let $U_\lambda$ to be the unary function with $U_\lambda(0)=\lambda$ and $U_\lambda(1)=1$.
When $\lambda=1$, $\#_p Z_{\gamma,1}$ is equivalent to $\pcsp(\{E_\gamma\})$. In any other case \glpart{} is essentialy 
a restricted input of $\pcsp(\{E_\gamma,U_\lambda\})$, where the unary function $U_\lambda$ is applied to 
every variable of the input exactly once. When $\pcsp(\{E_\gamma,U_\lambda\})$ is computable in polynomial time then 
\glpart{} is computable in polynomial time, as it is a special case of $\pcsp(\{E_\gamma,U_\lambda\})$. So by 
Lemma~\ref{lem:kcsp-dichitomy} when $E_\gamma,U_\lambda\in\calP_p$ or when $E_\gamma,U_\lambda\in\calA_p$, we have that 
\glpart{} is computable in polynomial time.

\begin{table}
\[
 \begin{array}{c|c|c|c|c|c|c}
 x & y & L_1(X) & L_2(X) & L_3(X) & L_4(X) & L_1(X)+3L_2(X)+3L_3(X)+L_4(X)\\
 \hline
 \hline
 0 & 0 & 1 & 1 & 1 & 1 & 8\\
 \hline
 1 & 0 & 0 & 0 & 1 & 1 & 4\\
  \hline
 0 & 1 & 0 & 1 & 0 & 1 & 4\\
  \hline
 1 & 1 & 1 & 0 & 0 & 1 & 2\\
 \end{array}
\]

 \caption{The table for the values of the indicator functions $L_1,\dots,L_4$ as they appear in the proof 
of Lemma~\ref{lem:spin-poly}.}\label{tab:Ax}
\end{table}


\begin{lemma}\label{lem:spin-poly}
 Let $p$ be a prime. The following hold.
 \begin{enumerate}
 \item For all $\gamma\in\zp$, $\pspin{\gamma}{0}$ is computable in polynomial time.
 \item For all $\lambda\in\zp$, $\pspin{1}{\lambda}$ is computable in polynomial time.
 \item For $\lambda\in\{0,\pm1,\pm i_p\}$, $\pspin{-1}{\lambda}$ is computable in polynomial time.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $G$ be a multigraph. When $\lambda\equiv0\pmod p$, $\spin{\gamma}{0}(G)=\gamma^{|E(G)|}$, so (1) follows.

To show~(2) notice that $E_1\in\calP_p$ as $E_1$ is a product of two unary functions: $E_1(x,y)=g(x)g(y)$ with 
$g(x)=1$. For any $\lambda\in\zp$, $U_\lambda$ is a unary function, therefore a member of $\calP_p$. From 
Lemma~\ref{lem:kcsp-dichitomy}, $\pcsp(\{E_1,U_\lambda\})$ is computable in polynomial time and so is $\#_p
Z_{1,\lambda}$.

Now we will show~(3). Recall Definition~\ref{defn:calA} of $\calA_p$. Let $A=[0,0,0]$ and let $X=(x,y,1)$, so $AX=(0)$ 
and, therefore, $\chi_{AX}(x,y)=1$. Now let $\alpha_1=(1,1,1)$, $\alpha_2=(1,0,1)$, $\alpha_3=(0,1,1)$ and 
$\alpha_4=(0,0,1)$. So $L_1(x)\equiv x+y+1 \pmod2$, $L_2(X)\equiv x+1\pmod2$, $L_3(X)\equiv y+1\pmod2$ and $L_4(X)=1$. 
As we can see from Table~\ref{tab:Ax} $E_{-1}=\chi_{AX}\cdot i_p^{L_1(X)+3L_2(X)+3L_3(X)+L_4(X)}$, so 
$E_{-1}\in\calA_p$. 

We claim that when $\lambda\in\{0,1,i_p,-1,-i_p\}$, $U_\lambda\in\calA_p$. Let $X'=(x,1)$. Let $A_0=[0,0]$ and let 
$\alpha_5=(1,1)$. So $\chi_{A_0X'}(x)=1$ and $L_5(X)\equiv x+1\pmod2$. Therefore, 
$U_{i_p}=\chi_{A_0X'}\cdot i_p^{L_5(X')}$, $U_{-1}=\chi_{A_0X'}\cdot i_p^{2L_5(X')}$, $U_{-i_p}=\chi_{A_0X'}\cdot 
i_p^{3L_5(X')}$ and $U_1=\chi_{A_0X'}\cdot i_p^{4L_1(X')}$.
From the above and Lemma~\ref{lem:kcsp-dichitomy}, when $\lambda\in\{0,1,i_p,-1,-i_p\}$, $\pcsp(\{E_{-1},U_\lambda\})$ 
is 
computable in polynomial time and so is $\#_pZ_{-1,\lambda}$.
\end{proof}

\subsection{Hardness results}
\label{sec:spins-hard-cases}

In this section we will show values of the parameter space $(\gamma,\lambda,p)$ for which \glpart{} is hard to compute. 
Lemma~\ref{p:lem:ISP-hardness} below shows that \glpart{} is $\numpp$-hard for all primes $p$ when 
$\lambda\not\equiv0\pmod 
p$ and $\gamma\equiv0\pmod p$. Lemma~\ref{lem:lambda-generator-hardness} shows that when $\lambda\not\equiv 1\pmod p$ 
and $\lambda=\gamma^k\pmod p$, 
\glpart{} is $\numpp$-hard. Lemma~\ref{lem:small-primes-spin-hard} shows that, for all primes $p<100$, where $p\neq41$, 
when $\gamma^2\not\equiv 1\pmod p$ \glpart{} is $\numpp$-complete.

When $\lambda\not\in\{0,\pm1,\pm i_p\}$ the complexity of $\pspin{-1}{\lambda}$ remains unknown. We have, by
Lemma~\ref{lem:kcsp-dichitomy}, that $\kcsp[p](\{E_{-1},U_\lambda\})$ is hard.\footnote{$E_{-1}\notin\calP_p$ as 
it cannot 
be a multiple of $F_1$ or $F_2$ from Definition~\ref{defn:calP} and it cannot be a multiple of only unary functions. 
Also $U_\lambda\notin\calA_p$ as the functions in $\calA_p$ can only have values in $\{0,\pm1,\pm i_p\}$.} Since 
$\pspin{-1}{\lambda}$ is a 
restricted input for $\kcsp[p](\{E_{-1},U_\lambda\})$, hardness for $\kcsp[p](\{E_{-1},U_\lambda\})$ does not imply 
hardness for $\pspin{-1}{\lambda}$. $\pspin{-1}{1}$ is computable in polynomial time and a reduction similar to the 
reductions we present in this chapter would not give us hardness for $\pspin{-1}{\lambda}$.

\subsubsection{Pinning in two-spin systems}
\label{sec:spins:pin}

The gadgets we will use for our reductions from \gpart{} to \glpart{} will be multigraphs with 
vertices pinned to either ``0'' or ``1''. In the setting of \glpart{}, a \emph{pinning 
function}~$\tau$ of a multigraph~$G$ is a partial function from $V(G)$ to $\{0,1\}$. A vertex~$v$ in the domain of the 
pinning function is said to be \emph{pinned} or \emph{pinned to $\tau(v)$}. A 
\emph{partially pinned multigraph} $J=(G,\tau)$ consists of an \emph{underlying graph}~$G$ and a pinning
function~$\tau$ from $V(G)$ to~$\{0,1\}$. 

\begin{definition}\label{defn:respect-tau}
 Let $G$ be a multigraph and let $\tau:V(G)\rightarrow\{0,1\}$ be a pinning function of $G$. 
$R(G,\tau)=\{\sigma:V(G)\rightarrow\{0,1\}\mid \sigma(v)=\tau(v)\textrm{ for 
} v\in\dom(\tau)\}$ is the set of mappings that respect 
$\tau$. 
\end{definition}


Given a partially pinned multigraph $(G,\tau)$ 
we define $\spin{\gamma}{\lambda}^\tau(G)=\sum_{\sigma\in 
R(G,\tau)}\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}$.
The pinned version of \glpart{} is the following.

\probpar{\pinnedglpart.}
{A prime $p$ and $\gamma,\lambda\in\zp$.}
{A partially pinned multigraph $J=(G,\tau)$.}
{$\spin{\gamma}{\lambda}^\tau(G)\pmod p$.}
 
The following lemma shows that computing \glpart{} is at least as hard as computing \pinnedglpart{}.

\begin{lemma}\label{lem:spin-pin}
 For any prime $p$ \pinnedglpart{} reduces to \glpart{} under polynomial-time Turing reductions.
\end{lemma}
\begin{proof}
Let $J=(G,\tau)$ be an instance of \pinnedglpart{}. Let $V_0=\{v\in\dom(\tau)\mid \tau(v)=0\}$ be the set of  
variables pinned to ``0'' and $V_1=\dom(\tau)\setminus V_0$ the set of variables pinned to ``1''. 
$\spin{\gamma}{\lambda}^\tau(G)=\lambda^{|V_0|}\spin{\gamma}{\lambda}^\tau(G[V\setminus V_0])$ so it suffices to 
show that the lemma holds for instances with $V_0=\emptyset$. 

Let $E_1=E(G[V_1])$ be the set of edges of $G$ between the vertices of $V_1$. Let $G'$ be the sub-multigraph of $G$ 
where all the edges in $E_1$ have been deleted. 
$\spin{\gamma}{\lambda}^\tau(G)=\gamma^{|E_1|}\spin{\gamma}{\lambda}^\tau(G')$, so it suffices to show 
that the lemma holds for inputs 
$J$ where $E_1=\emptyset$.

Let $G''$ be the multigraph produced from $G$, by identifying all the vertices in $V_1$. Call this vertex $v_1$.  
By construction, $\spin{\gamma}{\lambda}^\tau(G)=\spin{\gamma}{\lambda}^\tau(G'')$. 
$\spin{\gamma}{\lambda}(G'')=\spin{\gamma}{\lambda}^\tau(G'')+\lambda\spin{\gamma}{\lambda}(G''-v_1)$ and the 
lemma follows.
\end{proof}


\subsubsection{Gadgets for two-spin systems}
\label{sec:spins:property}

In order to prove hardness for \glpart{}, we need to find gadgets which, by attaching to every vertex of $G$, will 
cancel out the weights of $\lambda$ that the vertices mapped to ``0'' contribute to the partition function. Our gadgets 
$(J,x)$ 
consist of a partially pinned multigraph~$J=(G,\tau)$ with a distinguished vertex $x\in V(G(J))$. Recall 
Definition~\ref{defn:respect-tau} of $R(G,\tau)$. To express the properties of the gadgets we will need the following 
definitions.

\begin{definition}\label{dfn:zero-one}
 Let $(J,x)$ be a partially pinned multigraph with a distinguished vertex. Let 
$G=G(J)$ and let $\tau=\tau(J):V(G(J))\rightarrow\{0,1\}$ be the 
pinning function of $J$, such that $x\notin\dom(\tau)$. We define

\[
\spin{\gamma}{\lambda}^{\tau,0}(G,x)=\sum_{\substack{\sigma\in 
R(G,\tau),\\ \sigma(x)=0}}\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}\quad\textrm{ and}
\]

\[
 \spin{\gamma}{\lambda}^{\tau,1}(G,x)=\sum_{\substack{\sigma\in 
R(G,\tau),\\ \sigma(x)=1}}\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}.
\]
\end{definition}

As in Theorem~\ref{p:thm:hardness-gadget} we will use the following notation to build partially pinned multigraphs
containing many copies of some subgraph. For any ``tag''~$T$ (which we will treat just as an arbitrary string) and any 
partially labelled multigraph~$J$, denote by $J^T$ a copy of~$J$ with every vertex $v\in V(G(J))$ renamed~$v^T\!$. 

\begin{definition}\label{dfn:g-gamma}
Given a multigraph $G$ and a partially pinned multigraph with a distinguished vertex 
$(J,x)$ we define $G \odot(J,x)$ to be the partially pinned multigraph constructed in the following way. Take a copy of 
$G$ together with the union of disjoint copies~$G^v(J)$ of~$G(J)$ for each $v\in V(G)$. For 
each vertex $v\in V(G)$ identify $v$ with~$x^v$. Let $\tau(G \odot(J,x))=\bigcup_{v\in V(G)}\tau(G^v(J))$.
\end{definition}

The following theorem shows that if we find an appropriate partially pinned multigraph with a distinguished vertex 
$(J,x)$, we can obtain hardness for \glpart{}.

\begin{lemma}\label{lem:gadget-condition}
Let $p$ be a prime and let $\gamma,\lambda\in\zp$, with $\gamma^2\not\equiv1\pmod p$ and $\lambda\not\equiv 0\pmod p$. 
If 
there exists a partially pinned multigraph with a distinguished vertex~$(J,x)$ and $\tau=\tau(J)$, such that 
$\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)\equiv\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)\not\equiv0\pmod p$, then 
\glpart{} is $\numpp$-hard. 
\end{lemma}
\begin{proof}
 We first show that $\pspin{\gamma}{1}$ reduces to \pinnedglpart{}. 
Let $G$ be the input of $\pspin{\gamma}{1}$ and let $(J,x)$ be a partially pinned multigraph with a
distinguished vertex, such that 
$\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)\equiv\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)\equiv A \pmod p$. 
Let $J'=G\odot(J,x)$ be the partially pinned graph, as in Definition~\ref{dfn:g-gamma}. $J'$ will 
be the input for \pinnedglpart{}. We denote $G'=G(J')$ and $\tau'=\tau(J')$.

For $\sigma,\sigma' \in R(G',\tau')$ we write $\sigma\sim_G\sigma'$ if $\sigma|_G=\sigma'|_G$. We 
also write $\eqclass{\sigma}_G$ for the $\sim_G$-equivalence class of $\sigma$. The classes $\eqclass{\sigma}_G$ 
partition the set of configurations of $J'$. For $\sigma\in R(G',\tau')$ we define 
$W(\eqclass{\sigma}_G)=\sum_{\sigma\in\seqclass{\sigma}_G}\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}$. Let 
$\sigma\in 
R(G',\tau')$, be a configuration of $G'$ that respects $\tau'$. $\sigma$ maps $\ell(\sigma|_G)$ 
vertices of $G$ to ``0'' and $V(G)-\ell(\sigma|_G)$ vertices of $G$ to ``1''. Therefore, 

\[W(\eqclass{\sigma}_G)= \gamma^{c(\sigma|_G)} \left(\!\!\sum_{\substack{\sigma'\in 
R(G(J),\tau(J)),\\ \sigma'(x)=0}}\!\!\!\gamma^{c(\sigma')}\lambda^{\ell(\sigma')} 
\right)^{\ell(\sigma|_G)}\left(\!\!\sum_{\substack{\sigma'\in 
R(G(J),\tau(J)),\\ \sigma'(x)=1}}\!\!\!\gamma^{c(\sigma')}\lambda^{\ell(\sigma')} 
\right)^{V(G)-\ell(\sigma|_G)}\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!.\quad \quad \quad \quad \]

From Definition~\ref{dfn:zero-one} we now have,
		      
\[W(\eqclass{\sigma}_G)= \gamma^{c(\sigma|_G)}
\big(\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)\big)^{\ell(\sigma|_G)}\big(\spin{\gamma}{\lambda}^{\tau,1} 
(G(J),x)\big)^{V(G)-\ell(\sigma|_G)}\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!.\]

By the choice of $J$, $\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)\equiv\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)\equiv 
A \pmod p$, so

\begin{equation}\label{eqn:weight-conf}
W(\eqclass{\sigma}_G) \equiv \gamma^{c(\sigma|_G)} A^{|V(G)|} \pmod p .
\end{equation}



Now let $\sigma_1\dots\sigma_k$ be representatives of the $\sim_G$-equivalence classes.
\begin{align*}
 \spin{\gamma}{\lambda}^\tau(G')& = \sum_{\sigma\in R(G',\tau')}\!\!\gamma^{c(\sigma)}\lambda^{\ell(\sigma)} \\
				      & =\sum_{i=1}^k\sum_{\sigma\in\seqclass{\sigma_i}_G }
\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}\\
				      & =\sum_{i=1}^k W(\eqclass{\sigma_i}_G) \\
                                      & \equiv A^{|V(G)|}\sum_{i=1}^k\gamma^{c(\sigma_i|_G)} \pmod p\\
                                      & = A^{|V(G)|}\spin{\gamma}{1}(G).
\end{align*}
The equivalence above comes from Equation~\ref{eqn:weight-conf}.

We have shown that $\pspin{\gamma}{1}$ reduces to \pinnedglpart{}. $\pspin{\gamma}{1}=\gpart$ and by 
Corollary~\ref{cor:spin-unary} \gpart{} is $\numpp$-hard. By Lemma~\ref{lem:spin-pin}, \pinnedglpart{} reduces to 
\glpart{}.
\end{proof}




\subsubsection{Finding gadgets}
\label{sec:spins:gadgets}

In this section we show values of the parameter space $(\gamma,\lambda,p)$ for which \glpart{} is $\numpp$-hard. 
All the proofs of lemmas in this section essentially identify a partially pinned multigraph $(J,x)$ with a 
distinguished vertex so that Lemma~\ref{lem:gadget-condition} applies. First we show that when $\gamma\equiv0$ and 
$\lambda\not\equiv0$ \glpart{} is hard. The gadget is a clique of appropriate size.

\begin{lemma}\label{p:lem:ISP-hardness}
 For every prime~$p$ and $\lambda\not\equiv 0\pmod p$, $\pspin{0}{\lambda}$ is $\numpp$-hard.
\end{lemma}
\begin{proof}
Let $p$ prime and $\lambda\not\equiv 0\pmod p$. Define $(J,x)$ to be the following partially pinned multigraph with a 
distinguished vertex. $G(J)$ is the clique $K_k$ with $k>0$ and $k\equiv p+2-\lambda\pmod p$ vertices, where $x\in 
V(G(J))$ and $\tau=\tau(J)=\emptyset$.

$\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)=\lambda^{k-1}(\lambda+k-1)$ and 
$\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)=\lambda^{k-1}$. If we chose $k=p+2-\lambda$, then
\begin{align*}
 \spin{\gamma}{\lambda}^{\tau,0}(G(J),x)& =\lambda^{k-1}(\lambda+p+2-\lambda-1)\\
 & \equiv \lambda^{k-1} & \pmod p\\
 & \equiv \spin{\gamma}{\lambda}^{\tau,1}(G(J),x). &\pmod p
\end{align*}

Since $\lambda$ is 
non-zero and not a multiple of $p$, $\lambda^{k-1}$ is also non-zero and not a multiple of $p$. 
$\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)\not\equiv0\pmod p$ and the proof follows from Lemma~\ref{lem:gadget-condition}.
\end{proof}


The next lemma shows that if $\gamma$ is a generator in the multiplicative group $\mathbb{Z}^*_p$ or if $\gamma$ is in 
the same orbit as $\lambda$ in the multiplicative group $\mathbb{Z}^*_p$ the \glpart{} is hard. The gadget that we 
use in order to derive hardness is a pair of vertices connected with the appropriate 
number of parallel edges, where one of the vertices is pinned to ``1''.


\begin{lemma}\label{lem:lambda-generator-hardness}
Let $p$ be a prime and let $\gamma,\lambda\in\zp$, with $\gamma^2\not\equiv1\pmod p$ and $\lambda\not\equiv 0\pmod p$. 
If there exists $k\in\ints$ such that $\gamma^k\equiv\lambda\pmod p$, then \glpart{} is 
$\numpp$-hard.
\end{lemma}
\begin{proof}
 Let $(J,x)$ be the partially pinned multigraph with two vertices $x$ and $y$ and $k$ parallel edges $(x,y)$. 
Let $\tau=\tau(J)=\{y\mapsto 
1\}$. $\spin{\gamma}{\lambda}^{\tau,0}(J,x)=\lambda$ and $\spin{\gamma}{\lambda}^{\tau,1}(J,x)=\gamma^k$. 
Since $\gamma^k\equiv\lambda\not\equiv 0\pmod p$, the proof follows from Lemma~\ref{lem:gadget-condition}.
\end{proof}

Observe that for any partially pinned multigraph with a distinguished vertex $(J,x)$ with a 
pinning function $\tau=\tau(J)$, where $x\notin\dom(\tau)$, $\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)$ is a multiple 
of $\lambda$. 
That is because every term of $\sum_{\sigma\in 
R(J,\tau)}^{\sigma(x)=0}\gamma^{c(\sigma)}\lambda^{\ell(\sigma)}$ is a multiple of $\lambda$ since $x$ 
is always mapped to ``0''. We have the following observation.

\begin{observation}\label{obs:connect-gadgets}
 Let $(J_1,x_1)\dots(J_k,x_k)$ be a set of partially pinned multigraphs with distinguished vertices and let for 
$i\in[k]$, $\tau_i=\tau(J_i)$. Define $(J,x)$ to be the graph 
constructed by identifying all vertices $x_i$ and let $\tau=\bigcup_{i\in[k]}\tau_i$. If 
$\spin{\gamma}{\lambda}^{\tau_i,0}(J_i,x_i)=\lambda A_i$ and 
$\spin{\gamma}{\lambda}^{\tau_i,1}(J_i,x_i)=B_i$ then 
$\spin{\gamma}{\lambda}^{\tau,0}(J,x)=\lambda\prod_{i\in[k]}A_i$ and 
$\spin{\gamma}{\lambda}^{\tau,1}(J,x)=\prod_{i\in[k]}B_i$.
\end{observation}

Some of the graphs we consider as gadgets are cliques. For the clique $K_k$, 
$\spin{\gamma}{\lambda}(K_k)=\sum_{i=0}^k\binom{k}{i}\lambda^i\gamma^{\binom{k-i}{2}}$. This is true because there 
are $\binom{k}{i}$ mappings~$\sigma$ with $\ell(\sigma)=i$. For every such 
mapping~$\sigma$, $k-i$ vertices are mapped to ``1'', hence $c(\sigma)=\binom{k-i}{2}$. Based on the latter, we have 
the 
following observation.

\begin{observation}\label{obs:clique-spins}
 Let $(J,x)$ be a partially pinned graph, where $G(J)=K_{k+1}$ is the clique with $k+1$ vertices, one of which is $x$ 
and let $\tau=\tau(J)=\emptyset$. Then,
 \[\spin{\gamma}{\lambda}^{\tau,0}(G(J),x)=\lambda\sum_{i=0}^k\binom{k}{i}\lambda^i\gamma^{\binom{k-i}{2}}\]
 and
\[\spin{\gamma}{\lambda}^{\tau,1}(G(J),x)=\sum_{i=0}^k\binom{k}{i}\lambda^i\gamma^{\binom{k-i}{2}}
\gamma^{k-i}.\]
\end{observation}

The other gadgets we will consider are paths.

\begin{observation}\label{obs:paths-spins}
 Let $P_2=xx_1x_2$ be the path of length $2$ and let $P_3=xx_1x_2x_3$ be the path of length 3. We have,
 \begin{align*}
  \spin{\gamma}{\lambda}^{\tau,0}(P_2,x)&=\lambda(\lambda^2+2\lambda+\gamma)\\
  \spin{\gamma}{\lambda}^{\tau,1}(P_2,x)&=\lambda^2+\lambda\gamma+\lambda+\gamma^2\\
  \spin{\gamma}{\lambda}^{\tau,0}(P_3,x)&=\lambda(\lambda^3+3\lambda^2+2\lambda\gamma+\lambda+\gamma^2)\\ 
\spin{\gamma}{\lambda}^{\tau,1}(P_3,x)&=\lambda^3+2\lambda^2+\lambda^2\gamma+2\lambda\gamma+\lambda\gamma^2+\gamma^3.
 \end{align*}
\end{observation}


Using the previous observations we can produce a computer assisted proof identifying the values of the parameters 
$\gamma$, $\lambda$ and $p$ that make \glpart{} $\numpp$-hard, when $p$ is small.

\begin{lemma}\label{lem:small-primes-spin-hard}
 For all primes $p<100$, $p\neq41$ and all $\gamma,\lambda\in\mathbb{Z}_p$ with $\gamma^2\not\equiv1\pmod p$ and 
$\lambda\not\equiv0\pmod p$, \glpart{} is $\numpp$-hard.
\end{lemma}
\begin{proof}
 Let $\veck=(k_0,k_1\dots, k_m)$ be a vector of $(\mathbb{Z}_p)^{m+1}$ for $m\in\posints$. Let $(J(\veck),x)$ be the 
partially pinned multigraph with a distinguished vertex~$x$. $G(J(\veck))$ is constructed by taking the union of 
disjoint copies of the following multigraphs and identifying their distinguished vertices.

\begin{itemize}
 \item The multigraph with vertex set $\{x,y\}$ and $k_0$ parallel edges $(x,y)$, where $x$ is the distinguished vertex.
 \item For each $j\in[m-2]$, $k_j$ copies of the clique $K_{j+1}$, where $x_j\in V(K_{j+1})$ is the distinguished 
vertex.
 \item $k_{m-1}$ copies of the path $P_2=xx_1x_2$, where $x$ is the distinguished vertex.
 \item $k_{m}$ copies of the path $P_3=xx_1x_2x_3$, where $x$ is the distinguished vertex.
\end{itemize}
Let $\tau(J(\veck))=\tau=\{y\mapsto 1\}$.

From Observations~\ref{obs:connect-gadgets}, \ref{obs:clique-spins}, \ref{obs:paths-spins} and the proof of 
Lemma~\ref{lem:lambda-generator-hardness} we have,

\[\spin{\gamma}{\lambda}^{\tau,0}(G(J(\veck)),x)\!=\!\lambda\!\!
\left(\prod_{j=1}^{m-2}\big(\!\sum_{i=0} ^j\binom {j}{i}\lambda^i\gamma^{ \binom{j-i}{2}}\big)^{k_j}\!\!\right)\!\!\!
\left(\spin{\gamma}{\lambda}^{\tau,0}(P_2,x)/\lambda\right)^{k_{m-1}}\!\!
\left(\spin{\gamma}{\lambda}^{\tau,0}(P_3,x)/\lambda\right)^{k_m}\]
and
\[\spin{\gamma}{\lambda}^{\tau,1}(G(J(\veck)),x)\!=\! (\gamma)^{k_0}\!\!
\left(\prod_ { j=1 } ^{m-2}\big(\!\sum_{i=0}^j\binom{j}{i}\lambda^i\gamma^ 
{\binom{j-i}{2}}\gamma^{j-i}\big)^{k_j}\!\!\right)\!\!\!
\left(\spin{\gamma}{\lambda}^{\tau,1}(P_2,x)\right)^{k_{m-1}}\!\!
\left(\spin{\gamma}{\lambda}^{\tau,1}(P_3,x)\right)^{k_m}\!\!\!\!\!\!\!.
\]

Using the program presented in the Appendix, we can show that for all primes $p<100$, with $p\neq41$ and for all 
$\gamma,\lambda\in\zp$, where $\gamma^2\not\equiv1\pmod p$ and $\lambda\not\equiv0\pmod p$, there exists  
$\veck\in(\mathbb{Z}_p)^{m+1}$ for $m\in\posints$, such that 
$\spin{\gamma}{\lambda}^{\tau,0}(J(\veck),x)\equiv\spin{\gamma}{\lambda}^{\tau,1}(J(\veck),x)\not\equiv0\pmod p$. The 
lemma follows from 
Lemma~\ref{lem:gadget-condition}.
\end{proof}

The program we used in the above proof, only failed to find a gadget for $p=41, \gamma=18$, $\lambda=6$. We 
conjecture that there exists a gadget for these parameter values, so for all $\gamma,\lambda\in\mathbb{Z}_{41}$ 
with $\gamma^2\not\equiv1\pmod p$ and $\lambda\not\equiv0\pmod p$, $\#_{41} Z_{\gamma,\lambda}$ is $\numpp$-hard.

\subsection{Summary of results}
\label{sec:spins:summary}

Now we can summarise the results of this section. We will use the following.
\begin{lemma}\label{lem:plus-minus-one-square}
Let $p$ be a prime and let $\gamma\in\zp$. $\gamma^2\equiv 1 \pmod p$ if and only if $\gamma\equiv\pm1\pmod p$.
\end{lemma}
\begin{proof}
 If $\gamma\equiv\pm1\pmod p$ then, trivially $\gamma^2\equiv 1\pmod p$. Now assume that $\gamma^2\equiv1 \pmod p$ we 
have,
\begin{align*}
\gamma^2\equiv 1 &\pmod p \\
(\gamma-1)(\gamma+1)\equiv 0 &\pmod p.
\end{align*}
The latter equation is only true when $\gamma\equiv\pm 1\pmod p$, so the lemma follows.
\end{proof}


The main theorem of this section summarises our results on the complexity of \glpart{}.

{\renewcommand{\thetheorem}{\ref{thm:spin-field-main}}
\begin{theorem}
 Let $p$ be a prime and let $\gamma,\lambda\in\zp$. \glpart{} is computable in polynomial time when one of the 
following holds.
 \begin{enumerate}
  \item $\lambda=0$.
  \item $\gamma=1$.
  \item $\gamma=-1$ and $\lambda\in\{0,\pm1,\pm i_p\}$.
 \end{enumerate}
Furthermore, \glpart{} is $\numpp$-complete when one of the following holds.
\begin{enumerate}
\setcounter{enumi}{3}
 \item $\lambda\not\equiv 0\pmod p$ and $\gamma\equiv 0 \pmod p$.
 \item $\lambda\not\equiv 0\pmod p$, $\gamma\not\equiv\pm1\pmod p$ and there exists an integer~$k$ with 
$\gamma^k\equiv\lambda\pmod p$.
 \item $\lambda\not\equiv 0\pmod p$, $\gamma\not\equiv\pm1\pmod p$ and $p<100$, where $p\neq41$.
\end{enumerate}
\end{theorem}}
\begin{proof}
By Lemma~\ref{lem:spin-poly}, \glpart{} is computable in polynomial time when (1)-(3) hold. 
By Lemma~\ref{p:lem:ISP-hardness} \glpart{} is $\numpp$-hard when (4) holds. By Lemma~\ref{lem:plus-minus-one-square} 
and Lemma~\ref{lem:lambda-generator-hardness} \glpart{} is hard when (5) holds. Finally, by 
Lemma~\ref{lem:plus-minus-one-square} 
and Lemma~\ref{lem:small-primes-spin-hard} we have that \glpart is hard when~(6) holds.
\end{proof}

\subsection{Generalised spin systems with field}

For a $2\times2$ matrix and integer $\lambda$ and a multigraph $G$, we define
\[\spin{A}{\lambda}(G)=\!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\lambda^{\ell(\sigma)}\!\!\!\prod_{(u,v)\in E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)},\]
where $\ell(\sigma)$ is the number of vertices $\sigma$ maps to $0$. Thus $\spin{\gamma}{\lambda}=\alspin$, for $A=	
\left[\begin{smallmatrix}
		1 &  1 \\ 
		1 & \gamma
	\end{smallmatrix} \right]$

We will also study the following problem:
\GL{I appreciate this but can we just cease defining every special case for $\varpart{\alpha}{\beta}{\gamma}$ as a macro? I defined the general problem now as a macro, so please use this instead of defining the next special case. Keep it clean! }
\begin{problem}
 \item \emph{Name.} \palspin{}
\item \emph{Parameter.} a prime $p$, a $2\times2$ matrix $A$ with entries in $\zp$ and $\lambda\in\zp$.
\item \emph{Input.} A multigraph $G$.
\item \emph{Output.} $\alspin(G) \pmod p$.
\end{problem}

\noindent Let $\zp$ be the additive group of integers modulo~$p$. For a prime $p$ and an integer $k\in\zp$, when 
working in $\zp$ we will, sometimes, denote $p-k$ with $-k$.

\subsubsection{Vertex weights}
\label{sec:spins-field}

\agob{This is the section where we should use the reduction from $\lambda$ to $\lambda^{-1}$}
We defined \glpart{} so that vertices contribute a factor of $\lambda$ when they are mapped to ``0''. We can also 
consider the version of the problem when the unary weight comes from the vertices mapped to ``1''. Let $G$ be a 
multigraph, let $\sigma: V(G)\rightarrow\{0,1\}$ and let $\ell'(\sigma)=|V(G)|-\ell(\sigma)$, i.e. the number of 
vertices 
mapped to ``1'' by $\sigma$. Define

\[\spin{A}{\lambda}'(G)=\!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\lambda^{\ell'(\sigma)}\!\!\!\prod_{(u,v)\in E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}.\]

Let $p$ be a prime and let $\lambda^{-1}$ be the inverse of $\lambda$ in $\zp$. From the definitions of 
$\spin{A}{\lambda}$, $\spin{A}{\lambda}'$ and $\ell'$ we have,

\begin{align*}
(\lambda^{-1})^n\spin{A}{\lambda}(G)& \equiv (\lambda^{-1})^n \!\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!\!\lambda^{\ell(\sigma)} \prod_{(u,v)\in E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}& \pmod p \\
& \equiv\!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!(\lambda^{-1})^{|V(G)|-\ell(\sigma)}\prod_{(u,v)\in E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}& 
\pmod p\\
&\equiv \!\!\!\sum_{\sigma: 
V(G)\rightarrow\{0,1\}}\!\!\!(\lambda^{-1})^{\ell'(\sigma)}\prod_{(u,v)\in E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}& \pmod 
p\\
&\equiv\spin{A}{\lambda^{-1}}'(G). & \pmod p
\end{align*}

That is for any multigraph $G$, if we can compute $\spin{A}{\lambda}(G)$ modulo a prime~$p$, then we can compute 
$\spin{A}{\lambda^{-1}}'(G)$ modulo a prime~$p$. So classifying the complexity of \glpart{}, for every prime~$p$ 
and every $\lambda\in\zp$, is equivalent to determining the complexity of computing $\spin{A}{\lambda}'$ 
modulo~$p$. 

\subsubsection{Pinning in two-spin systems}
\label{sec:spins:pin}

% The gadgets we will use for our reductions from \gpart{} to \glpart{} will be multigraphs with 
% vertices pinned to either ``0'' or ``1''. 
In the setting of \alpart{}, a \emph{pinning function}~$\tau$ of a multigraph~$G$ is a partial function from $V(G)$ to 
$\{0,1\}$. A vertex~$v$ in the domain of the pinning function is said to be \emph{pinned} or \emph{pinned to $\tau(v)$}. 
A \emph{partially pinned multigraph} $J=(G,\tau)$ consists of an \emph{underlying graph}~$G$ and a pinning
function~$\tau$ from $V(G)$ to~$\{0,1\}$. 

\begin{definition}\label{defn:respect-tau}
 Let $G$ be a multigraph and let $\tau:V(G)\rightarrow\{0,1\}$ be a pinning function of $G$. 
$R(G,\tau)=\{\sigma:V(G)\rightarrow\{0,1\}\mid \sigma(v)=\tau(v)\textrm{ for 
} v\in\dom(\tau)\}$ is the set of mappings that respect $\tau$. 
\end{definition}


Given a partially pinned multigraph $(G,\tau)$ 
we define 
\[\spin{A}{\lambda}^\tau(G)=\sum_{\sigma\in R(G,\tau)}\!\!\!\lambda^{\ell(\sigma)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}.\]
The pinned version of \alpart{} is the following.

\probpar{\pinnedalpart.}
{A prime $p$ and $\gamma,\lambda\in\zp$.}
{A partially pinned multigraph $J=(G,\tau)$.}
{$\spin{A}{\lambda}^\tau(G)\pmod p$.}
 
The following lemma shows that computing \alpart{} is at least as hard as computing \pinnedalpart{}.

\begin{lemma}\label{lem:alspin-pin}
 For any prime $p$ \pinnedalpart{} reduces to \alpart{} under polynomial-time Turing reductions.
\end{lemma}
\begin{proof}
The proof is similar to that of Lemma~8 in The Complexity of Weighted Boolean \#CSP, by Dyer, Goldberg and Jerrum.
Will not write it down as we can just cite them, and for non symmetric matrices gets rather extensive. The only thing 
that changes is the unary weight of $\lambda$ comes in some of the equations, but it is no problem since it is only a 
constant.
\end{proof}


\subsubsection{Gadgets for two-spin systems}
\label{sec:spins:property}

In order to prove hardness for \alpart{}, we need to find gadgets which, by attaching to every vertex of $G$, will 
cancel out the weights of $\lambda$ that the vertices mapped to ``0'' contribute to the partition function. Our gadgets 
$(J,x)$ 
consist of a partially pinned multigraph~$J=(G,\tau)$ with a distinguished vertex $x\in V(G(J))$. Recall 
Definition~\ref{defn:respect-tau} of $R(G,\tau)$. To express the properties of the gadgets we will need the following 
definitions.

\begin{definition}\label{dfn:zero-one}
 Let $(J,x)$ be a partially pinned multigraph with a distinguished vertex. Let 
$G=G(J)$ and let $\tau=\tau(J):V(G(J))\rightarrow\{0,1\}$ be the 
pinning function of $J$, such that $x\notin\dom(\tau)$. \GL{The notation for $\tau$ should incorporate $x$.} We define

\[
\spin{A}{\lambda}^{\tau,0}(G,x)=\sum_{\substack{\sigma\in 
R(G,\tau),\\ \sigma(x)=0}}\lambda^{\ell(\sigma)} \prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}\quad\textrm{ and}
\]

\[
 \spin{A}{\lambda}^{\tau,1}(G,x)=\sum_{\substack{\sigma\in 
R(G,\tau),\\ \sigma(x)=1}}\lambda^{\ell(\sigma)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}.
\]
\end{definition}

As in Theorem~\ref{p:thm:hardness-gadget} we will use the following notation to build partially pinned multigraphs
containing many copies of some subgraph. For any ``tag''~$T$ (which we will treat just as an arbitrary string) and any 
partially labelled multigraph~$J$, denote by $J^T$ a copy of~$J$ with every vertex $v\in V(G(J))$ renamed~$v^T\!$. 

\begin{definition}\label{dfn:g-gamma}
Given a multigraph $G$ and a partially pinned multigraph with a distinguished vertex 
$(J,x)$ we define $G \odot(J,x)$ to be the partially pinned multigraph constructed in the following way. Take a copy of 
$G$ together with the union of disjoint copies~$G^v(J)$ of~$G(J)$ for each $v\in V(G)$. For 
each vertex $v\in V(G)$ identify $v$ with~$x^v$. Let $\tau(G \odot(J,x))=\bigcup_{v\in V(G)}\tau(G^v(J))$. \GL{Not sure which $\tau$ you are talking about here... see above comment}
\end{definition}

\agob{$\kappa$ and the other two partial spins could be zero, but that doesn't give us anything and makes the reduction 
fishy.}
\begin{lemma}\label{lem:gadget-condition_general}
	Let $p$ be a prime and let $\gamma,\lambda\in\zp$, with $\lambda\not\equiv 0\pmod p$. 
	If there exists a partially pinned multigraph with a distinguished vertex~$(J,x)$ and $\tau=\tau(J)$, such 
that 	$\spin{A}{\lambda}^{\tau,0}(G(J),x)\equiv\kappa \, \spin{A}{\lambda}^{\tau,1}(G(J),x)\not\equiv0\pmod 
p$ with $\kappa \in \mathbb{Z}^*_p$, then \akpart{} reduces to \alpart{}. 
\end{lemma}
\begin{proof}
Since, from Lemma~\ref{lem:alspin-pin} ,\pinnedalpart{} reduces to \alpart{}, it suffices to show that \akpart{} reduces 
to \pinnedalpart{}. 

	Let $G$ be the input of \akpart{} and let $(J,x)$ be a partially pinned multigraph with a
	distinguished vertex, such that 
	$\spin{A}{\lambda}^{\tau,0}(G(J),x)\equiv\kappa \,\spin{A}{\lambda}^{\tau,1}(G(J),x)\equiv a\not\equiv 0 \pmod 
p$.	Let $J'=G\odot(J,x)$ be the partially pinned graph, as in Definition~\ref{dfn:g-gamma}. $J'$ will 
	be the input for \pinnedalpart{}. We denote $G'=G(J')$ and $\tau'=\tau(J')$.
	
	For $\sigma,\sigma' \in R(G',\tau')$ we write $\sigma\sim_G\sigma'$ if $\sigma|_G=\sigma'|_G$. We 
	also write $\eqclass{\sigma}_G$ for the $\sim_G$-equivalence class of $\sigma$. The classes 
$\eqclass{\sigma}_G$ 
	partition the set of configurations of $J'$. For $\sigma\in R(G',\tau')$ we define 
	\[W(\eqclass{\sigma}_G)=\sum_{\sigma\in\seqclass{\sigma}_G}\lambda^{\ell(\sigma)}\!\!\!\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}.\]
	Let $\sigma\in R(G',\tau')$, be a configuration of $G'$ that respects $\tau'$. $\sigma$ maps 
$\ell(\sigma|_G)$ vertices of $G$ to ``0'' and $V(G)-\ell(\sigma|_G)$ vertices of $G$ to ``1''. Therefore,
	\begin{align*}
	W(\eqclass{\sigma}_G)= & \left(\sum_{\substack{\sigma'\in 
			R(G(J),\tau(J)),\\ \sigma'(x)=0}}\lambda^{\ell(\sigma')}\prod_{(u,v)\in 
E(G)}A_{\sigma'(u),\sigma'(v)}
	\right)^{\ell(\sigma|_G)} \\
	&\cdot \left(\sum_{\substack{\sigma'\in 
			R(G(J),\tau(J)),\\ \sigma'(x)=1}}\lambda^{\ell(\sigma')}\prod_{(u,v)\in 
E(G)}A_{\sigma(u),\sigma(v)}
	\right)^{V(G)-\ell(\sigma|_G)}
	 \prod_{(u,v)\in 
E(G)}A_{\sigma|_G(u),\sigma|_G(v)} \,.
	\end{align*}
	
	From Definition~\ref{dfn:zero-one} we now have,
	
	\[W(\eqclass{\sigma}_G)= 
	\big(\spin{A}{\lambda}^{\tau,0}(G(J),x)\big)^{\ell(\sigma|_G)}\big(\spin{A}{\lambda}^{\tau,1} 
	(G(J),x)\big)^{V(G)-\ell(\sigma|_G)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma|_G(u),\sigma|_G(v)}.\]
	
	By the choice of $J$, 
$\spin{A}{\lambda}^{\tau,0}(G(J),x)\equiv\kappa \,\spin{A}{\lambda}^{\tau,1}(G(J),x)\equiv a \pmod p$, so
	
	\begin{align*}\label{eqn:weight-conf}
	W(\eqclass{\sigma}_G) & \equiv a^{\ell(\sigma|_G)}(ak^{-1})^{V(G)-\ell(\sigma|_G)} \prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma|_G(u),\sigma|_G(v)}
	 \pmod p\\
	& \equiv a^{|V(G)|}\kappa^{-|V(G)|}\kappa ^{\ell(\sigma|_G)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma|_G(u),\sigma|_G(v)} \pmod p
	\end{align*}
	
	
	
	Now let $\sigma_1\dots\sigma_k$ be representatives of the $\sim_G$-equivalence classes.
	\begin{align*}
	\spin{A}{\lambda}^\tau(G')& = \sum_{\sigma\in R(G',\tau')}\!\!\lambda^{\ell(\sigma)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)} \\
	& =\sum_{i=1}^k\sum_{\sigma\in\seqclass{\sigma_i}_G }
	\lambda^{\ell(\sigma)} \prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma(u),\sigma(v)}\\
	& =\sum_{i=1}^k W(\eqclass{\sigma_i}_G) \\
	& \equiv \sum_{i=1}^k a^{|V(G)|}\kappa^{-|V(G)|}\kappa^{\ell(\sigma_i|_G)}\prod_{(u,v)\in 
E(G)}\!\!\!\!A_{\sigma|_G(u),\sigma|_G(v)} \pmod p\\
	& = a^{|V(G)|}\kappa^{-|V(G)|}\spin{A}{\kappa}(G).
	\end{align*}
The equivalence above comes from Equation~\ref{eqn:weight-conf}. This concludes the proof that 
$\pspin{A}{\kappa}$ reduces to \pinnedalpart{}.
\end{proof}




\subsection{New Gadgets}

In the following we will discuss various additional findings. Since we are concerned with $\kcsp[p]$ in a more general setting, we introduce the notation $\kcsp[p](\{B,U\})$, where $B$ is the matrix associated with the binary system and $U$ is the vector associated with the unary system. Let 
\[
	B_\gamma = 
	\begin{bmatrix}
		1 &  1 \\ 
		1 & \gamma
	\end{bmatrix}  
	\quad \mbox{and} \quad
	U_\lambda =
	\begin{bmatrix}
		\lambda \\ 
		1
	\end{bmatrix} \, ,
\]
then we have studied $\kcsp[p](\{B_\gamma,U_\lambda\})$ so far.

\begin{lemma}\label{lem:change_edge_inter}
	For $p>2$ prime and $\gamma, \lambda \not\equiv 1,-1 \pmod p$, $\lambda^2 \not\equiv -1 \pmod p$ with $|\Orb_p 
	(\gamma)|= \kappa$ even we have that $\kcsp[p](\{B,U_\lambda\})$ reduces to $\kcsp[p](\{B_\gamma,U_\lambda\})$ under 
	polynomial time Turing reduction, where
	\[
		B = 
		\begin{bmatrix}
			1 + \lambda &  \gamma^{\kappa/2} + \lambda \\ 
			\gamma^{\kappa/2} + \lambda & 1 + \lambda
		\end{bmatrix}  \, .
	\]
\end{lemma}
\iffalse
\begin{proof}
Let $p$, $\gamma$, $\lambda$ and $\kappa$ be as stated.

\end{proof}
\fi

%\iffalse
\begin{proof}
	First, we observe that $\mathbb{Z}_p^*$ is of even cardinality, hence (by Lagrange) $\kappa$ has to be even, where we further used the uniqueness of square-roots in $\mathbb{Z}_p^*$ \textbf{(actually this is not true in general, we needed the above assumption of $\kappa$ being even)}. Therefore, $\kappa /2$ is a natural number. We use the following gadget: Let $G=(V,E)$ be the graph with $V=\{x,y,z\}$ and $E = \{(xy)^{\kappa /2} , (yz)^{\kappa /2}\}$. We obtain for this gadget the following spin-system:
	\begin{align*}
		\spin{\gamma}{\lambda}^{x,z \mapsto 0} &= 1 + \lambda \,,\\
		\spin{\gamma}{\lambda}^{x\mapsto 0\, ,z \mapsto 1} &= \gamma^{\kappa/2} + \lambda \,,\\
		\spin{\gamma}{\lambda}^{x\mapsto 1\, ,z \mapsto 0} &= \gamma^{\kappa/2} + \lambda \,,\\
		\spin{\gamma}{\lambda}^{x,z \mapsto 1} &= \gamma^{\kappa} + \lambda \equiv 1 + \lambda \pmod p\,,\\
	\end{align*}
	leading to the binary system $B$. It remains to show, that hardness for $B$ implies hardness for $B_\gamma$. Due to (Guo et al. Lemma~$3.6.$) we know, that $B$ is hard whenever $(1+\lambda)^2 \, (\gamma^{\kappa/2} + \lambda )^2 \not\equiv 0 \pmod p$ and
	\[
		(1+\lambda)^4 \not\equiv (\gamma^{\kappa/2} + \lambda)^4 \pmod p \, .
	\]
	The first condition is easy to check as it reduces to each factor being non-zero. Since $\lambda \not\equiv -1 \pmod p$ the first factor cannot be $0$. If the second factor would be zero then 
	\[
		\gamma^{\kappa /2} \equiv -\lambda \pmod p
	\]
	and $(-\lambda)^2 \equiv 1 \pmod p$, therefore $-\lambda$ would be a square-root and thus $\lambda$ as well, which contradicts our assumption.
	
	Regarding the second condition by simply taking the complete expression we obtain
	\[
		(1+4\lambda +6\lambda^2+4\lambda^3+\lambda^4) \not\equiv (1 + 4\gamma^{\kappa/2}\lambda + 6\lambda^2 + 4\gamma^{\kappa/2}\lambda^3 + \lambda^4) \pmod p \,,
	\]
	which simplifies to
	\[
		4\lambda(1+\lambda^2) \not\equiv 4\gamma^{\kappa/2} \lambda (1+ \lambda^2) \pmod p \,.
	\]
	Therefore, under the assumption that $\lambda(1+\lambda^2) \not\equiv 0 \pmod p$, we obtain that 
	\[
		1 \not \equiv \gamma^{\kappa/2} \pmod p \, ,
	\]
	which is satisfied due to our choice of $\kappa$. Furthermore, observe that $\lambda(1+\lambda^2) \not\equiv 0 \pmod p$ holds since $\lambda^2 \not\equiv -1 \pmod p$.
\end{proof}


I was curious to see what happens when $\gamma=-1$ and $\lambda\notin\{0,\pm1,\pm i_p\}$. I conjecture that the 
problem is hard. \GL{Sure it is hard, just invert the $\gamma$, $\lambda -1$ with $\lambda$, $\gamma -1$. Thus, you  
observe now $\spin{3}{-2}$ and $3$ is a root of unity in $\Z_7$. Thus, by the graph with $1$ vertex and $5$ loops you 
find $\kappa \equiv 1 \pmod 7$ in Lemma~\ref{lem:gadget-condition_general}, which established hardness. AG: That is not 
true, you can not invert gamma and lambda in the spin systems, only in the reduction from the spin system to the 
homomorphism.}

\begin{lemma}
 Let $p=7$, $\gamma=-1$ and $\lambda=2$. \glpart{} is hard.
\end{lemma}

\begin{proof}
We only work mod 7. We start with the CSP expressed by the matrix  $\left[\begin{smallmatrix} 2 & 1\\
                 1 & 2
                 \end{smallmatrix}\right]$. and no unary weights. This is hard by Guo et al.
                 
This reduces to the CSP with edge interactions expressed by $\left[\begin{smallmatrix}
                 2 & 1\\
                 1 & 2
                 \end{smallmatrix}\right]$ and vertex weights expressed by $\left[\begin{smallmatrix}
                 2\\
                 1
                 \end{smallmatrix}\right]$. This reduction by applying lemma~\ref{lem:gadget-condition_general} using 
the single edge $(x,v)$ and pinning $v$ to 1.

Next we reduce to the CSP with edge interactions expressed by $\left[\begin{smallmatrix}
                 3 & 1\\
                 1 & 3
                 \end{smallmatrix}\right]$ and vertex weights expressed by $\left[\begin{smallmatrix}
                 2\\
                 1
                 \end{smallmatrix}\right]$. This is done just by doubling the edges of the input graph.
                 
Finally, using Lemma~\ref{lem:change_edge_inter}, with $\kappa=2$, we get our spin system.
\end{proof}


\begin{observation}
	\begin{enumerate}
		\item We observe, that Lemma~\ref{lem:gadget-condition} is a special case of Lemma~\ref{lem:gadget-condition_general}.
		\item (Gregor claim:) for every graph $G$ and any vertex $x \in V(G)$ there exists always a constant $\kappa$, such that the condition of Lemma~\ref{lem:gadget-condition_general} is satisfied.
		\item Taking $G$ to be the graph on one vertex with one loop, we observe
			$\spin{\gamma}{\lambda}^{\tau, 0}(G') = \lambda$ and $\spin{\gamma}{\lambda}^{\tau, 1}(G') = \gamma$, which implies that $\kappa = \gamma \lambda^{-1}$ and \gvarpart{\gamma \lambda^{-1}} reduces to \glpart{}.
		\item Iterating the above reduction with the same graph each time we obtain a cycle of reductions
			\[
				\gvarpart{\lambda} \,\mbox{reduces to}\, \gvarpart{\gamma \lambda^{-1}} \,\mbox{reduces to}\, \glpart{}.
			\]
		\item (Gregor claim:) It is obvious, that the repetition of above argument for any graph $G$ will always yield a cycle since we are in a finite field. However, it is not straightforward to assume that these reductions are legit ones, since we might violate the conditions of Lemma~\ref{lem:gadget-condition_general}. Therefore, I claim that for any graph $G$ and any vertex $x\in V(G)$ such that said conditions are satisfied, we will obtain a legit cycle of reductions. Moreover (see first claim), I highly doubt that there exists a graph $G$ and a vertex $x \in V(G)$, such that the conditions are not satisfied.
		\item Using the Graph consisting only of one vertex we obtain
			\[
					\glpart{} \,\mbox{reduces to}\,  \gvarpart{ \lambda^{-1}} \,\mbox{reduces to}\, \glpart{} .
			\]
		\item Using a combination of above gadgets we obtain
			\[
				\glpart{} \equiv \gvarpart{ \lambda^{-1}} \equiv \gvarpart{\gamma \lambda^{-1}} \equiv \gvarpart{\gamma \lambda} \equiv \gvarpart{\gamma^{-1} \lambda^{-1}} \gvarpart{\gamma^{-1} \lambda} ,
			\]
		\item Using the graph with one vertex and $\rho$ loops we obtain
			\[
			\glpart{} \equiv \gvarpart{ \lambda^{-1}} \equiv \gvarpart{\gamma^{\rho} \lambda^{-1}} \equiv \gvarpart{\gamma^{\rho} \lambda} \equiv \gvarpart{\gamma^{-\rho} \lambda^{-1}} \gvarpart{\gamma^{-\rho} \lambda} .
			\]			
	\end{enumerate}
\end{observation}

\begin{lemma}[Karen can prove this]
Let $p$ be a prime and $\calF = \{B,U\}$ for a binary Boolean function $B$ and a unary Boolean function $U$. 
If there exists a partially pinned set of constraints $(\mathcal{D},\tau)$ with a distinguished variable $x$ as well as $\kappa \in \mathbb{Z}^*_p$, such that 
$\kappa \, \csp_{\calF}^{\tau,0}(\mathcal{D},x) \equiv \csp_{\calF}^{\tau,1}(\mathcal{D},x) \not\equiv0\pmod p$, then 
$\kcsp[p]_{B,[\kappa^{-1},1]}^{\text{unary-complete}}$ reduces to $\textsc{Pinned}\kcsp[p]_{B,U}$. 
\end{lemma}


==> introduction-c.tex <==

A homomorphism from a graph~$G$ to a graph~$H$ 
is a mapping from~$V(G)$ to~$V(H)$ that preserves edges, in the sense that every edge of~$G$ must be mapped to an edge 
of~$H$; non-edges of~$G$ may be mapped to either edges or non-edges of~$H$.
Many notions of graph theory can be naturally described as graph homomorphisms. 
For example, the proper $q$-colourings of a graph~$G$
correspond to the homomorphisms from~$G$ 
to a $q$-clique. Independent sets of~$G$ correspond to the homomorphisms from~$G$ to
the connected graph with two vertices and one loop (vertices of~$G$ which are mapped to the vertex with a loop are 
out of the corresponding independent set; vertices which are mapped to the other vertex are in it).
Weighted sums of homomorphisms can also represent partition functions that appear in statistical physics such as the 
Ising model, the Potts model and the hard-core model arise naturally as weighted sums of graph homomorphisms 
\cite{DG00,GGJT}.

In this paper, we study the complexity of counting homomorphisms modulo a prime~$p$. For graphs $G$ and $H$, let 
$\Homs{G}{H}$ be the set of homomorphisms from $G$ to $H$. For each prime~$p$ and each graph~$H$, where $p$ and $H$ are 
fixed as parameters, we study the computational problem \phcol{}, that is the problem of computing $|\Homs{G}{H}|\pmod 
p$ for an input graph $G$.
The value of the modulo~$p$ and the structure of the target graph~$H$ influence the complexity of \phcol{}. Consider 
the graph $H$ in Figure~\ref{fig:intro_tree}. Our results show that \phcol{} is computable in 
polynomial time when $p=2,3$ while it is hard for any other prime~$p$.

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{TikZ/intro_tree.pdf}
	\caption{text}
	\label{fig:intro_tree}
\end{figure}

Our main goal is to obtain a ``dichotomy theorem'': that is to determine the graph--prime pairs~$(H,p)$ 
for which the problem is tractable, the graph--prime pairs for which the problem is hard and to prove that for all 
graph--prime pairs either the one or the either is true. Due to a theorem of Ladner~\cite{Lad75}, showing the 
existence of problems of intermediate complexity, it is not obvious that \phcol{} does not include any such problems.

\agob{I need this theorem to explain my stuff later on, but I am not sure if it interrupts the flow?}
The complexity \nhcol{}, the problem of computing $|\Homs{G}{H}|$ from an input graph $G$ to a fixed graph $H$, is 
quite well understood. Dyer and Greenhill~\cite{DG00} have shown the following dichotomy theorem.
\begin{theorem}[Dyer and Greenhill]\label{thm:dyer-greenhil}
 Let $H$ be a graph. If every component of $H$ is a complete bipartite graph with no self-loops or a complete 
graph with all self-loops present, then \nhcol{H} can be solved in polynomial time. Otherwise \nhcol{H} is 
$\shp$-complete.
\end{theorem}

The first to study graph homomorphisms under the setting of modular counting were Faben and Jerrum~\cite{FJ13}. To 
describe their work 
we first need to state a few definitions. An automorphism of a graph $G$ is a bijective function $\rho:V(G)\rightarrow 
V(G)$, such that  $(u,v)\in E(G)$ if and only if $(\rho(u),\rho(v))\in E(G)$. Let $k$ be a 
positive integer. For a function $\rho$ let $\rho^{(k)}=\rho\circ\rho\circ\dots\circ\rho$, where the composition
is applied $k$ times. An automorphism~$\rho$ of order $k$ is an automorphism of a graph $H$, such 
that for $\ell<k$, $\rho^{(\ell)}$ is not the identity, but $\rho^{(k)}$ is the identity.
Given a graph $H$ and an automorphism~$\rho$ of $H$, $H^\rho$ denotes the subgraph of $H$ induced by the 
fixpoints of $\rho$. If $\rho$ has no fixpoints, then $H^\rho$ is the empty graph, which we also consider it to be a 
graph. We write $H \Rightarrow_k H'$ if there is an automorphism~$\rho$ of order~$k$ of~$H$ such that $H^\rho=H'$ and we 
write $H \Rightarrow_k^* H'$ if either $H$ is isomorphic to~$H'$ (written
$H\isoto H'$) or, for some positive integer~$t$, there are graphs $H_1, \dots, H_t$ such that 
$H \isoto H_1$, $H_1 \Rightarrow_k \cdots \Rightarrow_k H_t$, and $H_t  \isoto H'$.

Let $H$ be a graph, $p$ be a prime and let $\rho$ be an automorphism of order~$p$ of $H$. Faben and Jerrum showed 
\cite[Lemma~3.3]{FJ13} and that for any graph $G$ and any prime $p$, $|\Homs{G}{H}|\equiv|\Homs{G}{H^\rho}|\pmod p$. 
They also showed \cite[Theorem~3.7]{FJ13} that for every graph~$H$ and any prime $p$, there is (up to isomorphism) 
exactly one graph~$H^{*p}$ that has no automorphisms of order~$p$ such that  $H\Rightarrow_p^* H^{*p}\!$. We call 
$H^{*p}$ the \emph{order~$p$ reduced form} of~$H$. See Figure~\ref{fig:reduced-form} for a diagram showing a graph 
reduced to its order~$p$ reduced form.

These results show the existence of graphs $H$ for which \phcol{} can be solved in polynomial time. If the order~$p$ 
reduced form~$H^{*p}$ of~$H$ falls into the polynomial computable cases of Theorem~\ref{thm:dyer-greenhil}, then 
\phcol{} is computable in polynomial time. For $p=2$, Faben and Jerrum conjectured that these are the only graphs~$H$ 
for which \parhcol{} is computable in polynomial time.

\begin{conjecture}[Faben and Jerrum] \label{conj:FJ}
  Let $H$ be a  graph.  If its order~2 reduced form~$H^{*2}$ has at most one vertex, then \parhcol{} is in
    $\pol$; otherwise, \parhcol{} is $\parp$-complete.\end{conjecture}
    
Faben and Jerrum~\cite[Theorem~3.8]{FJ13} proved Conjecture~\ref{conj:FJ} for the case in which~$H$ is a tree. The 
subsequent work of G\"obel, Goldberg and Richerby~\cite{GGR14,GGR15} extends the results of Faben and Jerrum to show 
that Conjecture~\ref{conj:FJ} is true when the target graph $H$ is a cactus graph or a square-free graph. Our work goes 
to a direction orthogonal to the work of G\"obel, Goldberg and Richerby: instead of trying to prove the conjecture for 
richer classes of graphs, we show a dichotomy theorem for all primes, while restricting the target graph $H$ to be 
trees. Our main result is the following. 

\begin{theorem}\label{thm:modp-trees}
 Let $p$ be a prime and let $H$ be a graph, such that, its order~$p$ reduced form~$H^{*p}$ is a tree. If $H^{*p}$ is a 
star, \phcol{} is computable in polynomial time, otherwise \phcol{} is $\numpp$-complete.
\end{theorem}

\agob{Might have to skip Gregors favourite quote to save space in references.}
Our results are the first to suggest that the conjecture of Faben and Jerrum might apply to counting graph 
homomorphisms modulo every prime~$p$ instead of counting modulo~2. This suggestion, however, remains hypothetical. 
Borrowing the words of Dyer, Frieze and Jerrum~\cite{DFJ02}: ``One might even rashly conjecture'' it ``(though we shall 
not do so)''.

If $H$ is a tree, every induced subgraph of $H$ is also a tree. This includes its order~$p$ reduced form $H^{*p}$, 
giving us the following corollary.

\begin{corollary}
 Let $p$ be a prime and let $H$ be a tree. If the order~$p$ reduced form~$H^{*p}$ of $H$ is a star, \phcol{} is 
computable in polynomial time, otherwise \phcol{} is $\numpp$-complete.
\end{corollary}

We note that, our claim in Figure~\ref{fig:intro_tree} is consistent with Theorem~\ref{thm:modp-trees}, since both the 
order~2 reduced form~$H^{*2}$ and the order~3 reduced form~$H^{*3}$ of $H$ are the graph with one vertex, while for any 
other prime~$p>3$, we have $H=H^{*p}$.

The hardness results that appear in the work of Faben and Jerrum~\cite{DFJ02} and G\"obel, Goldberg and 
Richerby~\cite{GGR14,GGR15} all use as starting point~\paris, the problem of computing the number independent sets 
of a graph~$G$ modulo~2, as a starting point. \paris{} was shown to be $\parp$ complete by 
Valiant~\cite{Val06}. Although 
Faben~\cite{Fab08} gives a hardness proof of \kis{} for all integers~$k$, for technical reasons that will be 
further explained in Section~\ref{sec:intro-our-technique}, we cannot use this problem as a starting point for our 
reductions. Instead we study the complexity of the following problem.

\probpar{\pbislr{\lweight}{\rweight}.\label{prob:bislr}.}
	{$p$ prime and $\lweight, \rweight \in\Z_p$.}
	{A bipartite graph $G=\bipG$.}
	{$\wISet{G} \pmod p$,}
\noindent where $\wISet{G}=\sum_{I\in\calI(G)}\lweight^{|\lpart \cap I|}\rweight^{|\rpart \cap I|}$ and $\calI(G)$ is 
the set of independent sets of~$G$. We obtain the following.
	
\begin{theorem}\label{thm:wbis-hardness}
Let $p$ be a prime and let $\lweight$, $\rweight \in\zp$. If $\lweight \equiv 0 \pmod p$ or $\rweight \equiv 0 \pmod p$ 
then \pbislr{\lweight}{\rweight} is computable in polynomial time. Otherwise, \pbislr{\lweight}{\rweight} is 
\numpp{}-complete.
\end{theorem}

In section~\ref{sec:intro-mod-count} we will provide some background knowledge on modular 
counting. In section~\ref{sec:intro-related-work} we will discuss some related work. In 
section~\ref{sec:intro-our-technique} we explain the technical obstacles that arise when dealing with values 
modulo~$p>2$, and how we overcome them, by generalising the techniques used for modulo~2. Finally, in 
Section~\ref{sec:intro-composites} we will explain why our results work only for prime values~$p$ of the modulo.

\agob{Maybe this should be a footnote on the first page?}
A preliminary version of the results presented here appeared in the second author’s doctoral thesis~\cite{GobThesis}.

\subsection{Modular counting}
\label{sec:intro-mod-count}
The complexity of modular counting is an interesting topic with some surprising results. Modular counting was 
originally studied from the point of view of decision problems, where the objective is to determine if the 
number of solutions is non-zero modulo~$k$. The complexity class $\oplus\pol$ was first studied by Papadimitriou and 
Zachos~\cite{PZ82} and by Goldschlager and Parberry~\cite{GP86:Parallel}. $\oplus\pol$ consists of the all 
problems of the form ``is $f(x)$ odd or even?'', where computing $f(x)$ is a function in $\shp$. Toda~\cite{Tod91} 
has shown that there is a randomised polynomial-time reduction from every problem in the polynomial hierarchy to some 
problem in~$\oplus\pol$. As such, $\oplus\pol$~is a large complexity class and $\oplus\pol$-completeness
seems to represent a high degree of intractability. 

Early work in modular counting~\cite{CH90,Her90,BG92} includes results on the classes $\mathrm{Mod}_k\pol$,
consisting of all the problems of the form ``is $f(x)\not\equiv 0\pmod k$?'', where computing $f(x)$ is a function in 
$\shp$. In our study of \khcol{} it is more natural to consider modular counting from the perspective of computing 
functions. For an integer $k$ the complexity class~$\nkp$ consists of all the problems of the form ``compute $f(x)$ 
modulo~$k$'', where $f(x)$ is a function in~$\shp$. In the special case of $k=2$, $\parp=\oplus\pol$, as the problems 
of $\parp$ require a one bit answer. Throughout this paper though, instead of the more traditional notation 
$\oplus\pol$, we will use $\parp$ to emphasise our interest in computing functions.

% Faben~\cite{Fabenthesis} compares the complexity of the function classes $\nkp$ and the decision classes 
% $\mathrm{Mod}_k\pol$. It is trivial to see that any problem in $\mathrm{Mod}_k\pol$ reduces to a problem in $\nkp$ via 
% Turing reductions. The inverse also holds (\cite[Theorem~3.1.20]{Faben}) as every problem in $\nkp$ reduces to 
% $\mathrm{Mod}_k\sat$, the problem of deciding whether the number of satisfying assignments to a CNF Boolean formula is 
% not divisible by $k$. $\mathrm{Mod}_k\sat$ is complete for $\mathrm{Mod}_k\pol$, as the reduction in Cook's theorem 
% showing the $\np$-completeness of \dsat{} preserves the number of solutions. Finally, 
% Faben~\cite[Theorem~3.1.24]{Fabenthesis} 
% also shows the existence of a $\#_3\pol$-complete problem for which the value is always non-zero, making its modular 
% decision version trivial.

Although counting modulo~$k$ resembles ordinary, non-modular counting, it is still very different. Clearly, 
if a counting problem can be solved in polynomial time, the corresponding decision and modular counting
problems can also be solved in polynomial time. The converse, though, does not necessarily
hold. The characteristic feature that makes the modular version of a hard counting problem tractable is cancellations. 

As an example consider the problem of counting proper $3$-colourings of a graph~$G$ modulo~$3$ (or even 
modulo~$6$). $3$-colourings of a graph that use all of the three colours can be grouped in sets of size~$6$, since 
there are $3!=6$ permutations of the colours. Thus the number of $3$-colourings of a graph that uses all colours is 
always a multiple of $6$, which means all such colourings ``cancel out''. It remains to compute the number of 
$3$-colourings using less than $3$ colours. For computing the number of $3$ colourings of $G$ usinc exactly $2$ 
colours we distinguish the following two cases: either $G$ is not bipartite and there are no such colourings; or $G$ 
is bipartite and the number of $3$-colourings of $G$ that use exactly $2$ colours is $3(2^c)$, where $c$ is the number 
of components of $G$.
%
\footnote{The factor of $3$ comes from the fact that there are $3$ ways to choose $2$-colours. 
To explain the factor $w^c$, assume that we chose the colours in $\{1,2\}$ to colour $G$. Let $G_1\dots G_c$ be the 
components of $G$. Every component $G_i$ of $G$ must be bipartite. For $i\in[c]$, let $V_{i,L}$, $V_{i,R}$ be the 
bipartition of $G_i$ ---since $G_i$ is connected there is only one bipartition of its vertices. If colour~1 is assigned 
to a vertex~$v\in V_{i,L}$, then colour~1 must be assigned to every vertex in $V_{i,L}$, while colour~2 must be 
assigned to every vertex in $V_{i,R}$. Otherwise colour~2 is assigned to every vertex in $V_{i,L}$ (including~$v$) and 
colour~1 is assigned to every vertex in $V_{i,R}$. Hence every component of $G$ can be coloured in two ways, and this 
explains the factor of $2^c$ in the number of the proper $3$-colourings of $G$ that use exactly two colours. } 
%
Finally, it is trivial to compute the number of proper $3$-colourings of 
$G$ that use exactly one colour: if $G$ has an edge, then there are no such colourings; otherwise $G$ has no edges and 
there are $3$ such colourings of $G$, one for each of the three colours.

Perhaps the most surprising feature of modular counting problems is that the value of the modulus can affect the 
tractability of the problem. This can be seen in Valiant's famous restricted version of $3$-SAT  for which counting 
solutions is $\shp$-complete \cite{XZZ07:3-regular}, counting solutions modulo~$7$ is in $\fp$ but counting solutions 
modulo~$2$ is $\parp$-complete \cite{Val06}. The seemingly mysterious number~$7$ was subsequently explained 
by Cai and Lu~\cite{CL11:Holographic}, who showed that the $k$-SAT version of Valiant's problem is tractable modulo any 
prime factor of $2^k-1$.

When studying the complexity of \phcol{} we will use cancellations extensively. For example, if we wish to compute the 
size of a set~$S$ modulo~$p$, then, for any $p$-cardinality subset~$X\subseteq S$, we have $|S|\equiv |S\setminus 
X|\pmod p$.  This means that we can ignore the elements of~$X$.

\subsection{Related work}
\label{sec:intro-related-work}
We have already mentioned earlier work on counting graph homomorphisms and counting graph homomorphisms modulo~2. In 
this section we highlight the work of Guo et al.~\cite{GHLX11} on the complexity of the modular counting variant 
of the constraint satisfaction problem. 

\begin{problem}\label{prb:pcsp}
\begin{description}
\item \emph{Name.} $\kcsp[k](\calF)$.
\item \emph{Parameter.} $k\in\posints$ and a set of functions $\calF=\{f_1\dots f_m\}$, where for each 
$j\in[m]$, $f_j:\{0,1\}^{r_j}\rightarrow \zp$ and $r_j\in\posints$.
\item \emph{Input.} A finite set of constraints over Boolean variables $x_1\dots x_n$ of the form \\ $f_j(x_{i_{j,1}}, 
x_{i_{j,2}},\dots,x_{i_{j,r_j}})$.
\item \emph{Output.} $\sum_{x_1,\dots,x_n\in\{0,1\}}\prod_j f_j(x_{i_{j,1}}, x_{i_{j,2}},\dots,x_{i_{j,r_j}})\pmod k$.
\end{description}
\end{problem}
Their results prove a dichotomy theorem~\cite[Theorem~4.1]{GHLX11} for \kcsp{}, when the domain of the functions 
in~$\calF$ is restricted to the Boolean domain $\{0,1\}$.

Constraint satisfaction problems generalise graph homomorphism problems. To see that \kcsp{} is a generalisation of 
\khcol{}, let $G$ be an input for \khcol{}. We describe an equivalent \kcsp{} instance. The domain of the constraint 
satisfaction problem is $D=V(H)$ and $\Gamma$ contains a single binary relation $R_H$, with $R_H(u,v)=1$ when $(u,v)\in 
E(H)$ and $R_H(u,v)=0$ otherwise. Thus \khcol{} is an instance of $\kcsp(\{R_H\})$. The input of the $\kcsp(\{R_H\})$  
contains a variable~$x_v$ for every vertex $v\in V(G)$ and a constraint~$R_H(x_u,x_v)$ for every edge $(u,v)\in E(G)$. 
As we can see from the construction, every valid homomorphism $\sigma:V(G)\rightarrow V(H)$ corresponds to an 
assignment of the variables $\{x_v\}_{v\in V(G)}$ that satisfies every constraint in the \csp{}.

\agob{I hope I am not downplaying, just want to explain why our results are not subsumed by theirs}
Although our results are more more restrictive compared to the results of Guo et al., as we only consider 
prime values of the modulo and a single binary relation, they are more general as the domain of our relation is 
arbitrarily large.

\subsection{Beyond one-bit functions}
\label{sec:intro-our-technique}
\agob{Do We need to say that we only need to prove hardness? I think its obvious from the description before.}

\paragraph{Pinning}
Every hardness result on modular counting graph homomorphisms uses some ``pinning'' approach. We briefly describe our 
pinning approach. A partial function from a set~$X$ to a set~$Y$ is a function $f:X'\rightarrow Y$ for some 
$X'\subseteq X$. For any graph~$H$, a \emph{partially $H$-labelled graph} $J=(G,\tau)$ consists of an \emph{underlying 
graph}~$G$ and a \emph{pinning function}~$\tau$, which is a partial function from $V(G)$ to~$V(H)$. A homomorphism from 
a partially labelled graph~$J=(G,\tau)$ to~$H$ is a homomorphism $\sigma\colon G\to H$ such that, for all vertices $v\in 
\dom(\tau)$, $\sigma(v) = \tau(v)$. The problem that we study then is \partlabphcol{}, the problem of computing 
$|\Homs{J}{H}| \pmod p$, given a prime~$p$ and graph~$H$ as the parameter of the problem and a partially $H$-labelled 
graph~$J$ as input. In Section~\ref{sec:pinning} we show that \partlabphcol{} reduces to \phcol{}. This allows to 
establish hardness for \phcol{}, by proving hardness for \partlabphcol{}. This reduction, generalises the pinning 
reduction of G\"obel, Goldberg and Richerby~\cite{GGR15} from \partlabparhcol{} to \parhcol{}. To explain the obstacles 
arising when generalising the result of~\cite{GGR15} to all primes~$p$, we explain how to prove pinning when we 
restrict the pinning function $\tau(J)=\{u\mapsto v\}$, to ``pin'' a single vertex.

Assume that the computations are done modulo~2. Given a graph with a distinguished vertex $(G,u)$ and a graph $H$, we 
define~$\vecv_H(G)$ to be the $\{0,1\}$-vector 
containing the entries $|\Homs{(G,u)}{(H,v)}|\pmod p$ for each vertex $v\in V(H)$. Observe that, for two vertices 
$v_1,v_2\in V(H)$, such that $(H,v_1)\isoto(H,v_2)$ and for any graph $G$, the relevant entry in $\vecv_G(H)$ will 
always be the same. Thus, we can contract all such entries and obtain the vectors $\vecv^*_H(G)$. Now suppose that 
there exists a graph with a distinguished vertex $(\Theta,u_\Theta)$, such that $\vecv^*_H(\Theta)=0\dots010\dots0$, 
where the 1-entry corresponds to the vertex $v$ of $H$. Given our input $J$ for \partlabparhcol{}, we can now define an 
input $G$ for \parhcol{}: $G$ contains a disjoint copy of $G(J)$ and $\Theta$, where the vertices $u$ and $u_\Theta$ 
are identified. From the value of $\vecv^*_H(\Theta)$ and the structure of $G$, we can see that there is an even number 
of homomorphisms that map $u$ to any vertex $v'\neq v$. Hence, $|\Homs{J}{H}|\equiv |\Homs{(G,u)}{(H,v)}|\pmod 2$, 
which is what we want.

In reality such a graph $\Theta$ is not guaranteed to exist. Instead we can define a set of operations on the vectors 
$\vecv^*_H$ that correspond to graph operations, and show that for any vector in $\{0,1\}^{|V(H)|}$ there exist a 
sequence of graphs with distinguished vertices $(\Theta_1, u_1), \dots , (\Theta_t, u_t)$ that generate it. Thus, there 
exists a set of graphs that generate $\vecv=0\dots010\dots0$, which gives the desired reduction. This reduction 
technique of~\cite{GGR15} abuses the fact that the value of the modulo is 2. The key observation 
to overcome this technical difficulty and show that this technique works modulo all primes~$p$ is 
that, information
%
\footnote{This information is essentially the number or entries that get contracted, which in the 
modulo 2 case is shown to always be odd.},
%
redundant only in the modulo~2 case, is lost from the contraction of the vectors~$\vecv_H$ 
to the vectors~$\vecv^*_H$. Utilising the the non-contracted vectors~$\vecv_H$, we can, eventually, restore pinning for 
counting homomorphisms modulo any prime~$p$.

\begin{theorem}\label{thm:partlabcol}
Let $p$ be a prime and let $H$ be a graph.
Then \partlabphcol{} reduces to \phcol{} via polynomial-time Turing reduction.
\end{theorem}

We note that our pinning theorem applies to all primes $p$ and all graphs $H$, so it does not restrict the family of 
target graphs to trees. The formal proofs described above are contained in Section~\ref{sec:pinning}.

\paragraph{Gadgets}

Gadgets are structures appearing in the target graph $H$ that allow us to show hardness for \parhcol{} by reducing 
\paris{} to \partlabphcol{} (the hardness of \parhcol{} is then immediate from Theorem~\ref{thm:partlabcol}). 
Simplifying the definitions of~\cite{GGR15} for illustrative purposes, gadgets for~\parhcol{} consist of two partially 
labelled graphs with specified vertices $(J_1,y)$, $(J_2,y,z)$ along with two ``special'' vertices $i,o\in V(H)$. Given 
a graph $G$, input for \paris{}, we construct a graph $G'$, input for \partlabparhcol{}, by attaching a copy of $J_1$ to 
every vertex~$u$ of $G$ (identifying $u$ with $y$) and replacing every edge of $G$ with a copy of $J_2$ (identifying $u$ 
with $y$ and $v$ with $z$). 
\agob{I could site the construction in our square-free paper, where we have a figure, but I have simplified the 
notation here: in the cactus there where 3 gadagets, and I merged the two of them into one.}
The properties of $J_1$ ensure that there is an odd number of homomorphisms from $G'$ to 
$H$ where the original vertices of $G$ are mapped to $i$ or $o$ and the rest homomorphisms cancel out. The properties 
of $J_2$ ensure that there is an even number of homomorphisms from $G'$ to $H$ when two adjacent vertices of $G$ are 
both 
mapped to $i$, and an odd number of homomorphisms in any other case. We can see now that $|\calI(G)|\equiv 
|\Homs{G'}{H}\pmod2$, as the set of homomorphisms that does not cancel out must map every vertex of $G$ to $i$ or $o$ 
and no adjacent vertices both to $i$ --- that is every vertex of $G$ that is in an independent set must be mapped 
to~$i$, in the corresponding homomorphism from $G'$ to $H$, and every vertex that is out of the independent set must be 
mapped to $o$. 

When counting modulo~$p>2$, the edge interaction gadget $J_2$ does not only differentiate between odd or even, but it 
differentiates between 1 and $\gamma\in\zp\setminus\{1\}$, i.e. the number of homomorphisms~$\sigma$ such that, for 
every pair of vertices $u,v\in V(G')$, where $u,v$ adjacent in $G$, is equivalent to $\gamma\not\equiv 1\pmod p$, while 
in any other case, this number is equivalent to 1 modulo~$p$. This obstacle can be overcome by using an appropriate 
\pcsp{}-instance as a  starting problem, utilising~\cite[Theorem~4.1]{GHLX11}. This \pcsp{} instance contains a 
single binary function~$f_e$, where $f_e(i,i)=\gamma$ and in any other case $f_e$ takes the value 1. For such a 
construction we refer the reader to~\cite[Section~3]{GobThesis}.

A bigger challenge comes when, additionally to $J_2$, now the vertex gadget $J_1$ does not only choose between two 
vertices, $i$ and $o$, but instead chooses between two sets of isomorphic vertices $I$ and $O$. An example of 
this can be seen in the graph $H$ of Figure~\ref{fig:intro_tree}. The vertices labelled $u_j$ ($v_j$ resp.) are 
isomorphic to each other, i.e. $(H,u_1)\isoto(H,u_2)$. So, for every homomorphism $\sigma$, such that for each $w\in 
V(G')$, $\sigma(w)=u_1$, there exists a homomorphism $\sigma'$, with $\sigma'(w)=u_2$ and for each $w'\neq w$, 
$\sigma'(w')=\sigma(w')$. So if $I=\{u_1,u_2\}$ for example, we have two possible choices of a type~$i$ vertex.
This, in the relevant \csp{} problem, introduces a unary weight of two which applies to every variable of the input 
(this is known as \emph{external field} in statistical physics). Now, the starting \pcsp{} instance has a restricted 
input form and the \kcsp{} dichotomy no longer applies. Proving hardness for \pcsp{} instances with an external 
field is rather challenging, even if we only consider them to contain only one binary relation. Instead we 
follow a simpler approach.

To explain our reduction, formally presented in Section~\ref{sec:trees}, we return to our example graph $H$ of 
Figure~\ref{fig:intro_tree}. Let $G=(V_L,V_R,E)$ 
be a bipartite graph. Homomorphisms from $G$ to $H$ must respect the partitioning of $G$, i.e. the vertices in $V_L$ 
can only be mapped to the vertices in $\{x_L,u_1,u_2,u_3\}$ and the vertices in $V_R$ can only be mapped to the vertices 
in $\{x_R, v_1, v_2\}$, or vice versa. Any homomorphism~$\sigma$ from~$G$ to~$H$, with $\sigma(w)\in\{u_1,u_2\}$, must 
map every vertex that is adjacent to~$w$ to~$x_R$. Similarly, any homomorphism from~$G$ to~$H$ with 
$\sigma(w)\in\{v_1,v_2,v_2\}$ must map every vertex that is adjacent to~$w$ to~$x_L$. Thus, homomorphisms 
from~$G$ to~$H$ correspond to independent sets of $G$: $\{u_1,u_2,u_3\}$ represent the vertices of $V_L$ that are in the 
independent set while $\{v_1,v_2\}$ represent the vertices of $V_R$ that are in the independent set, and vice versa. To 
fix the choice of $V_L$ and $V_R$ in the set homomorphisms from $G$ to $H$, we construct a partially labelled graph 
$J$ from $G$. $G(J)$ contains a copy of $G$, \agob{I followed the notation of Definition~\ref{def:gadget_wBIS_to_Homs}, 
but I am not content with that notation. See the section for my comment.} 
where every vertex in $V_L$ is attached to the new vertex $u_L$ and every vertex in $V_R$ is attached to the 
new vertex $v_R$. Let $\tau(J)=\{u_L\mapsto x_L,v_R\mapsto x_R\}$. It is easy to see now, that the vertices of $V_L$ 
can only be mapped to vertices in $\{x_L,u_1,u_2,u_3\}$ and vertices of $V_R$ can only be mapped to vertices 
in $\{x_R, v_1, v_2\}$. We have argued that the number of homomorphisms from $J$ to $H$ is equivalent to $Z_{3,2}(G)$ 
(recall the definition of $Z_{\lweight,\rweight}$ directly after Problem~\ref{prob:bislr}).

The properties of $H$ that we needed for the reduction above is the existence of two adjacent vertices of degree 
$a=\lweight+1\not\equiv 1\pmod p$ and $b=\rweight+1\not \equiv 1 \pmod p$ --- this is because, we need 
$\lweight,\rweight\not\equiv 0 \pmod p$ to obtain hardness (recall Theorem~\ref{thm:wbis-hardness}). It turns out that 
these vertices not need to be adjacent, as, during the construction of $J$, we can replace the edges of $G$ with paths 
of appropriate length. We call such a structure in $H$ an $(a,b,p)$-path. In Lemma~\ref{lem:Homs_trees_hardcase} we 
formally prove that if $H$ has an $(a,b,p)$-path, then \parhcol{} is hard. Observe that stars cannot contain 
$(a,b,p)$-paths. Finally, we show that every non-star tree~$H$ contains an $(a,b,p)$-path, which gives us our 
main result on \phcol{} (Lemma~\ref{lem:tree_star_or_hard}).

\paragraph{Weighted bipartite independent sets}

To prove Theorem~\ref{thm:wbis-hardness}, first, consider a bipartite graph $G=(V_L,V_R,E)$ and let $\lweight=0$ (the 
case $\rweight=0$ is symmetric). We observe that every independent set~$I$ contributing to $\wISet{G}$ contains only 
vertices of $V_R$. Now we can obtain the closed form $\wISet{G}=(\rweight+1)^{|V_R|}$, which we can compute in 
polynomial time. For the case $\lweight,\rweight\not\equiv 0 \pmod p$, we generalise a reduction of Faben~\cite[Theorem 
3.7]{Fab08}. Faben reduces \numpsat{}, the ``canonical'' $\numpp{}$-complete problem, to the problem of counting 
independent sets of a bipartite graph. 

In our weighted setting, since we allow different vertex weights for the
vertices of each partition, we must keep track during the construction, which vertex gets assigned to which 
part. Additionally, we need to show the existence of bipartite graphs~$B$, for which 
$\wISet{B}$ takes specific values. We can then attach these graphs as gadgets in our reduction. In 
the ``unweighted'' set setting of \pbislr{1}{1}, the graphs~$B$ were complete bipartite graphs. In our weighted setting 
of \pbislr{\lweight}{\rweight} we prove the existence the necessary bipartite gadgets~$B$ constructively. The technical 
proofs appear in Section~\ref{sec:bipartite}.

\subsection{Composites}
\label{sec:intro-composites}

We briefly explain why we are not able to give a dichotomy for \khcol{} for all integers~$k$. Let $H$ be a graph and 
let $k=\prod_{j=1}^m p_j^{r_j}$ be an integer and its the prime factorisation. If \khcol{} can be 
solved in polynomial time, then for each $j\in[m]$,  
$\#_{p_j^{r_j}}\prb{HomsTo}H$ can also be solved in polynomial time: since $p_j^{r_j}$ is a factor of $k$ we take the 
solution of \khcol{} modulo~$p_j^{r_j}$ and obtain a solution for  $\#_{p_j^{r_j}}\prb{HomsTo}H$. We can apply the 
Chinese remainder theorem, (Theorem~\ref{thm:chinese-remainder}) to show that the inverse is also true: if for each 
$j\in[m]$ we can solve $\#_{p_j^{r_j}}\prb{HomsTo}H$ in polynomial time, then we can also solve \khcol{} in polynomial 
time.

Now we can focus on integers of the form $k=p^r$, where $p$ is a prime and $r$ is a positive integer. If \khcol{} is 
computable in polynomial time then so is \phcol{}, by simply taking the solution of \khcol{} modulo~$p$. The 
inverse does not always hold. Surprisingly, Guo et al.~\cite{GHLX11} were able to obtain such a result for the 
constraint satisfaction problem. They were able to show~\cite[Lemma~4.1 and Lemma~4.3]{GHLX11} that, when $p$ is a 
prime, $\kcsp[{p^r}]$ is computable in polynomial time if \pcsp{} is computable in polynomial time.

Naturally, one would ask if the techniques of Guo et al., see~\cite[Lemma~16 and Lemma~18]{GHLX11} for \kcsp{} can be 
transferred to the setting of~\khcol{}. In Section~\ref{sec:composites} we give a negative answer to this question: we 
show that there is a graph~($P_4$) such that $\#_2\prb{HomsTo}P_4$ is computable in polynomial time, while 
$\#_4\prb{HomsTo}P_4$ is $\parp$-hard.

A direct approach might seem more appropriate to determine the complexity of \khcol{} for all integers~$k$. In this 
case fundamental obstacles arise, as neither the polynomial time algorithm of Faben and Jerrum, nor the pinning 
techniques we use to prove hardness seem to work. New approaches would be needed to generalise our results to all 
integers~$k$.


\subsection{Organisation}
\label{sec:organisation}
In Section~\ref{sec:prelim} we introduce notation. In Section~\ref{sec:bipartite} we study the complexity of the 
weighted bipartite independent sets problem modulo all primes. Section~\ref{sec:poly} presents the polynomial time 
algorithm of Faben and Jerrum for \phcol{}. In Section~\ref{sec:pinning} we deal with pinning. Section~\ref{sec:trees} 
contains the hardness reduction for \phcol{}. Section~\ref{sec:main-thm} collects all our results into the dichotomy 
theorem. Finally, in Section~\ref{sec:composites} we discuss the complications that arise when counting modulo all 
integers.
